Non-thermal radio supernova remnants of exiled Wolf-Rayet stars

A signification fraction of Galactic massive stars (> 8Mo) are ejected from their parent cluster and supersonically sail away through the interstellar medium (ISM). The winds of these fast-moving stars blow asymmetric bubbles thus creating a circumstellar environment in which stars eventually die with a supernova explosion. The morphology of the resulting remnant is largely governed by the circumstellar medium of the defunct progenitor star. In this paper, we present 2D magneto-hydrodynamical simulations investigating the effect of the ISM magnetic field on the shape of the supernova remnants of a 35Mo star evolving through a Wolf-Rayet phase and running with velocity 20 and 40 km/s, respectively. A 7 microG ambient magnetic field is sufficient to modify the properties of the expanding supernova shock front and in particular to prevent the formation of filamentary structures. Prior to the supernova explosion, the compressed magnetic field in the circumstellar medium stabilises the wind/ISM contact discontinuity in the tail of the wind bubble. A consequence is a reduced mixing efficiency of ejecta and wind materials in the inner region of the remnant, where the supernova shock wave propagates. Radiative transfer calculations for synchrotron emission reveal that the non-thermal radio emission has characteristic features reflecting the asymmetry of exiled core-collapse supernova remnants from Wolf-Rayet progenitors. Our models are qualitatively consistent with the radio appearance of several remnants of high-mass progenitors, namely the bilateral G296.5+10.0 and the shell-type remnants CTB109 and Kes 17, respectively.

==> grid <==
@ARTICLE{2019A&A...627A.166B,
       author = {{Brose}, R. and {Sushch}, I. and {Pohl}, M. and {Luken}, K.~J. and {Filipovi{\'c}}, M.~D. and {Lin}, R.},
        title = "{Nonthermal emission from the reverse shock of the youngest Galactic supernova remnant G1.9+0.3}",
      journal = {\aap},
     keywords = {acceleration of particles, turbulence, ISM: supernova remnants, gamma rays: ISM, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = jul,
       volume = {627},
          eid = {A166},
        pages = {A166},
          doi = {10.1051/0004-6361/201834430},
archivePrefix = {arXiv},
       eprint = {1906.02725},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...627A.166B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2008ARA&A..46...89R,
       author = {{Reynolds}, S.~P.},
        title = "{Supernova remnants at high energy.}",
      journal = {\araa},
         year = 2008,
        month = sep,
       volume = {46},
        pages = {89-126},
          doi = {10.1146/annurev.astro.46.060407.145237},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008ARA&A..46...89R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%% High energy bow shocks

@ARTICLE{DeBecker_mnras_471_2017,
       author = {{De Becker}, M. and {del Valle}, M.~V. and {Romero}, G.~E. and
         {Peri}, C.~S. and {Benaglia}, P.},
        title = "{X-ray study of bow shocks in runaway stars}",
      journal = {\mnras},
     keywords = {acceleration of particles, radiation mechanisms: non-thermal, stars: early-type, X-rays: stars, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2017",
        month = "Nov",
       volume = {471},
       number = {4},
        pages = {4452-4464},
          doi = {10.1093/mnras/stx1826},
archivePrefix = {arXiv},
       eprint = {1708.04082},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.471.4452D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{binder_aj_157_2019,
       author = {{Binder}, Breanna A. and {Behr}, Patrick and {Povich}, Matthew S.},
        title = "{Searching for Faint X-Ray Emission from Galactic Stellar Wind Bow Shocks}",
      journal = {\aj},
     keywords = {circumstellar matter, stars: massive, stars: winds, outflows, X-rays: ISM, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2019",
        month = "May",
       volume = {157},
       number = {5},
          eid = {176},
        pages = {176},
          doi = {10.3847/1538-3881/ab1073},
archivePrefix = {arXiv},
       eprint = {1903.06279},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019AJ....157..176B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{tola_apj_838_2017,
   author = {{Toal{\'a}}, J.~A. and {Oskinova}, L.~M. and {Ignace}, R.},
    title = "{On the Absence of Non-thermal X-Ray Emission around Runaway O Stars}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1703.04059},
 primaryClass = "astro-ph.HE",
 keywords = {stars: massive, stars: mass-loss, stars: winds, outflows, X-rays: ISM},
     year = 2017,
    month = apr,
   volume = 838,
      eid = {L19},
    pages = {L19},
      doi = {10.3847/2041-8213/aa667c},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2017ApJ...838L..19T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{delvalle_mnras_448_2015,
       author = {{del Valle}, M.~V. and {Romero}, G.~E. and {Santos-Lima}, R.},
        title = "{Runaway stars as cosmic ray injectors inside molecular clouds}",
      journal = {\mnras},
     keywords = {radiation mechanisms: non-thermal, ISM: clouds, cosmic rays, gamma-rays: ISM, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2015",
        month = "Mar",
       volume = {448},
       number = {1},
        pages = {207-220},
          doi = {10.1093/mnras/stu2732},
archivePrefix = {arXiv},
       eprint = {1412.6535},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.448..207D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{delvalle_apj_864_2018,
       author = {{del Valle}, M.~V. and {Pohl}, M.},
        title = "{Nonthermal Emission from Stellar Bow Shocks}",
      journal = {\apj},
     keywords = {gamma-rays: stars, hydrodynamics, radiation mechanisms: nonthermal, stars: winds, outflows, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2018",
        month = "Sep",
       volume = {864},
       number = {1},
          eid = {19},
        pages = {19},
          doi = {10.3847/1538-4357/aad333},
archivePrefix = {arXiv},
       eprint = {1807.05895},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...864...19D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{delvalle_aa_563_2014,
   author = {{del Valle}, M.~V. and {Romero}, G.~E.},
    title = "{Runaway massive stars as variable gamma-ray sources}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1401.3255},
 primaryClass = "astro-ph.HE",
 keywords = {stars: massive, gamma rays: stars, radiation mechanisms: non-thermal},
     year = 2014,
    month = mar,
   volume = 563,
      eid = {A96},
    pages = {A96},
      doi = {10.1051/0004-6361/201322308},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014A%26A...563A..96D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{delvalle_aa_550_2013,
   author = {{del Valle}, M.~V. and {Romero}, G.~E. and {De Becker}, M.},
    title = "{Is the bowshock of the runaway massive star HD 195592 a Fermi source?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1212.1549},
 primaryClass = "astro-ph.HE",
 keywords = {stars: early-type, gamma-rays: general, radiation mechanisms: non-thermal, stars individual: HD 195592},
     year = 2013,
    month = feb,
   volume = 550,
      eid = {A112},
    pages = {A112},
      doi = {10.1051/0004-6361/201220112},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2013A%26A...550A.112D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{schultz_aa_565_2014,
   author = {{Schulz}, A. and {Ackermann}, M. and {Buehler}, R. and {Mayer}, M. and 
	{Klepser}, S.},
    title = "{Systematic search for high-energy gamma-ray emission from bow shocks of runaway stars}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1404.4059},
 primaryClass = "astro-ph.HE",
 keywords = {radiation mechanisms: non-thermal, gamma rays: ISM, stars: early-type, stars: individual:{$\zeta$}Ophiuchi},
     year = 2014,
    month = may,
   volume = 565,
      eid = {A95},
    pages = {A95},
      doi = {10.1051/0004-6361/201423468},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014A%26A...565A..95S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{benaglia_aa_399_2003,
       author = {{Benaglia}, P. and {Romero}, G.~E.},
        title = "{Gamma-ray emission from Wolf-Rayet binaries}",
      journal = {\aap},
     keywords = {stars: early-type, stars: binaries: general, stars: winds, outflows, radio continuum: stars, gamma-rays: observations, gamma-rays: theory, Astrophysics},
         year = "2003",
        month = "Mar",
       volume = {399},
        pages = {1121-1134},
          doi = {10.1051/0004-6361:20021854},
archivePrefix = {arXiv},
       eprint = {astro-ph/0205375},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003A&A...399.1121B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{benaglia_aa_517_2010,
   author = {{Benaglia}, P. and {Romero}, G.~E. and {Mart{\'{\i}}}, J. and 
	{Peri}, C.~S. and {Araudo}, A.~T.},
    title = "{Detection of nonthermal emission from the bow shock of a massive runaway star}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1007.3279},
 primaryClass = "astro-ph.SR",
 keywords = {stars: early-type, stars: individual: BD+43{\deg}3654, radio continuum: general, infrared: stars},
     year = 2010,
    month = jul,
   volume = 517,
      eid = {L10},
    pages = {L10},
      doi = {10.1051/0004-6361/201015232},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2010A%26A...517L..10B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pereira_aa_588_2016,
   author = {{Pereira}, V. and {L{\'o}pez-Santiago}, J. and {Miceli}, M. and 
	{Bonito}, R. and {de Castro}, E.},
    title = "{Modeling nonthermal emission from stellar bow shocks}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1603.00309},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, radiation mechanisms: non-thermal, shock waves, X-rays: ISM},
     year = 2016,
    month = apr,
   volume = 588,
      eid = {A36},
    pages = {A36},
      doi = {10.1051/0004-6361/201527985},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2016A%26A...588A..36P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE B 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{bhatt_apj_aph_2020,
       author = {{Bhatt}, Maulik and {Sushch}, Iurii and {Pohl}, Martin and {Fedynitch}, Anatoli and {Das}, Samata and {Brose}, Robert and {Plotko}, Pavlo and {Meyer}, Dominique M. -A.},
        title = "{Production of secondary particles in heavy nuclei interactions in supernova remnants}",
      journal = {Astroparticle Physics},
     keywords = {Cosmic rays, Gamma rays, Abundances, Supernova remnants 95.85.Pw, 95.85.Ry, 98.35.Bd, 98.38.Mz, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2020,
        month = dec,
       volume = {123},
          eid = {102490},
        pages = {102490},
          doi = {10.1016/j.astropartphys.2020.102490},
archivePrefix = {arXiv},
       eprint = {2006.07018},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020APh...12302490B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@INPROCEEDINGS{bally_prpl_2007,
       author = {{Bally}, J. and {Reipurth}, B. and {Davis}, C.~J.},
        title = "{Observations of Jets and Outflows from Young Stars}",
    booktitle = {Protostars and Planets V},
         year = 2007,
       editor = {{Reipurth}, Bo and {Jewitt}, David and {Keil}, Klaus},
        month = jan,
        pages = {215},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007prpl.conf..215B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{bestenlehner_aa_570_2014,
       author = {{Bestenlehner}, J.~M. and {Gr{\"a}fener}, G. and {Vink}, J.~S. et al. },
        title = "{The VLT-FLAMES Tarantula Survey. XVII. Physical and wind properties of massive stars at the top of the main sequence}",
      journal = {\aap},
     keywords = {stars: Wolf-Rayet, stars: early-type, stars: atmospheres, stars: mass-loss, stars: fundamental parameters, Astrophysics - Solar and Stellar Astrophysics},
         year = 2014,
        month = oct,
       volume = {570},
          eid = {A38},
        pages = {A38},
          doi = {10.1051/0004-6361/201423643},
archivePrefix = {arXiv},
       eprint = {1407.1837},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...570A..38B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bolte_aa_582_2015,
       author = {{Bolte}, J. and {Sasaki}, M. and {Breitschwerdt}, D.},
        title = "{3D hydrodynamic simulations of the Galactic supernova remnant CTB 109}",
      journal = {\aap},
     keywords = {ISM: supernova remnants, evolution, shock waves, hydrodynamics, methods: numerical, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2015",
        month = "Oct",
       volume = {582},
          eid = {A47},
        pages = {A47},
          doi = {10.1051/0004-6361/201526000},
archivePrefix = {arXiv},
       eprint = {1508.05868},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...582A..47B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{arias_aa_627_2019,
       author = {{Arias}, M. and {Dom{\v{c}}ek}, V. and {Zhou}, P. and {Vink}, J.},
        title = "{The environment of supernova remnant VRO 42.05.01 as probed with IRAM 30m molecular line observations}",
      journal = {\aap},
     keywords = {ISM: supernova remnants, ISM: clouds, ISM: molecules, ISM: general, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2019,
        month = jul,
       volume = {627},
          eid = {A75},
        pages = {A75},
          doi = {10.1051/0004-6361/201935528},
archivePrefix = {arXiv},
       eprint = {1906.03801},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...627A..75A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{arias_aa_622_2019,
       author = {{Arias}, M. and {Vink}, J. and {Iacobelli}, M. and {Dom{\v{c}}ek}, V. and
         {Haverkorn}, M. and {Oonk}, J.~B.~R. and {Polderman}, I. and
         {Reich}, W. and {White}, G.~J. and {Zhou}, P.},
        title = "{A low-frequency view of mixed-morphology supernova remnant VRO 42.05.01, and its neighbourhood}",
      journal = {\aap},
     keywords = {ISM: supernova remnants, HII regions, ISM: individual objects: VRO 42.05.01, ISM: individual objects: OA 184, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2019",
        month = "Feb",
       volume = {622},
          eid = {A6},
        pages = {A6},
          doi = {10.1051/0004-6361/201833865},
archivePrefix = {arXiv},
       eprint = {1810.07584},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...622A...6A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{acke_aa_457_2006,
   author = {{Acke}, B. and {van den Ancker}, M.~E.},
    title = "{A survey for nanodiamond features in the 3 micron spectra of Herbig Ae/Be stars}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0606650},
 keywords = {circumstellar matter, stars: pre-main-sequence, planetary systems: protoplanetary disks},
     year = 2006,
    month = oct,
   volume = 457,
    pages = {171-181},
      doi = {10.1051/0004-6361:20065612},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...457..171A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{acreman_mnras_456_2016,
   author = {{Acreman}, D.~M. and {Stevens}, I.~R. and {Harries}, T.~J.},
    title = "{Modelling multiwavelength observational characteristics of bow shocks from runaway early-type stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1511.03059},
 primaryClass = "astro-ph.SR",
 keywords = {stars: early-type, ISM: general},
     year = 2016,
    month = feb,
   volume = 456,
    pages = {136-145},
      doi = {10.1093/mnras/stv2632},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2016MNRAS.456..136A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{aschenbach_aa_341_1999,
   author = {{Aschenbach}, B. and {Leahy}, D.~A.},
    title = "{ROSAT all-sky survey map of the Cygnus Loop: Overall structure and comparison with radio map}",
  journal = {\aap},
 keywords = {SHOCK WAVES, ISM: CYGNUS LOOP, ISM: SUPERNOVA REMNANTS, X-RAYS: ISM},
     year = 1999,
    month = jan,
   volume = 341,
    pages = {602-609},
   adsurl = {http://adsabs.harvard.edu/abs/1999A%26A...341..602A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{arthur_apjs_165_2006,
   author = {{Arthur}, S.~J. and {Hoare}, M.~G.},
    title = "{Hydrodynamics of Cometary Compact H II Regions}",
  journal = {\apjs},
   eprint = {astro-ph/0511035},
 keywords = {ISM: H II Regions, ISM: Kinematics and Dynamics, Shock Waves, Stars: Formation, Stars: Winds, Outflows},
     year = 2006,
    month = jul,
   volume = 165,
    pages = {283-306},
      doi = {10.1086/503899},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJS..165..283A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{avedisova_saj_15_1972,
   author = {{Avedisova}, V.~S.},
    title = "{Formation of Nebulae by Wolf-Rayet Stars.}",
  journal = {\sovast},
     year = 1972,
    month = apr,
   volume = 15,
    pages = {708},
   adsurl = {http://adsabs.harvard.edu/abs/1972SvA....15..708A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{abbott_apj_242_1980,
   author = {{Abbott}, D.~C.},
    title = "{The theory of radiatively driven stellar winds. I - A physical interpretation}",
  journal = {\apj},
 keywords = {EARLY STARS, RADIATIVE TRANSFER, STELLAR MASS EJECTION, STELLAR WINDS, GAS PRESSURE, INTERSTELLAR MATTER, MATHEMATICAL MODELS, SOUND WAVES, STELLAR MAGNETIC FIELDS, STELLAR ROTATION, WAVE PROPAGATION},
     year = 1980,
    month = dec,
   volume = 242,
    pages = {1183-1207},
      doi = {10.1086/158550},
   adsurl = {http://adsabs.harvard.edu/abs/1980ApJ...242.1183A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{abbott_apl_311_1986,
   author = {{Friend}, D.~B. and {Abbott}, D.~C.},
    title = "{The theory of radiatively driven stellar winds. III - Wind models with finite disk correction and rotation}",
  journal = {\apj},
 keywords = {STELLAR MASS EJECTION, STELLAR MODELS, STELLAR ROTATION, STELLAR WINDS, CENTRIFUGAL FORCE, EQUATIONS OF MOTION, HOT STARS, WIND VELOCITY},
     year = 1986,
    month = dec,
   volume = 311,
    pages = {701-707},
      doi = {10.1086/164809},
   adsurl = {http://adsabs.harvard.edu/abs/1986ApJ...311..701F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{abbott_apj_259_1982,
   author = {{Abbott}, D.~C.},
    title = "{The theory of radiatively driven stellar winds. II - The line acceleration}",
  journal = {\apj},
 keywords = {LINE SPECTRA, RADIATION PRESSURE, STELLAR ENVELOPES, STELLAR MASS EJECTION, STELLAR SPECTRA, STELLAR WINDS, B STARS, EARLY STARS, O STARS, STELLAR TEMPERATURE, SUPERGIANT STARS, WOLF-RAYET STARS},
     year = 1982,
    month = aug,
   volume = 259,
    pages = {282-301},
      doi = {10.1086/160166},
   adsurl = {http://adsabs.harvard.edu/abs/1982ApJ...259..282A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{abdo_apj_722_2010,
   author = {{Abdo}, A.~A. and {Ackermann}, M. and {Ajello}, M.
	},
    title = "{Fermi-LAT Study of Gamma-ray Emission in the Direction of Supernova Remnant W49B}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1008.4190},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, ISM: individual objects: W49B, radiation mechanisms: non-thermal},
     year = 2010,
    month = oct,
   volume = 722,
    pages = {1303-1311},
      doi = {10.1088/0004-637X/722/2/1303},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...722.1303A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{alexiades_cnme_12_1996,
   author = {{Alexiades}, V. and {Amiez}, G. and {Gremaud}, P.-A.},
    title = "{Super-time-stepping acceleration of explicit schemes for parabolic problems}",
  journal = {Communication in Numerical Methods in Engineering},
     year = 1996,
   volume = 12,
    pages = {31-42},
}

@INPROCEEDINGS{arnaud_aspc_101_1996,
   author = {{Arnaud}, K.~A.},
    title = "{XSPEC: The First Ten Years}",
booktitle = {Astronomical Data Analysis Software and Systems V},
     year = 1996,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 101,
   editor = {{Jacoby}, G.~H. and {Barnes}, J.},
    pages = {17},
   adsurl = {http://adsabs.harvard.edu/abs/1996ASPC..101...17A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{asplund_araa_47_2009,
   author = {{Asplund}, M. and {Grevesse}, N. and {Sauval}, A.~J. and {Scott}, P.
	},
    title = "{The Chemical Composition of the Sun}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {0909.0948},
 primaryClass = "astro-ph.SR",
     year = 2009,
    month = sep,
   volume = 47,
    pages = {481-522},
      doi = {10.1146/annurev.astro.46.060407.145222},
   adsurl = {http://adsabs.harvard.edu/abs/2009ARA%26A..47..481A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{avilaaroche_mnras_420_2020,
       author = {{{\'A}vila-Aroche}, A. and {Vel{\'a}zquez}, P.~F. and {Camps-Fari{\~n}a}, A. and {Toledo-Roy}, J.~C. and {Esquivel}, A.},
        title = "{Young bilateral supernova remnants evolving into a turbulent interstellar magnetic field}",
      journal = {\mnras},
     keywords = {MHD, polarization, radiation mechanisms: non-thermal, methods: numerical, ISM: supernova remnants},
         year = 2020,
        month = may,
       volume = {495},
       number = {2},
        pages = {2112-2124},
          doi = {10.1093/mnras/staa1301},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.495.2112A},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE B 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{debecker_mnras_371_2006,
       author = {{De Becker}, M. and {Rauw}, G. and {Sana}, H. and {Pollock}, A.~M.~T. and
         {Pittard}, J.~M. and {Blomme}, R. and {Stevens}, I.~R. and
         {van Loo}, S.},
        title = "{XMM-Newton observations of the massive colliding wind binary and non-thermal radio emitter CygOB2\#8A [O6If + O5.5III(f)]}",
      journal = {\mnras},
     keywords = {stars: binaries: general: stars: early-type: stars: individual: CygOB2\#8A: stars: winds, outflows: X-rays: stars, stars: binaries: general, stars: early-type, stars: individual: CygOB2\#8A, stars: winds, outflows, X-rays: stars},
         year = "2006",
        month = "Sep",
       volume = {371},
       number = {3},
        pages = {1280-1294},
          doi = {10.1111/j.1365-2966.2006.10746.x},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006MNRAS.371.1280D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{debecker_aa_558_2013,
       author = {{De Becker}, M. and {Raucq}, F.},
        title = "{Catalogue of particle-accelerating colliding-wind binaries}",
      journal = {\aap},
     keywords = {stars: massive, binaries: general, radiation mechanisms: non-thermal, acceleration of particles, radio continuum: stars, gamma rays: stars, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = "2013",
        month = "Oct",
       volume = {558},
          eid = {A28},
        pages = {A28},
          doi = {10.1051/0004-6361/201322074},
archivePrefix = {arXiv},
       eprint = {1308.3149},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...558A..28D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{brose_aa_593_2016,
       author = {{Brose}, R. and {Telezhinsky}, I. and {Pohl}, M.},
        title = "{Transport of magnetic turbulence in supernova remnants}",
      journal = {\aap},
     keywords = {ISM: supernova remnants, acceleration of particles, turbulence, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2016",
        month = "Aug",
       volume = {593},
          eid = {A20},
        pages = {A20},
          doi = {10.1051/0004-6361/201527345},
archivePrefix = {arXiv},
       eprint = {1606.04477},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016A&A...593A..20B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{brose_aa_627_2019,
       author = {{Brose}, R. and {Sushch}, I. and {Pohl}, M. and {Luken}, K.~J. and
         {Filipovi{\'c}}, M.~D. and {Lin}, R.},
        title = "{Nonthermal emission from the reverse shock of the youngest Galactic supernova remnant G1.9+0.3}",
      journal = {\aap},
     keywords = {acceleration of particles, turbulence, ISM: supernova remnants, gamma rays: ISM, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2019",
        month = "Jul",
       volume = {627},
          eid = {A166},
        pages = {A166},
          doi = {10.1051/0004-6361/201834430},
archivePrefix = {arXiv},
       eprint = {1906.02725},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...627A.166B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{binder_2019arXiv190306279B,
   author = {{Binder}, B.~A. and {Behr}, P. and {Povich}, M.~S.},
    title = "{Searching for Faint X-ray Emission from Galactic Stellar Wind Bow Shocks}",
  journal = {arXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1903.06279},
 primaryClass = "astro-ph.HE",
 keywords = {Astrophysics - High Energy Astrophysical Phenomena},
     year = 2019,
    month = mar,
   adsurl = {http://adsabs.harvard.edu/abs/2019arXiv190306279B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{baade_apj_88_1938,
   author = {{Baade}, W.},
    title = "{The Absolute Photographic Magnitude of Supernovae.}",
  journal = {\apj},
     year = 1938,
    month = oct,
   volume = 88,
    pages = {285},
      doi = {10.1086/143983},
   adsurl = {http://adsabs.harvard.edu/abs/1938ApJ....88..285B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{badenes_mnras_407_2010,
   author = {{Badenes}, C. and {Maoz}, D. and {Draine}, B.~T.},
    title = "{On the size distribution of supernova remnants in the Magellanic Clouds}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1003.3030},
 primaryClass = "astro-ph.GA",
 keywords = {supernovae: general, ISM: supernova remnants, galaxies: individual: LMC, galaxies: individual: SMC},
     year = 2010,
    month = sep,
   volume = 407,
    pages = {1301-1313},
      doi = {10.1111/j.1365-2966.2010.17023.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.407.1301B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{balsara_mnras_386_2008,
   author = {{Balsara}, D.~S. and {Tilley}, D.~A. and {Howk}, J.~C.},
    title = "{Simulating anisotropic thermal conduction in supernova remnants - I. Numerical methods}",
  journal = {\mnras},
 keywords = {conduction , MHD , methods: numerical , supernova remnants},
     year = 2008,
    month = may,
   volume = 386,
    pages = {627-641},
      doi = {10.1111/j.1365-2966.2008.13085.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2008MNRAS.386..627B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{baranov_jgr_1993,
   author = {{Baranov}, V.~B. and {Malama}, Y.~G.},
    title = "{Model of the solar wind interaction with the local interstellar medium - Numerical solution of self-consistent problem}",
  journal = {\jgr},
 keywords = {Flow Distribution, Interstellar Matter, Magnetohydrodynamic Flow, Plasma Composition, Plasma-Particle Interactions, Solar Wind, Hydrogen Atoms, Iterative Solution, Mathematical Models, Monte Carlo Method},
     year = 1993,
    month = sep,
   volume = 98,
    pages = {15157},
      doi = {10.1029/93JA01171},
   adsurl = {http://adsabs.harvard.edu/abs/1993JGR....9815157B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{baranov_sovastronlett_1_1975,
   author = {{Baranov}, V.~B. and {Krasnobaev}, K.~V. and {Onishchenko}, O.~G.
	},
    title = "{Proposed experimental test of a model for interaction between the solar wind and the interstellar medium}",
  journal = {Soviet Astronomy Letters},
 keywords = {ASTRONOMICAL MODELS, INTERSTELLAR MATTER, PLASMA-PARTICLE INTERACTIONS, SOLAR WIND, PULSARS, QUASARS, RADIO ASTRONOMY, SCINTILLATION, SUPERSONIC FLOW},
     year = 1975,
    month = apr,
   volume = 1,
    pages = {81},
   adsurl = {http://adsabs.harvard.edu/abs/1975SvAL....1...81B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{baranov_sphd_15_1971,
   author = {{Baranov}, V.~B. and {Krasnobaev}, K.~V. and {Kulikovskii}, A.~G.
	},
    title = "{A Model of the Interaction of the Solar Wind with the Interstellar Medium}",
  journal = {Soviet Physics Doklady},
     year = 1971,
    month = mar,
   volume = 15,
    pages = {791},
   adsurl = {http://adsabs.harvard.edu/abs/1971SPhD...15..791B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{balsara_MNRAS_386_2008a,
   author = {{Balsara}, D.~S. and {Bendinelli}, A.~J. and {Tilley}, D.~A. and 
	{Massari}, A.~R. and {Howk}, J.~C.},
    title = "{Simulating anisotropic thermal conduction in supernova remnants - 
    II. Implications for the interstellar medium}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0711.2295},
 keywords = {conduction , MHD , ISM: evolution , supernova remnants , X-rays: ISM},
     year = 2008,
    month = may,
   volume = 386,
    pages = {642-656},
      doi = {10.1111/j.1365-2966.2008.13121.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.386..642B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{balsara_MNRAS_386_2008b,
   author = {{Balsara}, D.~S. and {Tilley}, D.~A. and {Howk}, J.~C.},
    title = "{Simulating anisotropic thermal conduction in supernova remnants - I. Numerical methods}",
  journal = {\mnras},
 keywords = {conduction , MHD , methods: numerical , supernova remnants},
     year = 2008,
    month = may,
   volume = 386,
    pages = {627-641},
      doi = {10.1111/j.1365-2966.2008.13085.x},
   adsurl = {http://adsabs.harvard.edu/abs/2008MNRAS.386..627B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{bedogni_190_aa_1988,
   author = {{Bedogni}, R. and {D'Ercole}, A.},
    title = "{The electron thermal conduction in young supernova remnants}",
  journal = {\aap},
 keywords = {Astronomical Models, Conductive Heat Transfer, Supernova Remnants, Computational Astrophysics, Heat Flux, Hydrodynamic Equations, Plasma Turbulence, Shock Waves, Stellar Winds},
     year = 1988,
    month = jan,
   volume = 190,
    pages = {320-332},
   adsurl = {http://adsabs.harvard.edu/abs/1988A%26A...190..320B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bjorkman_paj_554_2001,
   author = {{Bjorkman}, J.~E. and {Wood}, K.},
    title = "{Radiative Equilibrium and Temperature Correction in Monte Carlo Radiation Transfer}",
  journal = {\apj},
   eprint = {astro-ph/0103249},
 keywords = {Stars: Circumstellar Matter, ISM: Dust, Extinction, Radiative Transfer, Scattering},
     year = 2001,
    month = jun,
   volume = 554,
    pages = {615-623},
      doi = {10.1086/321336},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2001ApJ...554..615B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{blaauw_bain_15_1961,
   author = {{Blaauw}, A.},
    title = "{On the origin of the O- and B-type stars with high velocities (the ''run-away'' stars), and some related problems}",
  journal = {\bain},
     year = 1961,
    month = may,
   volume = 15,
    pages = {265},
   adsurl = {http://adsabs.harvard.edu/abs/1961BAN....15..265B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{blandford_301_natur_1983,
   author = {{Blandford}, R.~D. and {Kennel}, C.~F. and {McKee}, C.~F. and 
	{Ostriker}, J.~P.},
    title = "{Trail of the Crab progenitor star}",
  journal = {\nat},
 keywords = {Astronomical Models, Crab Nebula, Red Giant Stars, Stellar Winds, Emission Spectra, H Lines, Jets, Oxygen, Stellar Mass Ejection},
     year = 1983,
    month = feb,
   volume = 301,
    pages = {586},
      doi = {10.1038/301586a0},
   adsurl = {http://adsabs.harvard.edu/abs/1983Natur.301..586B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{blau1993ASPC...35..207B,
   author = {{Blaauw}, A.},
    title = "{Massive Runaway Stars}",
booktitle = {Massive Stars:  Their Lives in the Interstellar Medium},
     year = 1993,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 35,
   editor = {{Cassinelli}, J.~P. and {Churchwell}, E.~B.},
    month = jan,
    pages = {207},
   adsurl = {http://adsabs.harvard.edu/abs/1993ASPC...35..207B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bjorkman_apj_409_1993,
   author = {{Bjorkman}, J.~E. and {Cassinelli}, J.~P.},
    title = "{Equatorial disk formation around rotating stars due to Ram pressure confinement by the stellar wind}",
  journal = {\apj},
 keywords = {B STARS, EARLY STARS, ROTATING DISKS, STELLAR ENVELOPES, STELLAR MASS EJECTION, STELLAR ROTATION, STELLAR WINDS, ANGULAR VELOCITY, EMISSION SPECTRA, LINE SPECTRA, STELLAR SPECTRA},
     year = 1993,
    month = may,
   volume = 409,
    pages = {429-449},
      doi = {10.1086/172676},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...409..429B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{benaglia_aa_517_2010,
   author = {{Benaglia}, P. and {Romero}, G.~E. and {Mart{\'{\i}}}, J. and 
	{Peri}, C.~S. and {Araudo}, A.~T.},
    title = "{Detection of nonthermal emission from the bow shock of a massive runaway star}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1007.3279},
 primaryClass = "astro-ph.SR",
 keywords = {stars: early-type, stars: individual: BD+43{\deg}3654, radio continuum: general, infrared: stars},
     year = 2010,
    month = jul,
   volume = 517,
      eid = {L10},
    pages = {L10},
      doi = {10.1051/0004-6361/201015232},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...517L..10B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{beuther_aa_503_2009,
   author = {{Beuther}, H. and {Henning}, T.},
    title = "{Multiple low-turbulence starless cores associated with intermediate- to high-mass star formation}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0907.4565},
 primaryClass = "astro-ph.SR",
 keywords = {stars: formation, stars: individual: IRDC 19175-4, IRDC 19175-5, techniques: interferometric, line: formation, line: profiles, turbulence},
     year = 2009,
    month = sep,
   volume = 503,
    pages = {859-867},
      doi = {10.1051/0004-6361/200912036},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...503..859B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{boulanger_aa_312_1996,
   author = {{Boulanger}, F. and {Abergel}, A. and {Bernard}, J.-P. and {Burton}, W.~B. and 
	{Desert}, F.-X. and {Hartmann}, D. and {Lagache}, G. and {Puget}, J.-L.
	},
    title = "{The dust/gas correlation at high Galactic latitude.}",
  journal = {\aap},
 keywords = {ISM: ATOMS, ISM: DUST, EXTINCTION, ISM: MOLECULES, ISM: GENERAL, INFRARED: INTERSTELLAR: CONTINUUM},
     year = 1996,
    month = aug,
   volume = 312,
    pages = {256-262},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26A...312..256B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{bohren_book_1983,
   author = {{Bohren}, C.~F. and {Huffman}, D.~R.},
    title = "{Absorption and scattering of light by small particles}",
 keywords = {LIGHT SCATTERING, ABSORPTION, PARTICLES, DUST, THEORY},
booktitle = {New York: Wiley, 1983},
     year = 1983,
   adsurl = {http://adsabs.harvard.edu/abs/1983asls.book.....B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{borkowski_apj_400_1992,
   author = {{Borkowski}, K.~J. and {Blondin}, J.~M. and {Sarazin}, C.~L.
	},
    title = "{Dynamics of Kepler's supernova remnant}",
  journal = {\apj},
 keywords = {Hydrodynamics, Interstellar Matter, Kepler Laws, Stellar Envelopes, Stellar Winds, Supernova Remnants, Milky Way Galaxy, Shock Wave Interaction, Stellar Mass Ejection, Taylor Instability},
     year = 1992,
    month = nov,
   volume = 400,
    pages = {222-237},
      doi = {10.1086/171989},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...400..222B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bowler_aj_137_2009,
   author = {{Bowler}, B.~P. and {Waller}, W.~H. and {Megeath}, S.~T. and 
	{Patten}, B.~M. and {Tamura}, M.},
    title = "{An Infrared Census of Star Formation in the Horsehead Nebula}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {0901.0564},
 primaryClass = "astro-ph.SR",
 keywords = {ISM: clouds, ISM: globules, ISM: individual: Horsehead Nebula, stars: formation, stars: pre-main sequence},
     year = 2009,
    month = mar,
   volume = 137,
    pages = {3685-3699},
      doi = {10.1088/0004-6256/137/3/3685},
   adsurl = {http://adsabs.harvard.edu/abs/2009AJ....137.3685B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{blondin_apj_472_1996,
   author = {{Blondin}, J.~M. and {Lundqvist}, P. and {Chevalier}, R.~A.},
    title = "{Axisymmetric Circumstellar Interaction in Supernovae}",
  journal = {\apj},
   eprint = {astro-ph/9601137},
 keywords = {STARS: CIRCUMSTELLAR MATTER, HYDRODYNAMICS, ISM: STRUCTURE, SHOCK WAVES, ISM: SUPERNOVA REMNANTS, STARS: SUPERNOVAE: GENERAL},
     year = 1996,
    month = nov,
   volume = 472,
    pages = {257},
      doi = {10.1086/178060},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...472..257B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{blondin_na_57_1998,
   author = {{Blondin}, J.~M. and {Koerwer}, J.~F.},
    title = "{Instability of isothermal stellar wind bowshocks}",
  journal = {\na},
 keywords = {Hydrodynamics, Instabilities, Shock waves, Circumstellar matter, Hydrodynamics, Circumstellar shells, clouds, and expanding envelopes; circumstellar masers, Mass loss and stellar winds},
     year = 1998,
    month = dec,
   volume = 3,
    pages = {571-582},
      doi = {10.1016/S1384-1076(98)00028-1},
   adsurl = {http://adsabs.harvard.edu/abs/1998NewA....3..571B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Unpublished{ braithwait_2011b,
	title = "An introduction to hydrodynamics and astrophysical manetohydrodynamics",
	author = "J. Braithwait",
	note = "Aifa lecture note",
	month = "March",
	year = "2011"
}

@Unpublished{braithwait_2011a,
	title = "An introduction to astrophysical manetohydrodynamics",
	author = "J. Braithwait",
	note = "Aifa lecture note"
}


@ARTICLE{brighenti_mnras_273_1995,
   author = {{Brighenti}, F. and {D'Ercole}, A.},
    title = "{Evolution of WR ring nebulae generated by moving central stars - I. The paradigm of G2.4+1.4}",
  journal = {\mnras},
 keywords = {STARS: MASS-LOSS, STARS: WOLF-RAYET, ISM: BUBBLES, ISM: INDIVIDUAL: G2.4+1.4.},
     year = 1995,
    month = mar,
   volume = 273,
    pages = {443-448},
   adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.273..443B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{brighenti_mnras_277_1995,
   author = {{Brighenti}, F. and {D'Ercole}, A.},
    title = "{Evolution of WR ring nebulae generated by a moving central star - II. The influence of the red supergiant bow shock}",
  journal = {\mnras},
 keywords = {HYDRODYNAMICS, INSTABILITIES, STARS: WOLF-RAYET, ISM: BUBBLES},
     year = 1995,
    month = nov,
   volume = 277,
    pages = {53-69},
   adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.277...53B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{brighenti_mnras_270_1994,
   author = {{Brighenti}, F. and {D'Ercole}, A.},
    title = "{Evolution of Supernova Remnants Generated by Moving Massive Stars}",
  journal = {\mnras},
     year = 1994,
    month = sep,
   volume = 270,
    pages = {65},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1994MNRAS.270...65B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{brott_aa_530_2011b,
   author = {{Brott}, I. and {Evans}, C.~J. and {Hunter}, I. and {de Koter}, A. and 
	{Langer}, N. and {Dufton}, P.~L. and {Cantiello}, M. and {Trundle}, C. and 
	{Lennon}, D.~J. and {de Mink}, S.~E. and {Yoon}, S.-C. and {Anders}, P.
	},
    title = "{Rotating massive main-sequence stars. II. Simulating a population of LMC early B-type stars as a test of rotational mixing}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1102.0766},
 primaryClass = "astro-ph.SR",
 keywords = {methods: statistical, stars: abundances, stars: evolution, stars: early-type, stars: massive, stars: rotation},
     year = 2011,
    month = jun,
   volume = 530,
      eid = {A116},
    pages = {A116},
      doi = {10.1051/0004-6361/201016114},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...530A.116B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{brott_aa_530_2011a,
   author = {{Brott}, I. and {de Mink}, S.~E. and {Cantiello}, M. and {Langer}, N. and 
	{de Koter}, A. and {Evans}, C.~J. and {Hunter}, I. and {Trundle}, C. and 
	{Vink}, J.~S.},
    title = "{Rotating massive main-sequence stars. I. Grids of evolutionary models and isochrones}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1102.0530},
 primaryClass = "astro-ph.SR",
 keywords = {stars: abundances, stars: evolution, stars: early-type, stars: rotation, stars: massive},
     year = 2011,
    month = jun,
   volume = 530,
      eid = {A115},
    pages = {A115},
      doi = {10.1051/0004-6361/201016113},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...530A.115B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{brown_aa_439_2005,
   author = {{Brown}, D. and {Bomans}, D.~J.},
    title = "{To see or not to see a bow shock. Identifying bow shocks with H{$\alpha$} allsky surveys}",
  journal = {\aap},
   eprint = {astro-ph/0505098},
 keywords = {stars: early-type, stars: kinematics, stars: mass-loss, ISM: bubble, ISM: structure},
     year = 2005,
    month = aug,
   volume = 439,
    pages = {183-194},
      doi = {10.1051/0004-6361:20041054},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2005A%26A...439..183B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{bucciantini_aa_405_2003,
   author = {{Bucciantini}, N. and {Blondin}, J.~M. and {Del Zanna}, L. and 
	{Amato}, E.},
    title = "{Spherically symmetric relativistic MHD simulations of pulsar wind nebulae in supernova remnants}",
  journal = {\aap},
   eprint = {astro-ph/0303491},
 keywords = {ISM: supernova remnants, stars: pulsars: general, stars: winds, outflows, magnetohydrodynamics, shock waves, relativity},
     year = 2003,
    month = jul,
   volume = 405,
    pages = {617-626},
      doi = {10.1051/0004-6361:20030624},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...405..617B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{burlaga_apj_804_2015,
   author = {{Burlaga}, L.~F. and {Florinski}, V. and {Ness}, N.~F.},
    title = "{In Situ Observations of Magnetic Turbulence in the Local Interstellar Medium}",
  journal = {\apjl},
 keywords = {ISM: magnetic fields},
     year = 2015,
    month = may,
   volume = 804,
      eid = {L31},
    pages = {L31},
      doi = {10.1088/2041-8205/804/2/L31},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...804L..31B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{buren_apj_329_1988,
   author = {{van Buren}, D. and {McCray}, R.},
    title = "{Bow shocks and bubbles are seen around hot stars by IRAS}",
  journal = {\apjl},
 keywords = {BOW WAVES, EARLY STARS, HOT STARS, INFRARED STARS, INTERSTELLAR MATTER, PLASMA BUBBLES, STELLAR WINDS, COSMIC DUST, H II REGIONS, INFRARED ASTRONOMY SATELLITE, RADIATION PRESSURE, STELLAR LUMINOSITY},
     year = 1988,
    month = jun,
   volume = 329,
    pages = {L93-L96},
      doi = {10.1086/185184},
   adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...329L..93V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE C 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{castro_apj_756_2012,
       author = {{Castro}, Daniel and {Slane}, Patrick and {Ellison}, Donald C. and {Patnaude}, Daniel J.},
        title = "{Fermi-LAT Observations and a Broadband Study of Supernova Remnant CTB 109}",
      journal = {\apj},
     keywords = {acceleration of particles, cosmic rays, gamma rays: ISM, ISM: individual objects: CTB 109, ISM: supernova remnants, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2012,
        month = sep,
       volume = {756},
       number = {1},
          eid = {88},
        pages = {88},
          doi = {10.1088/0004-637X/756/1/88},
archivePrefix = {arXiv},
       eprint = {1207.1432},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...756...88C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{castro_apj_734_2011,
       author = {{Castro}, D. and {Slane}, P.~O. and {Gaensler}, B.~M. and {Hughes}, J.~P. and {Patnaude}, D.~J.},
        title = "{An XMM-Newton Study of the Bright, Nearby Supernova Remnant G296.1-0.5}",
      journal = {\apj},
     keywords = {ISM: individual objects: G296.1-0.5, ISM: supernova remnants, X-rays: individual: G296.1-0.5 2XMMi J115004.8-622442, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2011,
        month = jun,
       volume = {734},
       number = {2},
          eid = {86},
        pages = {86},
          doi = {10.1088/0004-637X/734/2/86},
archivePrefix = {arXiv},
       eprint = {1104.1423},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...734...86C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{caswell_mnras_187_1979,
       author = {{Caswell}, J.~L. and {Lerche}, I.},
        title = "{Galactic supernova remnants: dependence of radio brightness on galactic height and its implications.}",
      journal = {\mnras},
     keywords = {Brightness, Scale Height, Shells (Structural Forms), Supernova Remnants, Interstellar Magnetic Fields, Loops, Pulsars, Astrophysics, Radio Radiation:Supernova Remnants},
         year = 1979,
        month = apr,
       volume = {187},
        pages = {201-216},
          doi = {10.1093/mnras/187.2.201},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1979MNRAS.187..201C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{coe_mnras_238_1989,
       author = {{Coe}, M.~J. and {Davies}, S.~R. and {Fahlman}, G.~G. and
         {Gregory}, P.~C.},
        title = "{The far-IR structure of the SNR G 109.1-1.0.}",
      journal = {\mnras},
     keywords = {Far Infrared Radiation, Infrared Astronomy Satellite, Molecular Clouds, Pulsars, Supernova Remnants, X Ray Sources, Astronomical Maps, Binary Stars, Heao 2, Astrophysics},
         year = "1989",
        month = "May",
       volume = {238},
        pages = {649-655},
          doi = {10.1093/mnras/238.2.649},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1989MNRAS.238..649C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2019arXiv190908947C,
       author = {{Chiotellis}, A. and {Boumis}, P. and {Derlopa}, S. and {Steffen}, W.},
        title = "{VRO 42.05.01: A supernova remnant resulted by a supersonic, mass losing progenitor star}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = "2019",
        month = "Sep",
          eid = {arXiv:1909.08947},
        pages = {arXiv:1909.08947},
archivePrefix = {arXiv},
       eprint = {1909.08947},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190908947C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{cichowolski_aa_478_2008,
       author = {{Cichowolski}, S. and {Pineault}, S. and {Arnal}, E.~M. and
         {Cappa}, C.~E.},
        title = "{VLA and Effelsberg observations of the interstellar medium around the runaway star WR 124}",
      journal = {\aap},
     keywords = {ISM: bubbles, ISM: individual objects: WR 124, stars: Wolf-Rayet, ISM: H II regions},
         year = "2008",
        month = "Feb",
       volume = {478},
       number = {2},
        pages = {443-452},
          doi = {10.1051/0004-6361:20078339},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2008A&A...478..443C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{chu_apj_599_2003,
       author = {{Chu}, You-Hua and {Guerrero}, Mart{\'\i}n A. and {Gruendl}, Robert A. and
         {Garc{\'\i}a-Segura}, Guillermo and {Wendker}, Heinrich J.},
        title = "{Hot Gas in the Circumstellar Bubble S308}",
      journal = {\apj},
     keywords = {ISM: Bubbles, ISM: Individual: Alphanumeric: S308, Stars: Individual: Henry Draper Number: HD 50896, Stars: Winds, Outflows, Stars: Wolf-Rayet, X-rays: Individual: Alphanumeric: S308, Astrophysics},
         year = "2003",
        month = "Dec",
       volume = {599},
       number = {2},
        pages = {1189-1195},
          doi = {10.1086/379607},
archivePrefix = {arXiv},
       eprint = {astro-ph/0309192},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...599.1189C},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@INPROCEEDINGS{castor_apj_200_1975,
   author = {{Castor}, J.~I. and {McCray}, R. and {Weaver}, R.},
    title = "{Interstellar Bubbles}",
booktitle = {Bulletin of the American Astronomical Society},
     year = 1975,
   series = {Bulletin of the American Astronomical Society},
   volume = 7,
    month = jun,
    pages = {428},
   adsurl = {http://adsabs.harvard.edu/abs/1975BAAS....7..428C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ciotti_aa_215_1989,
   author = {{Ciotti}, L. and {D'Ercole}, A.},
    title = "{SNR expansion in a pre-existent cavity}",
  journal = {\aap},
 keywords = {B STARS, COMPUTATIONAL ASTROPHYSICS, O STARS, STELLAR WINDS, SUPERNOVA REMNANTS, ASTRONOMICAL MODELS, STELLAR TEMPERATURE, WAVE PROPAGATION},
     year = 1989,
    month = may,
   volume = 215,
    pages = {347-359},
   adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...215..347C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{cherchneff_proc_232_1994,
   author = {{Cherchneff}, I. and {Tielens}, A.~G.~G.~M.},
    title = "{Mass loss from late type stars}",
booktitle = {Circumstellar Media in Late Stages of Stellar Evolution},
     year = 1994,
   editor = {{Clegg}, R.~E.~S. and {Stevens}, I.~R. and {Meikle}, W.~P.~S.
	},
    pages = {232},
   adsurl = {http://adsabs.harvard.edu/abs/1994cmls.conf..232C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{chevalier_apj_344_1989,
   author = {{Chevalier}, R.~A. and {Liang}, E.~P.},
    title = "{The interaction of supernovae with circumstellar bubbles}",
  journal = {\apj},
 keywords = {STELLAR ENVELOPES, STELLAR WINDS, SUPERNOVA REMNANTS, SUPERNOVAE, RADIO SOURCES (ASTRONOMY), SHOCK WAVES, STELLAR EVOLUTION, STELLAR MASS, SUPERNOVA 1987A, X RAY SOURCES},
     year = 1989,
    month = sep,
   volume = 344,
    pages = {332-340},
      doi = {10.1086/167802},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...344..332C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{chevalier_apj_258_1982,
   author = {{Chevalier}, R.~A.},
    title = "{Self-similar solutions for the interaction of stellar ejecta with an external medium}",
  journal = {\apj},
 keywords = {Interstellar Matter, Stellar Mass Ejection, Supernova Remnants, Density Distribution, Gas Density, Gas-Gas Interactions, Gas-Solid Interactions, Light Curve, X Ray Spectra},
     year = 1982,
    month = jul,
   volume = 258,
    pages = {790-797},
      doi = {10.1086/160126},
   adsurl = {http://adsabs.harvard.edu/abs/1982ApJ...258..790C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@PhDThesis{ chita_phd_2011,
	title = "Models for circumstellar nebulae around red and blue supergiant",
	author = "S. M. Chita",
	school = "Utrecht University",
	month = "September",
	year = "2011",
	address = "Netherland"
}

@INPROCEEDINGS{chita_revmexaa_30_2007,
   author = {{Chita}, S.~M. and {van Marle}, A.~J. and {Langer}, N. and {Garc{\'{\i}}a-Segura}, G.
	},
    title = "{The Evolution of Circumstellar Medium around Rotating Massive Stars}",
 keywords = {Hydrodynamics, ISM: bubbles, Stars: supergiants, Stars: winds, outflows},
booktitle = {Revista Mexicana de Astronomia y Astrofisica Conference Series},
     year = 2007,
   series = {Revista Mexicana de Astronomia y Astrofisica Conference Series},
   volume = 30,
    month = aug,
    pages = {80-83},
   adsurl = {http://adsabs.harvard.edu/abs/2007RMxAC..30...80C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{chita_aa_488_2008,
   author = {{Chita}, S.~M. and {Langer}, N. and {van Marle}, A.~J. and {Garc{\'{\i}}a-Segura}, G. and 
	{Heger}, A.},
    title = "{Multiple ring nebulae around blue supergiants}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0807.3049},
 keywords = {hydrodynamics, ISM: bubbles, stars: winds, outflows, stars: supergiants},
     year = 2008,
    month = sep,
   volume = 488,
    pages = {L37-L41},
      doi = {10.1051/0004-6361:200810087},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...488L..37C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{chiotellis_aa_537_2012,
   author = {{Chiotellis}, A. and {Schure}, K.~M. and {Vink}, J.},
    title = "{The imprint of a symbiotic binary progenitor on the properties of Kepler's supernova remnant}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1103.5487},
 primaryClass = "astro-ph.GA",
 keywords = {ISM: supernova remnants, hydrodynamics, binaries: symbiotic, supernovae: individual: SN1604},
     year = 2012,
    month = jan,
   volume = 537,
      eid = {A139},
    pages = {A139},
      doi = {10.1051/0004-6361/201014754},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...537A.139C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{comeron_aa_326_1997,
   author = {{Comer\`{o}n}, F.},
    title = "{Dynamical evolution of wind-driven HII regions in strong density gradients.}",
  journal = {\aap},
 keywords = {STARS: EARLY-TYPE, ISM: BUBBLES, CLOUDS, HII REGIONS, KINEMATICS AND DYNAMICS, HYDRODYNAMICS},
     year = 1997,
    month = oct,
   volume = 326,
    pages = {1195-1214},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...326.1195C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{comeron_aa_338_1998,
   author = {{Comer\'{o}n}, F. and {Kaper}, L.},
    title = "{Numerical simulations of wind bow shocks produced by runaway OB stars}",
  journal = {\aap},
 keywords = {SHOCK WAVES, STARS: EARLY-TYPE, ISM: BUBBLES, ISM: KINEMATICS AND DYNAMICS},
     year = 1998,
    month = oct,
   volume = 338,
    pages = {273-291},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...338..273C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{compiegne_aa_491_2008,
   author = {{Compi{\`e}gne}, M. and {Abergel}, A. and {Verstraete}, L. and 
	{Habart}, E.},
    title = "{Dust processing in photodissociation regions. Mid-IR emission modelling}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0809.5026},
 keywords = {ISM: individual objects: Horsehead, ISM: individual objects: NGC 2023, ISM: dust, extinction, infrared: ISM},
     year = 2008,
    month = dec,
   volume = 491,
    pages = {797-807},
      doi = {10.1051/0004-6361:200809850},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...491..797C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{conlon_aa_236_1990,
   author = {{Conlon}, E.~S. and {Dufton}, P.~L. and {Keenan}, F.~P. and 
	{Leonard}, P.~J.~T.},
    title = "{The runaway nature of distant early-type stars in the galactic halo}",
  journal = {\aap},
 keywords = {B STARS, BINARY STARS, BLUE STARS, EARLY STARS, GALACTIC STRUCTURE, STELLAR EVOLUTION, MANY BODY PROBLEM, MASS TRANSFER, OPEN CLUSTERS, REFERENCE STARS, STELLAR MASS, SUPERNOVAE},
     year = 1990,
    month = sep,
   volume = 236,
    pages = {357-361},
   adsurl = {http://adsabs.harvard.edu/abs/1990A%26A...236..357C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{couch_aspc_393_2008,
   author = {{Couch}, S.~M. and {Wheeler}, J.~C. and {Milosavljevi{\'c}}, M.
	},
    title = "{Hydrodynamic Instabilities in Jet-Induced Supernovae: Results of 2D Simulations}",
booktitle = {New Horizons in Astronomy},
     year = 2008,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 393,
   editor = "{A.~Frebel, J.~R.~Maund, J.~Shen, \& M.~H.~Siegel}",
    month = aug,
    pages = {183},
   adsurl = {http://adsabs.harvard.edu/abs/2008ASPC..393..183C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cox_apj_178_1974,
   author = {{Cox}, D.~P.},
    title = "{Cooling and Evolution of a Supernova Remnant}",
  journal = {\apj},
     year = 1972,
    month = nov,
   volume = 178,
    pages = {159-168},
      doi = {10.1086/151775},
   adsurl = {http://adsabs.harvard.edu/abs/1972ApJ...178..159C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{cox_aa_537_2012,
   author = {{Cox}, N.~L.~J. and {Kerschbaum}, F. and {van Marle}, A.~J. and {Decin}, L. and {Ladjal}, D. and {Mayer}, A.},
    title = "{A far-infrared survey of bow shocks and detached shells around AGB stars and red supergiants (Corrigendum)}",
  journal = {\aap},
 keywords = {stars: AGB and post-AGB, circumstellar matter, infrared: ISM, hydrodynamics, stars: mass-loss, errata, addenda},
     year = 2012,
    month = jul,
   volume = 543,
      eid = {C1},
    pages = {C1},
      doi = {10.1051/0004-6361/201117910e},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012A},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cox_mnras_250_1991,
   author = {{Cox}, C.~I. and {Gull}, S.~F. and {Green}, D.~A.},
    title = "{Numerical simulations of the 'jet' in the Crab nebula}",
  journal = {\mnras},
 keywords = {Crab Nebula, Stellar Models, Stellar Winds, Cool Stars, Cooling Flows (Astrophysics), Digital Simulation, Plasma Jets, Supernova Remnants},
     year = 1991,
    month = jun,
   volume = 250,
    pages = {750-759},
   adsurl = {http://adsabs.harvard.edu/abs/1991MNRAS.250..750C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{cowie_apj_211_1977,
   author = {{Cowie}, L.~L. and {McKee}, C.~F.},
    title = "{The evaporation of spherical clouds in a hot gas. I - Classical and saturated mass loss rates}",
  journal = {\apj},
 keywords = {EVAPORATION, HIGH TEMPERATURE GASES, INTERSTELLAR GAS, NEBULAE, SUPERNOVA REMNANTS, CONDUCTIVE HEAT TRANSFER, HEAT FLUX, MASS FLOW RATE, SOLAR WIND, TEMPERATURE PROFILES},
     year = 1977,
    month = jan,
   volume = 211,
    pages = {135-146},
      doi = {10.1086/154911},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...211..135C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{crutcher_apj_515_1999,
   author = {{Crutcher}, R.~M. and {Roberts}, D.~A. and {Troland}, T.~H. and 
	{Goss}, W.~M.},
    title = "{The Magnetic Field of the NGC 2024 Molecular Cloud}",
  journal = {\apj},
 keywords = {ISM: CLOUDS, ISM: INDIVIDUAL (NGC 2024), ISM: KINEMATICS AND DYNAMICS, ISM: MAGNETIC FIELDS, ISM: MOLECULES, ISM: Clouds, ISM: individual (NGC 2024), ISM: Kinematics and Dynamics, ISM: Magnetic Fields, ISM: Molecules},
     year = 1999,
    month = apr,
   volume = 515,
    pages = {275-285},
      doi = {10.1086/307026},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...515..275C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE D 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



@ARTICLE{drury_rpph_46_1983,
       author = {{Drury}, L. Oc.},
        title = "{REVIEW ARTICLE: An introduction to the theory of diffusive shock acceleration of energetic particles in tenuous plasmas}",
      journal = {Reports on Progress in Physics},
     keywords = {Energetic Particles, Particle Acceleration, Plasma-Particle Interactions, Rarefied Plasmas, Shock Wave Propagation, Kinematics, Nonlinear Systems, Oblique Shock Waves, Plane Waves, Rankine-Hugoniot Relation, Time Dependence, Plasma Physics},
         year = 1983,
        month = aug,
       volume = {46},
       number = {8},
        pages = {973-1027},
          doi = {10.1088/0034-4885/46/8/002},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1983RPPh...46..973D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{drury_ssrv_36_1983,
       author = {{Drury}, L.},
        title = "{On Particle Acceleration in Supernova Remnants}",
      journal = {\ssr},
     keywords = {Energetic Particles, Gamma Ray Astronomy, Particle Acceleration, Supernova Remnants, Radio Emission, Shock Waves, Synchrotron Radiation, Astrophysics},
         year = 1983,
        month = sep,
       volume = {36},
       number = {1},
        pages = {57-60},
          doi = {10.1007/BF00171901},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1983SSRv...36...57D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{dincel_mnras_448_2015,
       author = {{Din{\c{c}}el}, B. and {Neuh{\"a}user}, R. and {Yerli}, S.~K. and
         {Ankay}, A. and {Tetzlaff}, N. and {Torres}, G. and {Mugrauer}, M.},
        title = "{Discovery of an OB runaway star inside SNR S147}",
      journal = {\mnras},
     keywords = {stars: early type, stars: individual: HD37424, pulsars: individual: PSR J0538+2817, ISM: individual objects: SNR G180.0-1.7 (S147), ISM: supernova remnants, Astrophysics - Solar and Stellar Astrophysics},
         year = "2015",
        month = "Apr",
       volume = {448},
       number = {4},
        pages = {3196-3205},
          doi = {10.1093/mnras/stv124},
archivePrefix = {arXiv},
       eprint = {1501.07220},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.448.3196D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{dincel_mnras_448_2015,
       author = {{Din{\c{c}}el}, B. and {Neuh{\"a}user}, R. and {Yerli}, S.~K. and
         {Ankay}, A. and {Tetzlaff}, N. and {Torres}, G. and {Mugrauer}, M.},
        title = "{Discovery of an OB runaway star inside SNR S147}",
      journal = {\mnras},
     keywords = {stars: early type, stars: individual: HD37424, pulsars: individual: PSR J0538+2817, ISM: individual objects: SNR G180.0-1.7 (S147), ISM: supernova remnants, Astrophysics - Solar and Stellar Astrophysics},
         year = "2015",
        month = "Apr",
       volume = {448},
       number = {4},
        pages = {3196-3205},
          doi = {10.1093/mnras/stv124},
archivePrefix = {arXiv},
       eprint = {1501.07220},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.448.3196D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2019arXiv190906131D,
       author = {{Derlopa}, Sophia and {Boumis}, Panos and {Chiotellis}, Alexandros and
         {Steffen}, Wolfgang and {Akras}, Stavros},
        title = "{The first 3D Morpho-kinematical model of a Supernova Remnant: The case of VRO 42.05.01 (G 166.0+4.3)}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Sep",
          eid = {arXiv:1909.06131},
        pages = {arXiv:1909.06131},
archivePrefix = {arXiv},
       eprint = {1909.06131},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190906131D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{deBecker_mnras_471_2017,
   author = {{De Becker}, M. and {del Valle}, M.~V. and {Romero}, G.~E. and 
	{Peri}, C.~S. and {Benaglia}, P.},
    title = "{X-ray study of bow shocks in runaway stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1708.04082},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, radiation mechanisms: non-thermal, stars: early-type, X-rays: stars},
     year = 2017,
    month = nov,
   volume = 471,
    pages = {4452-4464},
      doi = {10.1093/mnras/stx1826},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.471.4452D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{davies_apj_671_2007,
   author = {{Davies}, R.~I. and {M{\"u}ller S{\'a}nchez}, F. and {Genzel}, R. and 
	{Tacconi}, L.~J. and {Hicks}, E.~K.~S. and {Friedrich}, S. and 
	{Sternberg}, A.},
    title = "{A Close Look at Star Formation around Active Galactic Nuclei}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0704.1374},
 keywords = {Galaxies: Active, Galaxies: Nuclei, Galaxies: Seyfert, Galaxies: Starburst, Infrared: Galaxies},
     year = 2007,
    month = dec,
   volume = 671,
    pages = {1388-1412},
      doi = {10.1086/523032},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...671.1388D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{desterck_aipc_537_2000,
   author = {{de Sterck}, H. and {Poedts}, S.},
    title = "{Disintegration and reformation of intermediate shock segments in 3D MHD bow shock flows}",
 keywords = {Magnetohydrodynamics and plasmas, Magnetohydrodynamic waves, Shock waves and discontinuities, Magnetohydrodynamic and fluid equation},
booktitle = {Waves in Dusty, Solar, and Space Plasmas},
     year = 2000,
   series = {American Institute of Physics Conference Series},
   volume = 537,
   editor = {{Verheest}, F. and {Goossens}, M. and {Hellberg}, M.~A. and 
	{Bharuthram}, R.},
    month = oct,
    pages = {232-239},
      doi = {10.1063/1.1324945},
   adsurl = {http://adsabs.harvard.edu/abs/2000AIPC..537..232D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{desterck_2001,
   author = {{de Sterck}, H. and {Poedts}, S.},
    title = "{Overcompressive shocks and compound shocks in 2D and 3D magnetohydrodynamic flows}",
 keywords = {Magnetohydrodynamics and plasmas, Magnetohydrodynamic waves, Shock waves and discontinuities, Magnetohydrodynamic and fluid equation},
booktitle = {Waves in Dusty, Solar, and Space Plasmas},
     year = 2001,
   series = {International Series of Numerical Mathematics},
   volume = 141,
   editor = {{Freistühler}, H. and {Warnecke}, G.},
    month = feb,
    pages = {791-801}
}

@ARTICLE{decin_asr_50_2012,
   author = {{Decin}, L.},
    title = "{Late stages of stellar evolution - Herschel's contributions}",
  journal = {Advances in Space Research},
archivePrefix = "arXiv",
   eprint = {1212.4861},
 primaryClass = "astro-ph.SR",
     year = 2012,
    month = oct,
   volume = 50,
    pages = {843-863},
      doi = {10.1016/j.asr.2012.06.024},
   adsurl = {http://adsabs.harvard.edu/abs/2012AdSpR..50..843D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2,
   author = {{Decin}, L. and {
}, N.~L.~J. and {Royer}, P. and {Van Marle}, A.~J. and 
	{Vandenbussche}, B. and {Ladjal}, D. and {Kerschbaum}, F. and 
	{Ottensamer}, R. and {Barlow}, M.~J. and {Blommaert}, J.~A.~D.~L. and 
	{Gomez}, H.~L. and {Groenewegen}, M.~A.~T. and {Lim}, T. and 
	{Swinyard}, B.~M. and {Waelkens}, C. and {Tielens}, A.~G.~G.~M.
	},
    title = "{The enigmatic nature of the circumstellar envelope and bow shock surrounding Betelgeuse as revealed by Herschel. I. Evidence of clumps, multiple arcs, and a linear bar-like structure}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1212.4870},
 primaryClass = "astro-ph.SR",
 keywords = {stars: AGB and post-AGB, stars: mass-loss, circumstellar matter, stars: individual: Betelgeuse, methods: numerical, infrared: stars},
     year = 2012,
    month = dec,
   volume = 548,
      eid = {A113},
    pages = {A113},
      doi = {10.1051/0004-6361/201219792},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...548A.113D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dejager_aas_72_1988,
   author = {{de Jager}, C. and {Nieuwenhuijzen}, H. and {van der Hucht}, K.~A.
	},
    title = "{Mass loss rates in the Hertzsprung-Russell diagram}",
  journal = {\aaps},
 keywords = {Hertzsprung-Russell Diagram, O Stars, Planetary Nebulae, Stellar Luminosity, Stellar Mass Ejection, Wolf-Rayet Stars, B Stars, Carbon Stars, Computational Astrophysics, High Temperature, Hot Stars, Stellar Mass},
     year = 1988,
    month = feb,
   volume = 72,
    pages = {259-289},
   adsurl = {http://adsabs.harvard.edu/abs/1988A%26AS...72..259D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{diazmiller_apj_501_1998,
   author = {{Diaz-Miller}, R.~I. and {Franco}, J. and {Shore}, S.~N.},
    title = "{Photoionized and Photodissociated Regions around Main-Sequence Stars}",
  journal = {\apj},
 keywords = {ISM: CLOUDS, ISM: MOLECULES, RADIATIVE TRANSFER, STARS: FORMATION},
     year = 1998,
    month = jul,
   volume = 501,
    pages = {192},
      doi = {10.1086/305793},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...501..192D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{donati_mnras_333_2002,
   author = {{Donati}, J.-F. and {Babel}, J. and {Harries}, T.~J. and {Howarth}, I.~D. and 
	{Petit}, P. and {Semel}, M.},
    title = "{The magnetic field and wind confinement of {\thetas}$^{1}$ Orionis C}",
  journal = {\mnras},
 keywords = {stars: individual: {\thetas}1 Ori C, stars: magnetic fields, stars: rotation, stars: winds, outflows},
     year = 2002,
    month = jun,
   volume = 333,
    pages = {55-70},
      doi = {10.1046/j.1365-8711.2002.05379.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2002MNRAS.333...55D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dgani_apr_461_1996,
   author = {{Dgani}, R. and {van Buren}, D. and {Noriega-Crespo}, A.},
    title = "{The Transverse Acceleration Instability for Bow Shocks in the Nonlinear Regime}",
  journal = {\apj},
 keywords = {HYDRODYNAMICS, INSTABILITIES, SHOCK WAVES, STARS: INDIVIDUAL CONSTELLATION NAME: ALPHA CAMELOPARDALIS, TURBULENCE},
     year = 1996,
    month = apr,
   volume = 461,
    pages = {372},
      doi = {10.1086/177065},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...461..372D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dgani_apj_461_1996,
   author = {{Dgani}, R. and {van Buren}, D. and {Noriega-Crespo}, A.},
    title = "{Stability Analysis of Bow Shocks}",
  journal = {\apj},
 keywords = {SHOCK WAVES, STARS: MASS LOSS},
     year = 1996,
    month = apr,
   volume = 461,
    pages = {927},
      doi = {10.1086/177114},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...461..927D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dopita_aa_29_1973,
   author = {{Dopita}, M.~A.},
    title = "{Photoelectric Photometry of Gaseous Nebulae. I. The Temperature and lonisation Struc- ture of the Orion Nebula}",
  journal = {\aap},
     year = 1973,
    month = dec,
   volume = 29,
    pages = {387},
   adsurl = {http://adsabs.harvard.edu/abs/1973A%26A....29..387D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@BOOK{draine_piim_bool_2011,
   author = {{Draine}, B.~T.},
    title = "{Physics of the Interstellar and Intergalactic Medium}",
booktitle = {Physics of the Interstellar and Intergalactic Medium by Bruce T.~Draine.~Princeton University Press, 2011.~ISBN: 978-0-691-12214-4},
     year = 2011,
   adsurl = {http://adsabs.harvard.edu/abs/2011piim.book.....D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{draine_apj_285_1984,
   author = {{Draine}, B.~T. and {Lee}, H.~M.},
    title = "{Optical properties of interstellar graphite and silicate grains}",
  journal = {\apj},
 keywords = {GRANULAR MATERIALS, GRAPHITE, INTERSTELLAR MATTER, OPTICAL PROPERTIES, SILICATES, ABSORPTION CROSS SECTIONS, INFRARED ASTRONOMY, OPACITY, PARTICLE INTERACTIONS, SCATTERING CROSS SECTIONS},
     year = 1984,
    month = oct,
   volume = 285,
    pages = {89-108},
      doi = {10.1086/162480},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApJ...285...89D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@MISC{dullemond_2012,
   author = {{Dullemond}, C.~P.},
    title = "{RADMC-3D: A multi-purpose radiative transfer tool}",
howpublished = {Astrophysics Source Code Library},
     year = 2012,
    month = feb,
archivePrefix = "ascl",
   eprint = {1202.015},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012ascl.soft02015D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dyson_ass_35_1975,
   author = {{Dyson}, J.~E.},
    title = "{Stellar winds and globules in H II regions}",
  journal = {\apss},
 keywords = {H II REGIONS, PARTICLE INTERACTIONS, SHOCK WAVE PROPAGATION, STELLAR WINDS, ASTRONOMICAL MODELS, GAS FLOW, GLOBULES, STELLAR MASS EJECTION, SUPERSONIC FLOW},
     year = 1975,
    month = jul,
   volume = 35,
    pages = {299-312},
      doi = {10.1007/BF00636999},
   adsurl = {http://adsabs.harvard.edu/abs/1975Ap%26SS..35..299D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dyson_apss_37_1975,
   author = {{Dyson}, J.~E. and {Gulliford}, P.},
    title = "{The dynamical effects of supernovae on the interstellar medium. I - Spherical shock waves in an adiabatic medium}",
  journal = {\apss},
 keywords = {ADIABATIC CONDITIONS, INTERSTELLAR GAS, SHOCK WAVE PROPAGATION, SPHERICAL WAVES, SUPERNOVAE, ASTRONOMICAL MODELS, DYNAMIC MODELS, FINITE DIFFERENCE THEORY, NEBULAE, SHOCK HEATING, STELLAR MASS EJECTION},
     year = 1975,
    month = oct,
   volume = 37,
    pages = {477-498},
      doi = {10.1007/BF00640367},
   adsurl = {http://adsabs.harvard.edu/abs/1975Ap%26SS..37..477D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dwarkadas_apj_630_2005,
   author = {{Dwarkadas}, V.~V.},
    title = "{The Evolution of Supernovae in Circumstellar Wind-Blown Bubbles. I. Introduction and One-Dimensional Calculations}",
  journal = {\apj},
   eprint = {astro-ph/0410464},
 keywords = {Stars: Circumstellar Matter, Hydrodynamics, Shock Waves, ISM: Supernova Remnants, Stars: Supernovae: General, X-Rays: ISM},
     year = 2005,
    month = sep,
   volume = 630,
    pages = {892-910},
      doi = {10.1086/432109},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...630..892D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{dwarkadas_apj_667_2007,
   author = {{Dwarkadas}, V.~V.},
    title = "{The Evolution of Supernovae in Circumstellar Wind Bubbles. II. Case of a Wolf-Rayet Star}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0706.1049},
 keywords = {Hydrodynamics, Instabilities, Shock Waves, Stars: Winds, Outflows, ISM: Supernova Remnants, Stars: Supernovae: General},
     year = 2007,
    month = sep,
   volume = 667,
    pages = {226-247},
      doi = {10.1086/520670},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...667..226D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Dwarkadas_HEDP_2013,
       author = {{Dwarkadas}, V.~V. and {Rosenberg}, D.~L.},
        title = "{Simulated X-ray spectra from ionized wind-blown nebulae around massive stars}",
      journal = {High Energy Density Physics},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = "2013",
        month = "Mar",
       volume = {9},
       number = {1},
        pages = {226-230},
          doi = {10.1016/j.hedp.2012.12.003},
archivePrefix = {arXiv},
       eprint = {1206.1348},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013HEDP....9..226D},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE E 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{ekstroem_aa_537_2012,
   author = {{Ekstr{\"o}m}, S. and {Georgy}, C. and {Eggenberger}, P. and 
	{Meynet}, G. and {Mowlavi}, N. and {Wyttenbach}, A. and {Granada}, A. and 
	{Decressin}, T. and {Hirschi}, R. and {Frischknecht}, U. and 
	{Charbonnel}, C. and {Maeder}, A.},
    title = "{Grids of stellar models with rotation. I. Models from 0.8 to 120 M$_{?}$ at solar metallicity (Z = 0.014)}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1110.5049},
 primaryClass = "astro-ph.SR",
 keywords = {stars: general, stars: evolution, stars: massive, stars: low-mass, stars: rotation},
     year = 2012,
    month = jan,
   volume = 537,
      eid = {A146},
    pages = {A146},
      doi = {10.1051/0004-6361/201117751},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012A%26A...537A.146E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{eldridge_mnras_367_2006,
   author = {{Eldridge}, J.~J. and {Genet}, F. and {Daigne}, F. and {Mochkovitch}, R.
	},
    title = "{The circumstellar environment of Wolf-Rayet stars and gamma-ray burst afterglows}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0509749},
 keywords = {circumstellar matter-stars: evolution-stars: winds, outflows-stars: Wolf-Rayet-gamma-rays: bursts},
     year = 2006,
    month = mar,
   volume = 367,
    pages = {186-200},
      doi = {10.1111/j.1365-2966.2005.09938.x},
   adsurl = {http://adsabs.harvard.edu/abs/2006MNRAS.367..186E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{eldridge_mnras_414_2011,
   author = {{Eldridge}, J.~J. and {Langer}, N. and {Tout}, C.~A.},
    title = "{Runaway stars as progenitors of supernovae and gamma-ray bursts}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1103.1877},
 primaryClass = "astro-ph.SR",
 keywords = {binaries: general, stars: evolution, gamma-ray burst: general, stars: massive, supernovae: general, stars: Wolf-Rayet},
     year = 2011,
    month = jul,
   volume = 414,
    pages = {3501-3520},
      doi = {10.1111/j.1365-2966.2011.18650.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.414.3501E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{evans_iaus_30_1967,
   author = {{Evans}, D.~S.},
    title = "{The Revision of the General Catalogue of Radial Velocities}",
booktitle = {Determination of Radial Velocities and their Applications},
     year = 1967,
   series = {IAU Symposium},
   volume = 30,
   editor = {{Batten}, A.~H. and {Heard}, J.~F.},
    pages = {57},
   adsurl = {http://adsabs.harvard.edu/abs/1967IAUS...30...57E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{everet_apj_713_2010,
   author = {{Everett}, J.~E. and {Churchwell}, E.},
    title = "{Dusty Wind-blown Bubbles}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1003.0838},
 primaryClass = "astro-ph.SR",
 keywords = {dust, extinction, infrared: ISM, ISM: bubbles, stars: individual: N49},
     year = 2010,
    month = apr,
   volume = 713,
    pages = {592-602},
      doi = {10.1088/0004-637X/713/1/592},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...713..592E},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE F 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




@ARTICLE{fendt_apj_692_2009,
       author = {{Fendt}, C.},
        title = "{Formation of Protostellar Jets as Two-Component Outflows from Star-Disk Magnetospheres}",
      journal = {\apj},
     keywords = {accretion, accretion disks, galaxies: jets, ISM: jets and outflows, MHD, stars: mass loss, stars: pre-main sequence, Astrophysics},
         year = 2009,
        month = feb,
       volume = {692},
       number = {1},
        pages = {346-363},
          doi = {10.1088/0004-637X/692/1/346},
archivePrefix = {arXiv},
       eprint = {0810.4154},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ApJ...692..346F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{fendt_apj_774_2013,
       author = {{Fendt}, Christian and {Sheikhnezami}, Somayeh},
        title = "{Bipolar Jets Launched from Accretion Disks. II. The Formation of Asymmetric Jets and Counter Jets}",
      journal = {\apj},
     keywords = {accretion, accretion disks, galaxies: active, galaxies: jets, ISM: jets and outflows, magnetohydrodynamics: MHD, stars: protostars, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = sep,
       volume = {774},
       number = {1},
          eid = {12},
        pages = {12},
          doi = {10.1088/0004-637X/774/1/12},
archivePrefix = {arXiv},
       eprint = {1305.1263},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...774...12F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{falceta_mnras_438_2014,
       author = {{Falceta-Gon{\c{c}}alves}, D. and {Monteiro}, H.},
        title = "{On the alignment of PNe and local magnetic field at the Galactic centre: magnetohydrodynamical numerical simulations}",
      journal = {\mnras},
     keywords = {hydrodynamics, methods: numerical, ISM: magnetic fields, planetary nebulae: general, Galaxy: bulge, Astrophysics - Astrophysics of Galaxies},
         year = 2014,
        month = mar,
       volume = {438},
       number = {4},
        pages = {2853-2863},
          doi = {10.1093/mnras/stt2393},
archivePrefix = {arXiv},
       eprint = {1312.2910},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.438.2853F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{ferrand_apj_789_2014,
       author = {{Ferrand}, Gilles and {Decourchelle}, Anne and {Safi-Harb}, Samar},
        title = "{Three-dimensional Simulations of the Non-thermal Broadband Emission from Young Supernova Remnants Including Efficient Particle Acceleration}",
      journal = {\apj},
     keywords = {acceleration of particles, cosmic rays, ISM: supernova remnants, methods: numerical, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = jul,
       volume = {789},
       number = {1},
          eid = {49},
        pages = {49},
          doi = {10.1088/0004-637X/789/1/49},
archivePrefix = {arXiv},
       eprint = {1405.0614},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...789...49F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{fang_mnras_464_2017,
       author = {{Fang}, Jun and {Yu}, Huan and {Zhang}, Li},
        title = "{Numerically modelling the Cygnus Loop as a remnant evolved in an anisotropic cavity}",
      journal = {\mnras},
     keywords = {hydrodynamics, methods: numerical, ISM: individual objects: Cygnus Loop, ISM: supernova remnants},
         year = "2017",
        month = "Jan",
       volume = {464},
       number = {1},
        pages = {940-945},
          doi = {10.1093/mnras/stw2473},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.464..940F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{freyer_apj_638_2006,
       author = {{Freyer}, Tim and {Hensler}, Gerhard and {Yorke}, Harold W.},
        title = "{Massive Stars and the Energy Balance of the Interstellar Medium. II. The 35 M$_{solar}$ Star and a Solution to the ``Missing Wind Problem''}",
      journal = {\apj},
     keywords = {ISM: H II Regions, Hydrodynamics, ISM: Bubbles, ISM: Individual: Alphanumeric: S308, ISM: Structure, X-rays: Individual: Alphanumeric: S308, Astrophysics},
         year = "2006",
        month = "Feb",
       volume = {638},
       number = {1},
        pages = {262-280},
          doi = {10.1086/498734},
archivePrefix = {arXiv},
       eprint = {astro-ph/0512110},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...638..262F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{freyer_apj_594_2003,
       author = {{Freyer}, Tim and {Hensler}, Gerhard and {Yorke}, Harold W.},
        title = "{Massive Stars and the Energy Balance of the Interstellar Medium. I. The Impact of an Isolated 60 M$_{solar}$ Star}",
      journal = {\apj},
     keywords = {Galaxies: Evolution, ISM: H II Regions, Hydrodynamics, Instabilities- ISM: Bubbles, ISM: Structure, Astrophysics},
         year = "2003",
        month = "Sep",
       volume = {594},
       number = {2},
        pages = {888-910},
          doi = {10.1086/376937},
archivePrefix = {arXiv},
       eprint = {astro-ph/0306541},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...594..888F},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{florinski_apj_604_2004,
   author = {{Florinski}, V. and {Pogorelov}, N.~V. and {Zank}, G.~P. and 
	{Wood}, B.~E. and {Cox}, D.~P.},
    title = "{On the Possibility of a Strong Magnetic Field in the Local Interstellar Medium}",
  journal = {\apj},
 keywords = {ISM: Clouds, ISM: Magnetic Fields, Magnetohydrodynamics: MHD, Shock Waves, Sun: Solar Wind, Ultraviolet: Solar System},
     year = 2004,
    month = apr,
   volume = 604,
    pages = {700-706},
      doi = {10.1086/382017},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...604..700F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{falle_mnras_250_1991,
   author = {{Falle}, S.~A.~E.~G.},
    title = "{Self-similar jets}",
  journal = {\mnras},
 keywords = {EXTRAGALACTIC RADIO SOURCES, GALACTIC STRUCTURE, GAS JETS, RADIO JETS (ASTRONOMY), SUPERSONIC JET FLOW, HYDRODYNAMICS, MATHEMATICAL MODELS},
     year = 1991,
    month = jun,
   volume = 250,
    pages = {581-596},
   adsurl = {http://adsabs.harvard.edu/abs/1991MNRAS.250..581F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{filipovi_mnras_364_2005,
   author = {{Filipovi{\'c}}, M.~D. and {Payne}, J.~L. and {Reid}, W. and 
	{Danforth}, C.~W. and {Staveley-Smith}, L. and {Jones}, P.~A. and 
	{White}, G.~L.},
    title = "{An ATCA radio-continuum study of the Small Magellanic Cloud - III. Supernova remnants and their environments}",
  journal = {\mnras},
 keywords = {H II regions, supernova remnants, Magellanic Clouds},
     year = 2005,
    month = nov,
   volume = 364,
    pages = {217-236},
      doi = {10.1111/j.1365-2966.2005.09554.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.364..217F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{filippenko_araa_35_1997,
   author = {{Filippenko}, A.~V.},
    title = "{Optical Spectra of Supernovae}",
  journal = {\araa},
     year = 1997,
   volume = 35,
    pages = {309-355},
      doi = {10.1146/annurev.astro.35.1.309},
   adsurl = {http://adsabs.harvard.edu/abs/1997ARA%26A..35..309F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fiedler_apj_415_1993,
   author = {{Fiedler}, R.~A. and {Mouschovias}, T.~C.},
    title = "{Ambipolar Diffusion and Star Formation: Formation and Contraction of Axisymmetric Cloud Cores. II. Results}",
  journal = {\apj},
 keywords = {DIFFUSION, ISM: CLOUDS, ISM: MAGNETIC FIELDS, MAGNETOHYDRODYNAMICS: MHD, PLASMAS, STARS: FORMATION},
     year = 1993,
    month = oct,
   volume = 415,
    pages = {680},
      doi = {10.1086/173193},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...415..680F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{fink_aa_476_2007,
   author = {{Fink}, M. and {Hillebrandt}, W. and {R{\"o}pke}, F.~K.},
    title = "{Double-detonation supernovae of sub-Chandrasekhar mass white dwarfs}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0710.5486},
 keywords = {supernovae: general, nuclear reactions, nucleosynthesis, , abundances, hydrodynamics, methods: numerical},
     year = 2007,
    month = dec,
   volume = 476,
    pages = {1133-1143},
      doi = {10.1051/0004-6361:20078438},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...476.1133F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{frail_aj_111_1996,
   author = {{Frail}, D.~A. and {Goss}, W.~M. and {Reynoso}, E.~M. and {Giacani}, E.~B. and 
	{Green}, A.~J. and {Otrupcek}, R.},
    title = "{A Survey for OH (1720 MHz) Maser Emission Toward Supernova Remnants}",
  journal = {\aj},
 keywords = {SUPERNOVA REMNANTS, MASERS, CIRCUMSTELLAR MATTER, ISM: CLOUDS},
     year = 1996,
    month = apr,
   volume = 111,
    pages = {1651},
      doi = {10.1086/117904},
   adsurl = {http://adsabs.harvard.edu/abs/1996AJ....111.1651F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{franco_pasp_103_1991,
   author = {{Franco}, J. and {Tenorio-Tagle}, G. and {Bodenheimer}, P. and 
	{Rozyczka}, M.},
    title = "{Evolution of supernova remnants inside preexisting wind-driven cavities}",
  journal = {\pasp},
 keywords = {CAVITIES, EJECTA, SHOCK WAVES, STELLAR EVOLUTION, STELLAR WINDS, SUPERNOVA REMNANTS, LIGHT EMISSION, STELLAR MASS EJECTION, X RAY SOURCES},
     year = 1991,
    month = aug,
   volume = 103,
    pages = {803-810},
      doi = {10.1086/132884},
   adsurl = {http://adsabs.harvard.edu/abs/1991PASP..103..803F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ferreira_478_aa_2008,
   author = {{Ferreira}, S.~E.~S. and {de Jager}, O.~C.},
    title = "{Supernova remnant evolution in uniform and non-uniform media}",
  journal = {\aap},
 keywords = {stars: supernovae: general, ISM: supernovae remnants, methods: numerical, magnetohydrodynamics (MHD), shock waves, ISM: cosmic rays},
     year = 2008,
    month = jan,
   volume = 478,
    pages = {17-29},
      doi = {10.1051/0004-6361:20077824},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...478...17F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{frick_mnras_325_2001,
   author = {{Frick}, P. and {Stepanov}, R. and {Shukurov}, A. and {Sokoloff}, D.
	},
    title = "{Structures in the rotation measure sky}",
  journal = {\mnras},
   eprint = {astro-ph/0012459},
 keywords = {MAGNETIC FIELDS, POLARIZATION, METHODS: DATA ANALYSIS, ISM: MAGNETIC FIELDS, GALAXY: STRUCTURE},
     year = 2001,
    month = aug,
   volume = 325,
    pages = {649-664},
      doi = {10.1046/j.1365-8711.2001.04462.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.325..649F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{foglizzo_apj_654_2007,
   author = {{Foglizzo}, T. and {Galletti}, P. and {Scheck}, L. and {Janka}, H.-T.
	},
    title = "{Instability of a Stalled Accretion Shock: Evidence for the Advective-Acoustic Cycle}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0606640},
 keywords = {Accretion, Accretion Disks, Hydrodynamics, Instabilities, Shock Waves, Stars: Supernovae: General},
     year = 2007,
    month = jan,
   volume = 654,
    pages = {1006-1021},
      doi = {10.1086/509612},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...654.1006F},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE G 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{gelfand_apj_777_2013,
       author = {{Gelfand}, Joseph D. and {Castro}, Daniel and {Slane}, Patrick O. and {Temim}, Tea and {Hughes}, John P. and {Rakowski}, Cara},
        title = "{Supernova Remnant Kes 17: An Efficient Cosmic Ray Accelerator inside a Molecular Cloud}",
      journal = {\apj},
     keywords = {cosmic rays, gamma rays: ISM, ISM: individual objects: Kes 17, ISM: supernova remnants, X-rays: individual: Kes 17, Astrophysics - Galaxy Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2013,
        month = nov,
       volume = {777},
       number = {2},
          eid = {148},
        pages = {148},
          doi = {10.1088/0004-637X/777/2/148},
archivePrefix = {arXiv},
       eprint = {1311.6894},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013ApJ...777..148G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{Gvaramadze_nature,
       author = {{Gvaramadze}, Vasilii V. and {Langer}, Norbert and {Fossati}, Luca and
         {Bock}, Douglas C. -J. and {Castro}, Norberto and
         {Georgiev}, Iskren Y. and {Greiner}, Jochen and {Johnston}, Simon and
         {Rau}, Arne and {Tauris}, Thomas M.},
        title = "{A solar-type star polluted by calcium-rich supernova ejecta inside the supernova remnant RCW 86}",
      journal = {Nature Astronomy},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = jun,
       volume = {1},
          eid = {0116},
        pages = {0116},
          doi = {10.1038/s41550-017-0116},
archivePrefix = {arXiv},
       eprint = {1702.00936},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017NatAs...1E.116G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2010MNRAS.405.1047G,
       author = {{Gvaramadze}, V.~V. and {Kniazev}, A.~Y. and {Fabrika}, S.},
        title = "{Revealing evolved massive stars with Spitzer}",
      journal = {\mnras},
     keywords = {circumstellar matter, stars: emission-line, Be, stars: individual: HD 326823, stars: individual: HD 269445, stars: Wolf-Rayet, Astrophysics - Solar and Stellar Astrophysics},
         year = 2010,
        month = jun,
       volume = {405},
       number = {2},
        pages = {1047-1060},
          doi = {10.1111/j.1365-2966.2010.16496.x},
archivePrefix = {arXiv},
       eprint = {0909.0458},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.405.1047G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{gvaramadze_aa_454_2006,
       author = {{Gvaramadze}, V.~V.},
        title = "{Supernova remnant S 147 and its associated neutron star(s)}",
      journal = {\aap},
     keywords = {stars: pulsars: individual: PSR J 0538+2817, ISM: bubbles, ISM: individual objects: S 147, ISM: individual objects: G 180.0-1.7, ISM: supernova remnants, stars: binaries: general, Astrophysics},
         year = "2006",
        month = "Jul",
       volume = {454},
       number = {1},
        pages = {239-246},
          doi = {10.1051/0004-6361:20054114},
archivePrefix = {arXiv},
       eprint = {astro-ph/0508595},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006A&A...454..239G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{gonzales_aa_561_2014,
       author = {{Gonz{\'a}lez}, Ricardo F. and {Koenigsberger}, Gloria},
        title = "{Observations of the early stages in the formation of an LBV shell}",
      journal = {\aap},
     keywords = {ISM: general, stars: individual: HD 5980, stars: winds, outflows, stars: variables: general, stars: massive},
         year = "2014",
        month = "Jan",
       volume = {561},
          eid = {A105},
        pages = {A105},
          doi = {10.1051/0004-6361/201322980},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014A&A...561A.105G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{graefener_aa_608_2017,
       author = {{Gr{\"a}fener}, G. and {Owocki}, S.~P. and {Grassitelli}, L. and
         {Langer}, N.},
        title = "{On the optically thick winds of Wolf-Rayet stars}",
      journal = {\aap},
     keywords = {stars: Wolf-Rayet, stars: early-type, stars: atmospheres, stars: mass-loss, stars: winds, outflows, Astrophysics - Solar and Stellar Astrophysics},
         year = "2017",
        month = "Dec",
       volume = {608},
          eid = {A34},
        pages = {A34},
          doi = {10.1051/0004-6361/201731590},
archivePrefix = {arXiv},
       eprint = {1710.04543},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...608A..34G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Grassitelli_aa_614_2018,
       author = {{Grassitelli}, L. and {Langer}, N. and {Grin}, N.~J. and {Mackey}, J. and
         {Bestenlehner}, J.~M. and {Gr{\"a}fener}, G.},
        title = "{Subsonic structure and optically thick winds from Wolf-Rayet stars}",
      journal = {\aap},
     keywords = {hydrodynamics, stars: atmospheres, stars: massive, stars: Wolf-Rayet, stars: winds, outflows, stars: mass-loss, Astrophysics - Solar and Stellar Astrophysics},
         year = "2018",
        month = "Jun",
       volume = {614},
          eid = {A86},
        pages = {A86},
          doi = {10.1051/0004-6361/201731542},
archivePrefix = {arXiv},
       eprint = {1803.03033},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...614A..86G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{groh_aa564_2014,
   author = {{Groh}, J.~H. and {Meynet}, G. and {Ekstr{\"o}m}, S. and {Georgy}, C.
	},
    title = "{The evolution of massive stars and their spectra. I. A non-rotating 60 M$_{⊙}$ star from the zero-age main sequence to the pre-supernova stage}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1401.7322},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, stars: atmospheres, stars: mass-loss, stars: massive, supernovae: general, stars: winds, outflows},
     year = 2014,
    month = apr,
   volume = 564,
      eid = {A30},
    pages = {A30},
      doi = {10.1051/0004-6361/201322573},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014A%26A...564A..30G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gvaramadze_mnras_474_2018,
   author = {{Gvaramadze}, V.~V. and {Alexashov}, D.~B. and {Katushkina}, O.~A. and 
	{Kniazev}, A.~Y.},
    title = "{Modelling interstellar structures around Vela X-1}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1711.09910},
 primaryClass = "astro-ph.SR",
 keywords = {MHD, shock waves, stars: individual: Vela X-1, ISM: bubbles},
     year = 2018,
    month = mar,
   volume = 474,
    pages = {4421-4431},
      doi = {10.1093/mnras/stx3089},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.474.4421G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2019A&A...625A...4G,
       author = {{Green}, Samuel and {Mackey}, Jonathan and {Haworth}, Thomas J. and
         {Gvaramadze}, Vasilii V. and {Duffy}, Peter},
        title = "{Thermal emission from bow shocks. I. 2D hydrodynamic models of the Bubble Nebula}",
      journal = {\aap},
     keywords = {hydrodynamics, instabilities, radiative transfer, methods: numerical, stars: winds, outflows, ISM: bubbles, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "May",
       volume = {625},
          eid = {A4},
        pages = {A4},
          doi = {10.1051/0004-6361/201834832},
archivePrefix = {arXiv},
       eprint = {1903.05505},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019A&A...625A...4G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{gaspar_apj_672_2008,
   author = {{G{\'a}sp{\'a}r}, A. and {Su}, K.~Y.~L. and {Rieke}, G.~H. and 
	{Balog}, Z. and {Kamp}, I. and {Mart{\'{\i}}nez-Galarza}, J.~R. and 
	{Stapelfeldt}, K.},
    title = "{Modeling the Infrared Bow Shock at {$\delta$} Velorum: Implications for Studies of Debris Disks and {$\lambda$} Bo{\"o}tis Stars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0709.4247},
 keywords = {infrared: ISM, ISM: kinematics and dynamics, radiation mechanisms: thermal, stars: evolution, stars: imaging, stars: individual: HD 74956 {$\delta$} Velorum, shock waves},
     year = 2008,
    month = jan,
   volume = 672,
      eid = {974-983},
    pages = {974-983},
      doi = {10.1086/523299},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2008ApJ...672..974G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@PHDTHESIS{gaensler_phd_1999,
   author = {{Gaensler}, B.~M.},
    title = "{Barrels, jets and smoke-rings: Understanding the bizarre shapes of radio supernova remnants}",
   school = {University of Sydney},
     year = 1999,
    month = May,
   adsurl = {http://adsabs.harvard.edu/abs/1999PhDT..........G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gaetz_apjs_155_1983,
   author = {{Gaetz}, T.~J. and {Salpeter}, E.~E.},
    title = "{Line radiation from a hot, optically thin plasma - Collision strengths and emissivities}",
  journal = {\apjs},
 keywords = {COLLISION RATES, EMISSIVITY, HIGH TEMPERATURE PLASMAS, LINE SPECTRA, PLASMA RADIATION, SOLAR CORONA, SUPERNOVA REMNANTS, ATOMIC COLLISIONS, COSMIC PLASMA, ELECTRON TRANSITIONS, FINE STRUCTURE, OPTICAL THICKNESS, TABLES (DATA), TEMPERATURE DEPENDENCE},
     year = 1983,
    month = jun,
   volume = 52,
    pages = {155-168},
      doi = {10.1086/190862},
   adsurl = {http://adsabs.harvard.edu/abs/1983ApJS...52..155G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gaensler_apj_580_2002,
   author = {{Gaensler}, B.~M. and {Jones}, D.~H. and {Stappers}, B.~W.},
    title = "{An Optical Bow Shock around the Nearby Millisecond Pulsar J2124-3358}",
  journal = {\apjl},
   eprint = {astro-ph/0210543},
 keywords = {ISM: General, Stars: Pulsars: Individual: Alphanumeric: PSR J2124-3358, Stars: Neutron, Stars: Winds, Outflows},
     year = 2002,
    month = dec,
   volume = 580,
    pages = {L137-L141},
      doi = {10.1086/345750},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2002ApJ...580L.137G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gaensler_apj_493_1998,
   author = {{Gaensler}, B.~M.},
    title = "{The Nature of Bilateral Supernova Remnants}",
  journal = {\apj},
   eprint = {astro-ph/9707149},
 keywords = {ISM: STRUCTURE, ISM: INDIVIDUAL ALPHANUMERIC: G003.7-00.2, ISM: INDIVIDUAL ALPHANUMERIC: G350.0-02.0, ISM: MAGNETIC FIELDS, ISM: SUPERNOVA REMNANTS, RADIO CONTINUUM: ISM, ISM: Individual: Alphanumeric: G003.7-00.2, ISM: Individual: Alphanumeric: G350.0-02.0, ISM: Magnetic Fields, ISM: Structure, Radio Continuum: ISM, ISM: Supernova Remnants},
     year = 1998,
    month = jan,
   volume = 493,
    pages = {781-792},
      doi = {10.1086/305146},
   adsurl = {http://adsabs.harvard.edu/abs/1998ApJ...493..781G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garciasegura_1996_aa_316ff,
   author = {{Garcia-Segura}, G. and {Langer}, N. and {Mac Low}, M.-M.},
    title = "{The hydrodynamic evolution of circumstellar gas around massive stars. II. The impact of the time sequence O star -{\gt} RSG -{\gt} WR star.}",
  journal = {\aap},
 keywords = {HYDRODYNAMICS, STARS: MASS LOSS, ISM: BUBBLES, STARS: WOLF-RAYET, SUPERGIANTS, STARS: EVOLUTION},
     year = 1996,
    month = dec,
   volume = 316,
    pages = {133-146},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26A...316..133G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garciasegura_1996_aa_305f,
   author = {{Garcia-Segura}, G. and {Mac Low}, M.-M. and {Langer}, N.},
    title = "{The dynamical evolution of circumstellar gas around massive stars. I. The impact of the time sequence Ostar -{\gt} LBV -{\gt} WR star.}",
  journal = {\aap},
 keywords = {HYDRODYNAMICS, STARS: EVOLUTION, MASS LOSS, STARS: WOLF-RAYET, ISM: BUBBLES, ISM: INDIVIDUAL (RCW 58)},
     year = 1996,
    month = jan,
   volume = 305,
    pages = {229},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26A...305..229G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garciasegura_apj_517_1999,
   author = {{Garc{\'{\i}}a-Segura}, G. and {Langer}, N. and {R{\'o}{\.z}yczka}, M. and 
	{Franco}, J.},
    title = "{Shaping Bipolar and Elliptical Planetary Nebulae: Effects of Stellar Rotation, Photoionization Heating, and Magnetic Fields}",
  journal = {\apj},
 keywords = {ISM: MAGNETIC FIELDS, ISM: STRUCTURE, MAGNETOHYDRODYNAMICS: MHD, ISM: PLANETARY NEBULAE: GENERAL, STARS: AGB AND POST-AGB, STARS: MASS LOSS},
     year = 1999,
    month = jun,
   volume = 517,
    pages = {767-781},
      doi = {10.1086/307205},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...517..767G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garciasegura_aa_455_1995a,
   author = {{Garcia-Segura}, G. and {Mac Low}, M.-M.},
    title = "{Wolf-Rayet Bubbles. I. Analytic Solutions}",
  journal = {\apj},
 keywords = {ISM: BUBBLES, ISM: INDIVIDUAL NGC NUMBER: NGC 6888, ISM: STRUCTURE, STARS: MASS LOSS, STARS: WOLF-RAYET},
     year = 1995,
    month = dec,
   volume = 455,
    pages = {145},
      doi = {10.1086/176563},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...455..145G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garciasegura_aa_455_1995b,
   author = {{Garcia-Segura}, G. and {Mac Low}, M.-M.},
    title = "{Wolf-Rayet Bubbles. II. Gasdynamical Simulations}",
  journal = {\apj},
 keywords = {HYDRODYNAMICS, ISM: BUBBLES, STARS: MASS LOSS, STARS: WOLF-RAYET},
     year = 1995,
    month = dec,
   volume = 455,
    pages = {160},
      doi = {10.1086/176564},
   adsurl = {http://adsabs.harvard.edu/abs/1995ApJ...455..160G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{garmany_apj_242_1980,
   author = {{Garmany}, C.~D. and {Conti}, P.~S. and {Massey}, P.},
    title = "{Spectroscopic studies of O type stars. IX - Binary frequency}",
  journal = {\apj},
 keywords = {ASTRONOMICAL SPECTROSCOPY, BINARY STARS, EARLY STARS, O STARS, X RAY SOURCES, MASS RATIOS, STELLAR LUMINOSITY, STELLAR MOTIONS, TABLES (DATA)},
     year = 1980,
    month = dec,
   volume = 242,
    pages = {1063-1076},
      doi = {10.1086/158537},
   adsurl = {http://adsabs.harvard.edu/abs/1980ApJ...242.1063G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gies_apjs_64_1987,
   author = {{Gies}, D.~R.},
    title = "{The kinematical and binary properties of association and field O stars}",
  journal = {\apjs},
 keywords = {ASTRONOMICAL CATALOGS, BINARY STARS, MILKY WAY GALAXY, O STARS, STELLAR MOTIONS, VELOCITY DISTRIBUTION, EARLY STARS, GRAVITATIONAL EFFECTS, RADIAL VELOCITY, STAR CLUSTERS, STELLAR GRAVITATION},
     year = 1987,
    month = jul,
   volume = 64,
    pages = {545-563},
      doi = {10.1086/191208},
   adsurl = {http://adsabs.harvard.edu/abs/1987ApJS...64..545G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{golub_1997,
   author = {{Golub}, L. and {Pasachoff}, J.~M.},
    title = "{The Solar Corona, Cambridge University Press}",
booktitle = {The Solar Corona, by Leon Golub and Jay M.~Pasachoff, pp.~388.~ISBN 0521480825.~Cambridge, UK: Cambridge University Press, September 1997.},
     year = 1997,
    month = sep,
   adsurl = {http://adsabs.harvard.edu/abs/1997soco.book.....G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{giuliani_apj_277_1984,
   author = {{Giuliani}, Jr., J.~L.},
    title = "{On the dynamics in evaporating cloud envelopes}",
  journal = {\apj},
 keywords = {ASTROPHYSICS, CLOUDS, HYDRODYNAMICS, INTERSTELLAR GAS, HYDRODYNAMIC EQUATIONS, INVISCID FLOW, SHOCK WAVES, VISCOUS FLOW},
     year = 1984,
    month = feb,
   volume = 277,
    pages = {605-614},
      doi = {10.1086/161731},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApJ...277..605G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{graham_apj_179_1973,
   author = {{Graham}, R. and {Langer}, W.~D.},
    title = "{Pressure Equilibrium of Finite-Size Clouds in the Interstellar Medium}",
  journal = {\apj},
     year = 1973,
    month = jan,
   volume = 179,
    pages = {469-482},
      doi = {10.1086/151887},
   adsurl = {http://adsabs.harvard.edu/abs/1973ApJ...179..469G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{green_lnp_598_2003,
   author = {{Green}, D.~A. and {Stephenson}, F.~R.},
    title = "{Historical Supernovae}",
booktitle = {Supernovae and Gamma-Ray Bursters},
     year = 2003,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 598,
   eprint = {astro-ph/0301603},
   editor = {{Weiler}, K.},
    pages = {7-19},
   adsurl = {http://adsabs.harvard.edu/abs/2003LNP...598....7G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{green_cat_2009,
   author = {{Green}, D.~A.},
    title = "{A Catalogue of Galactic Supernova Remnants (Green, 2009)}",
  journal = {VizieR Online Data Catalog},
 keywords = {Supernova remnants, Milky Way, Nonstellar objects},
     year = 2009,
    month = jun,
   volume = 7253,
    pages = {0},
   adsurl = {http://adsabs.harvard.edu/abs/2009yCat.7253....0G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{grunhut_mnras_400_2009,
   author = {{Grunhut}, J.~H. and {Wade}, G.~A. and {Marcolino}, W.~L.~F. and 
	{Petit}, V. and {Henrichs}, H.~F. and {Cohen}, D.~H. and {Alecian}, E. and 
	{Bohlender}, D. and {Bouret}, J.-C. and {Kochukhov}, O. and 
	{Neiner}, C. and {St-Louis}, N. and {Townsend}, R.~H.~D.},
    title = "{Discovery of a magnetic field in the O9 sub-giant star HD 57682 by the MiMeS Collaboration}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0910.0214},
 primaryClass = "astro-ph.SR",
 keywords = {stars: early-type , stars: individual: HD 57682 , stars: magnetic fields , stars: rotation , stars: winds, outflows},
     year = 2009,
    month = nov,
   volume = 400,
    pages = {L94-L98},
      doi = {10.1111/j.1745-3933.2009.00771.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.400L..94G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gotthelf_apj_552_2001,
   author = {{Gotthelf}, E.~V. and {Koralesky}, B. and {Rudnick}, L. and 
	{Jones}, T.~W. and {Hwang}, U. and {Petre}, R.},
    title = "{Chandra Detection of the Forward and Reverse Shocks in Cassiopeia A}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/0104161},
 keywords = {ISM: Supernova Remnants, Stars: Supernovae: Individual: Name: Cassiopeia A, X-Rays: General},
     year = 2001,
    month = may,
   volume = 552,
    pages = {L39-L43},
      doi = {10.1086/320250},
   adsurl = {http://adsabs.harvard.edu/abs/2001ApJ...552L..39G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{guarcello_aa_521_2010,
   author = {{Guarcello}, M.~G. and {Micela}, G. and {Peres}, G. and {Prisinzano}, L. and 
	{Sciortino}, S.},
    title = "{Chronology of star formation and disk evolution in the Eagle Nebula}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1008.0422},
 primaryClass = "astro-ph.SR",
 keywords = {protoplanetary disks, stars: formation, stars: pre-main sequence, infrared: stars: X-rays: stars},
     year = 2010,
    month = oct,
   volume = 521,
      eid = {A61},
    pages = {A61},
      doi = {10.1051/0004-6361/201014351},
   adsurl = {http://adsabs.harvard.edu/abs/2010A%26A...521A..61G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gonzalezcasanova_apj_781_2014,
   author = {{Gonz{\'a}lez-Casanova}, D.~F. and {De Colle}, F. and {Ramirez-Ruiz}, E. and 
	{Lopez}, L.~A.},
    title = "{The Morphology and Dynamics of Jet-driven Supernova Remnants: The Case of W49B}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1309.7049},
 primaryClass = "astro-ph.HE",
 keywords = {hydrodynamics, ISM: individual objects: W49B G43.3{\ndash}0.2, ISM: supernova remnants, methods: numerical, nuclear reactions, nucleosynthesis, abundances},
     year = 2014,
    month = feb,
   volume = 781,
      eid = {L26},
    pages = {L26},
      doi = {10.1088/2041-8205/781/2/L26},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...781L..26G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gull_apj_230_1979,
   author = {{Gull}, T.~R. and {Sofia}, S.},
    title = "{Discovery of two distorted interstellar bubbles}",
  journal = {\apj},
 keywords = {INTERSTELLAR GAS, NEBULAE, ORION NEBULA, ASTRONOMICAL SPECTROSCOPY, GALACTIC STRUCTURE, STELLAR LUMINOSITY, STELLAR MASS EJECTION},
     year = 1979,
    month = jun,
   volume = 230,
    pages = {782-785},
      doi = {10.1086/157137},
   adsurl = {http://adsabs.harvard.edu/abs/1979ApJ...230..782G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{gusdorf_iaus_296_2014,
   author = {{Gusdorf}, A. and {G{\"u}sten}, R. and {Anderl}, S. and {Hezareh}, T. and 
	{Wiesemeyer}, H.},
    title = "{The molecular emission from old supernova remnants}",
 keywords = {ISM: supernova remnants, Shock waves, Submillimeter: ISM, ISM: individual objects: W28, IC443 {\amp} 3C391, Stars: formation, cosmic rays,},
booktitle = {IAU Symposium},
     year = 2014,
   series = {IAU Symposium},
   volume = 296,
archivePrefix = "arXiv",
   eprint = {1403.5909},
   editor = {{Ray}, A. and {McCray}, R.~A.},
    month = jan,
    pages = {178-182},
      doi = {10.1017/S1743921313009435},
   adsurl = {http://adsabs.harvard.edu/abs/2014IAUS..296..178G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gvaramadze_mnras_427_2012,
   author = {{Gvaramadze}, V.~V. and {Langer}, N. and {Mackey}, J.},
    title = "{{$\zeta$} Oph and the weak-wind problem}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1209.0455},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, stars: individual: {$\zeta$} Oph, stars: mass-loss, stars: winds, outflows, H II regions},
     year = 2012,
    month = nov,
   volume = 427,
    pages = {L50-L54},
      doi = {10.1111/j.1745-3933.2012.01343.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012MNRAS.427L..50G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gvaramadze_424_mnras_2012,
   author = {{Gvaramadze}, V.~V. and {Weidner}, C. and {Kroupa}, P. and {Pflamm-Altenburg}, J.
	},
    title = "{Field O stars: formed in situ or as runaways?}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1206.1596},
 primaryClass = "astro-ph.SR",
 keywords = {stars: early-type, stars: formation, stars: kinematics and dynamics, stars: massive, Magellanic Clouds, galaxies: star formation },
     year = 2012,
    month = aug,
   volume = 424,
    pages = {3037-3049},
      doi = {10.1111/j.1365-2966.2012.21452.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.424.3037G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{gvaramadze_aa_490_2008,
   author = {{Gvaramadze}, V.~V. and {Bomans}, D.~J.},
    title = "{Search for OB stars running away from young star clusters. I. NGC 6611}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0809.0650},
 keywords = {stars: individual: BD-14{\deg} 5040, stars: individual: HD 165319, open clusters and associations: general, open clusters and associations: individual: NGC 6611, ISM: individual objects: RCW 158},
     year = 2008,
    month = nov,
   volume = 490,
    pages = {1071-1077},
      doi = {10.1051/0004-6361:200810411},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...490.1071G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gvaramadze_aa_535_2011,
   author = {{Gvaramadze}, V.~V. and {Kniazev}, A.~Y. and {Kroupa}, P. and 
	{Oh}, S.},
    title = "{Search for OB stars running away from young star clusters. II. The NGC 6357 star-forming region}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1109.2116},
 primaryClass = "astro-ph.SR",
 keywords = {stars: kinematics and dynamics, stars: massive, open clusters and associations: general, open clusters and associations: individual: AH03 J1725-34.4, ISM: individual objects: NGC 6357},
     year = 2011,
    month = nov,
   volume = 535,
      eid = {A29},
    pages = {A29},
      doi = {10.1051/0004-6361/201117746},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...535A..29G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gvaramadze_mnras_410_2011,
   author = {{Gvaramadze}, V.~V. and {Gualandris}, A.},
    title = "{Very massive runaway stars from three-body encounters}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1007.5057},
 primaryClass = "astro-ph.SR",
 keywords = {methods: numerical, binaries: general, stars: individual: {$\lambda$} Cep, BD+43{\deg}3654, Sk -67{\deg}22, BI 237, 30 Dor 016, HD269928, stars: kinematics and dynamics, galaxies: star clusters: individual: 30 Doradus},
     year = 2011,
    month = jan,
   volume = 410,
    pages = {304-312},
      doi = {10.1111/j.1365-2966.2010.17446.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.410..304G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gvaramadze_aa_529_2011,
   author = {{Gvaramadze}, V.~V. and {R{\"o}ser}, S. and {Scholz}, R.-D. and 
	{Schilbach}, E.},
    title = "{4U 1907+09: an HMXB running away from the Galactic plane}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1102.2437},
 primaryClass = "astro-ph.SR",
 keywords = {proper motions, stars: early-type, stars: kinematics and dynamics, stars: individual: 4U 1907+09, stars: individual: Vela X-1, X-rays: binaries},
     year = 2011,
    month = may,
   volume = 529,
      eid = {A14},
    pages = {A14},
      doi = {10.1051/0004-6361/201016256},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...529A..14G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gvaramadze_mnras_427_2012,
   author = {{Gvaramadze}, V.~V. and {Langer}, N. and {Mackey}, J.},
    title = "{{$\zeta$} Oph and the weak-wind problem}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1209.0455},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, stars: individual: {$\zeta$} Oph, stars: mass-loss, stars: winds, outflows, H II regions},
     year = 2012,
    month = nov,
   volume = 427,
    pages = {L50-L54},
      doi = {10.1111/j.1745-3933.2012.01343.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.427L..50G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Gvaramadze_2013,
   author = {{Gvaramadze}, V.~V. and {Menten}, K.~M. and {Kniazev}, A.~Y. and 
	{Langer}, N. and {Mackey}, J. and {Kraus}, A. and {Meyer}, D.~M.-A. and 
	{Kami{\'n}ski}, T.},
    title = "{IRC -10414: a bow-shock-producing red supergiant star}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1310.2245},
 primaryClass = "astro-ph.SR",
 keywords = {masers, shock waves, circumstellar matter, stars: individual: IRC -10414, stars: kinematics and dynamics, stars: massive},
     year = 2014,
    month = jan,
   volume = 437,
    pages = {843-856},
      doi = {10.1093/mnras/stt1943},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.437..843G},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{gvaramadze_mnras_405_2010,
       author = {{Gvaramadze}, V.~V. and {Kniazev}, A.~Y. and {Fabrika}, S.},
        title = "{Revealing evolved massive stars with Spitzer}",
      journal = {\mnras},
     keywords = {circumstellar matter, stars: emission-line, Be, stars: individual: HD 326823, stars: individual: HD 269445, stars: Wolf-Rayet, Astrophysics - Solar and Stellar Astrophysics},
         year = "2010",
        month = "Jun",
       volume = {405},
       number = {2},
        pages = {1047-1060},
          doi = {10.1111/j.1365-2966.2010.16496.x},
archivePrefix = {arXiv},
       eprint = {0909.0458},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.405.1047G},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE H 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



@ARTICLE{hess_2018AA_612A_8H,
       author = {{H.~E.~S.~S. Collaboration}},
        title = "{A search for new supernova remnant shells in the Galactic plane with H.E.S.S.}",
      journal = {\aap},
     keywords = {astroparticle physics, ISM: supernova remnants, cosmic rays, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = apr,
       volume = {612},
          eid = {A8},
        pages = {A8},
          doi = {10.1051/0004-6361/201730737},
archivePrefix = {arXiv},
       eprint = {1801.06020},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018A&A...612A...8H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{halpern_apj_882_2019,
       author = {{Halpern}, J.~P. and {Gotthelf}, E.~V.},
        title = "{No Pulsar Wind Nebula in the Southern Blowout Region of the Cygnus Loop}",
      journal = {\apj},
     keywords = {ISM: individual objects: Cygnus Loop, pulsars: general},
         year = 2019,
        month = sep,
       volume = {882},
       number = {2},
          eid = {155},
        pages = {155},
          doi = {10.3847/1538-4357/ab3809},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019ApJ...882..155H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Hillebrandt_nature_327_1987,
       author = {{Hillebrandt}, W. and {Hoeflich}, P. and {Weiss}, A. and {Truran}, J.~W.},
        title = "{Explosion of a blue supergiant: a model for supernova SN1987A}",
      journal = {\nat},
     keywords = {Blue Stars, Stellar Models, Supergiant Stars, Supernova 1987a, Magellanic Clouds, Spectrum Analysis, Stellar Evolution, Stellar Magnitude, Stellar Temperature, Astrophysics},
         year = 1987,
        month = jun,
       volume = {327},
       number = {6123},
        pages = {597-600},
          doi = {10.1038/327597a0},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1987Natur.327..597H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Hamann2006,
       author = {{Hamann}, W. -R. and {Gr{\"a}fener}, G. and {Liermann}, A.},
        title = "{The Galactic WN stars. Spectral analyses with line-blanketed model atmospheres versus stellar evolution models with and without rotation}",
      journal = {\aap},
     keywords = {stars: mass-loss, stars: winds, outflows, stars: Wolf-Rayet, stars: atmospheres, stars: early-type, stars: evolution, Astrophysics},
         year = 2006,
        month = oct,
       volume = {457},
       number = {3},
        pages = {1015-1031},
          doi = {10.1051/0004-6361:20065052},
archivePrefix = {arXiv},
       eprint = {astro-ph/0608078},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006A&A...457.1015H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{humphreys_apj_844_2017,
       author = {{Humphreys}, Roberta M. and {Davidson}, Kris and {Hahn}, David and
         {Martin}, John C. and {Weis}, Kerstin},
        title = "{Luminous and Variable Stars in M31 and M33. V. The Upper HR Diagram}",
      journal = {\apj},
     keywords = {galaxies: individual: M31, M33, stars: massive, supergiants, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2017",
        month = "Jul",
       volume = {844},
       number = {1},
          eid = {40},
        pages = {40},
          doi = {10.3847/1538-4357/aa7cef},
archivePrefix = {arXiv},
       eprint = {1707.01916},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017ApJ...844...40H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{haikala_aa_431_2005,
   author = {{Haikala}, L.~K. and {Harju}, J. and {Mattila}, K. and {Toriseva}, M.
	},
    title = "{Clumpy filaments of the Chamaeleon I cloud: C$^{18}$O mapping with the SEST}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0407608},
 keywords = {ISM: clouds, ISM: molecules, ISM: structure, ISM: individual objects: Chamaeleon I},
     year = 2005,
    month = feb,
   volume = 431,
    pages = {149-163},
      doi = {10.1051/0004-6361:200400057},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...431..149H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{hll_ref,
author = {Amiram Harten and Peter D. Lax and Bram van Leer},
title = {On Upstream Differencing and Godunov-Type Schemes for Hyperbolic Conservation Laws},
journal = {SIAM Review},
volume = {25},
number = {1},
pages = {35-61},
year = {1983},
doi = {10.1137/1025002},
URL = {         http://dx.doi.org/10.1137/1025002    },
eprint = {         http://dx.doi.org/10.1137/1025002   }
}

@ARTICLE{harvey_apj_736_2011,
   author = {{Harvey-Smith}, L. and {Madsen}, G.~J. and {Gaensler}, B.~M.
	},
    title = "{Magnetic Fields in Large-diameter H II Regions Revealed by the Faraday Rotation of Compact Extragalactic Radio Sources}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1106.0931},
 keywords = {H II regions, ISM: magnetic fields, polarization, radio continuum: ISM},
     year = 2011,
    month = aug,
   volume = 736,
      eid = {83},
    pages = {83},
      doi = {10.1088/0004-637X/736/2/83},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...736...83H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{harvey_apj_712_2010,
       author = {{Harvey-Smith}, L. and {Gaensler}, B.~M. and {Kothes}, R. and
         {Townsend}, R. and {Heald}, G.~H. and {Ng}, C. -Y. and {Green}, A.~J.},
        title = "{Faraday Rotation of the Supernova Remnant G296.5+10.0: Evidence for a Magnetized Progenitor Wind}",
      journal = {\apj},
     keywords = {ISM: individual objects: G296.5+10.0, ISM: supernova remnants, magnetic fields, polarization, radio continuum: ISM, stars: winds, outflows, Astrophysics - Astrophysics of Galaxies},
         year = "2010",
        month = "Apr",
       volume = {712},
       number = {2},
        pages = {1157-1165},
          doi = {10.1088/0004-637X/712/2/1157},
archivePrefix = {arXiv},
       eprint = {1001.3462},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...712.1157H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{heger_apj_apj_2000,
   author = {{Heger}, A. and {Langer}, N. and {Woosley}, S.~E.},
    title = "{Presupernova Evolution of Rotating Massive Stars. I. Numerical Method and Evolution of the Internal Stellar Structure}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9904132},
 keywords = {HYDRODYNAMICS, METHODS: NUMERICAL, STARS EARLY-TYPE, STARS: EVOLUTION, STARS: INTERIORS, STARS ROTATION},
     year = 2000,
    month = jan,
   volume = 528,
    pages = {368-396},
      doi = {10.1086/308158},
   adsurl = {http://adsabs.harvard.edu/abs/2000ApJ...528..368H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{heitsch_apj_665_2007,
   author = {{Heitsch}, F. and {Slyz}, A.~D. and {Devriendt}, J.~E.~G. and 
	{Hartmann}, L.~W. and {Burkert}, A.},
    title = "{Magnetized Nonlinear Thin-Shell Instability: Numerical Studies in Two Dimensions}",
  journal = {\apj},
   eprint = {astro-ph/0610949},
 keywords = {Instabilities, ISM: Clouds, ISM: Magnetic Fields, Methods: Numerical, Magnetohydrodynamics: MHD, Turbulence},
     year = 2007,
    month = aug,
   volume = 665,
    pages = {445-456},
      doi = {10.1086/519513},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...665..445H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{henyey_apj_93_1941,
   author = {{Henyey}, L.~G. and {Greenstein}, J.~L.},
    title = "{Diffuse radiation in the Galaxy}",
  journal = {\apj},
     year = 1941,
    month = jan,
   volume = 93,
    pages = {70-83},
      doi = {10.1086/144246},
   adsurl = {http://adsabs.harvard.edu/abs/1941ApJ....93...70H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{henney_2019_arXiv190400343H,
       author = {{Henney}, William J. and {Arthur}, S.~J.},
        title = "{Bow shocks, bow waves, and dust waves. III. Diagnostics}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Mar",
          eid = {arXiv:1904.00343},
        pages = {arXiv:1904.00343},
archivePrefix = {arXiv},
       eprint = {1904.00343},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190400343H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{henney_486_mnras_2019,
       author = {{Henney}, William J. and {Arthur}, S.~J.},
        title = "{Bow shocks, bow waves, and dust waves - II. Beyond the rip point}",
      journal = {\mnras},
     keywords = {radiation: dynamics, circumstellar matter, stars: winds, outflows, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Jul",
       volume = {486},
       number = {3},
        pages = {4423-4442},
          doi = {10.1093/mnras/stz1130},
archivePrefix = {arXiv},
       eprint = {1903.07774},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.486.4423H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{henney_mnras_486_2019,
       author = {{Henney}, William J. and {Arthur}, S.~J.},
        title = "{Bow shocks, bow waves, and dust waves - I. Strong coupling limit}",
      journal = {\mnras},
     keywords = {circumstellar matter, stars: winds, outflows, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2019",
        month = "Jul",
       volume = {486},
       number = {3},
        pages = {3423-3433},
          doi = {10.1093/mnras/stz1043},
archivePrefix = {arXiv},
       eprint = {1903.03737},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019MNRAS.486.3423H},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{henney_mnras_398_2009,
   author = {{Henney}, W.~J. and {Arthur}, S.~J. and {de Colle}, F. and {Mellema}, G.
	},
    title = "{Radiation-magnetohydrodynamic simulations of the photoionization of magnetized globules}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0810.1531},
 keywords = {MHD , stars: formation , ISM: globules , HII regions},
     year = 2009,
    month = sep,
   volume = 398,
    pages = {157-175},
      doi = {10.1111/j.1365-2966.2009.15153.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.398..157H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hibbs_360_mnras_2005,
   author = {{Hobbs}, G. and {Lorimer}, D.~R. and {Lyne}, A.~G. and {Kramer}, M.
	},
    title = "{A statistical study of 233 pulsar proper motions}",
  journal = {\mnras},
   eprint = {astro-ph/0504584},
 keywords = {stars: kinematics, pulsars: general},
     year = 2005,
    month = jul,
   volume = 360,
    pages = {974-992},
      doi = {10.1111/j.1365-2966.2005.09087.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.360..974H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hollenbach_apj_342_1989,
   author = {{Hollenbach}, D. and {McKee}, C.~F.},
    title = "{Molecule formation and infrared emission in fast interstellar shocks. III - Results for J shocks in molecular clouds}",
  journal = {\apj},
 keywords = {EMISSION SPECTRA, INFRARED SOURCES (ASTRONOMY), INTERSTELLAR CHEMISTRY, MOLECULAR CLOUDS, SHOCK FRONTS, COSMIC RAYS, FINE STRUCTURE, HERBIG-HARO OBJECTS, MOLECULAR GASES, SUPERNOVA REMNANTS, WATER MASERS},
     year = 1989,
    month = jul,
   volume = 342,
    pages = {306-336},
      doi = {10.1086/167595},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...342..306H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hummer_mnras_268_1994,
   author = {{Hummer}, D.~G.},
    title = "{Total Recombination and Energy Loss Coefficients for Hydrogenic Ions at Low Density for 10{\lt}T/E/Z/2{\lt}10/7K}",
  journal = {\mnras},
 keywords = {atomic data},
     year = 1994,
    month = may,
   volume = 268,
    pages = {109},
   adsurl = {http://adsabs.harvard.edu/abs/1994MNRAS.268..109H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{huthoff_aa_383_2002,
   author = {{Huthoff}, F. and {Kaper}, L.},
    title = "{On the absence of wind bow-shocks around OB-runaway stars: Probing the physical conditions of the interstellar medium}",
  journal = {\aap},
   eprint = {astro-ph/0112428},
 keywords = {STARS: EARLY-TYPE, STARS: KINEMATICS, STARS: MASS LOSS, ISM: BUBBLES, ISM: STRUCTURE -$\backslash$ X-RAYS: BINARIES},
     year = 2002,
    month = mar,
   volume = 383,
    pages = {999-1010},
      doi = {10.1051/0004-6361:20011793},
   adsurl = {http://adsabs.harvard.edu/abs/2002A%26A...383..999H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{neilson_apj_684_2008,
   author = {{Neilson}, H.~R. and {Lester}, J.~B.},
    title = "{On the Enhancement of Mass Loss in Cepheids Due to Radial Pulsation}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0803.4198},
 keywords = {Stars: Variables: Cepheids, Stars: Circumstellar Matter, Stars: Mass Loss},
     year = 2008,
    month = sep,
   volume = 684,
    pages = {569-587},
      doi = {10.1086/588650},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...684..569N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{neilson_apj_690_2009,
   author = {{Neilson}, H.~R. and {Lester}, J.~B.},
    title = "{On the Enhancement of Mass Loss in Cepheids due to Radial Pulsation. II. The Effect of Metallicity}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0809.2793},
 keywords = {Cepheids, circumstellar matter, Magellanic Clouds, stars: mass loss},
     year = 2009,
    month = jan,
   volume = 690,
    pages = {1829-1838},
      doi = {10.1088/0004-637X/690/2/1829},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...690.1829N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hollenbach_apj_208_1976,
   author = {{Hollenbach}, D. and {Chu}, S.-I. and {McCray}, R.},
    title = "{H2 in expanding circumstellar shells}",
  journal = {\apj},
 keywords = {EARLY STARS, HYDROGEN, MOLECULAR GASES, STELLAR ENVELOPES, GAS DENSITY, MOLECULAR EXCITATION, MOLECULAR ROTATION, STELLAR MODELS, STELLAR WINDS},
     year = 1976,
    month = sep,
   volume = 208,
    pages = {458-467},
      doi = {10.1086/154627},
   adsurl = {http://adsabs.harvard.edu/abs/1976ApJ...208..458H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{heiligman_mnras_191_1980,
   author = {{Heiligman}, G.~M.},
    title = "{Planetary nebulae and the interstellar magnetic field}",
  journal = {\mnras},
 keywords = {Interstellar Magnetic Fields, Magnetohydrodynamics, Planetary Nebulae, Cold Plasmas, Pressure Effects, Thermal Instability},
     year = 1980,
    month = jun,
   volume = 191,
    pages = {761-766},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1980MNRAS.191..761H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{heger_apj_626_2005,
   author = {{Heger}, A. and {Woosley}, S.~E. and {Spruit}, H.~C.},
    title = "{Presupernova Evolution of Differentially Rotating Massive Stars Including Magnetic Fields}",
  journal = {\apj},
   eprint = {astro-ph/0409422},
 keywords = {Stars: Pulsars: General, Stars: Evolution, Stars: Magnetic Fields, Stars: Rotation},
     year = 2005,
    month = jun,
   volume = 626,
    pages = {350-363},
      doi = {10.1086/429868},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...626..350H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{hollenbach_apj_41_1979,
   author = {{Hollenbach}, D. and {McKee}, C.~F.},
    title = "{Molecule formation and infrared emission in fast interstellar shocks. I Physical processes}",
  journal = {\apjs},
 keywords = {ASTROPHYSICS, INFRARED RADIATION, INTERSTELLAR GAS, MOLECULAR GASES, SHOCK WAVES, CHEMICAL REACTIONS, DEUTERIUM, GAS DENSITY, GAS DISSOCIATION, GAS TEMPERATURE, MOLECULAR INTERACTIONS, SHOCK FRONTS},
     year = 1979,
    month = nov,
   volume = 41,
    pages = {555-592},
      doi = {10.1086/190631},
   adsurl = {http://adsabs.harvard.edu/abs/1979ApJS...41..555H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{holzer_araa_8_1970,
   author = {{Holzer}, T.~E. and {Axford}, W.~I.},
    title = "{The Theory of Stellar Winds and Related Flows}",
  journal = {\araa},
     year = 1970,
   volume = 8,
    pages = {31},
      doi = {10.1146/annurev.aa.08.090170.000335},
   adsurl = {http://adsabs.harvard.edu/abs/1970ARA%26A...8...31H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{houk_1975,
   author = {{Houk}, N. and {Cowley}, A.~P.},
    title = "{University of Michigan Catalogue of two-dimensional spectral types for the HD stars. Volume I. Declinations -90\_ to -53\_{\fnof}0.}",
booktitle = {University of Michigan Catalogue of two-dimensional spectral types for the HD stars.~Volume I.~Declinations -90\_ to -53\_{\fnof}0., by Houk, N.; Cowley, A.~P..~ Ann Arbor, MI (USA): Department of Astronomy, University of Michigan, 19 + 452 p.},
     year = 1975,
   adsurl = {http://cdsads.u-strasbg.fr/abs/1975mcts.book.....H},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE I 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%



@ARTICLE{izmodenov_apj_795_2014,
   author = {{Izmodenov}, V.~V. and {Alexashov}, D.~B. and {Ruderman}, M.~S.
	},
    title = "{Electron Thermal Conduction as a Possible Physical Mechanism to Make the Inner Heliosheath Thinner}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1409.8128},
 primaryClass = "astro-ph.SR",
 keywords = {conduction, solar wind, Sun: heliosphere},
     year = 2014,
    month = nov,
   volume = 795,
      eid = {L7},
    pages = {L7},
      doi = {10.1088/2041-8205/795/1/L7},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...795L...7I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{indebetouw_apj_619_2005,
   author = {{Indebetouw}, R. and {Mathis}, J.~S. and {Babler}, B.~L. and 
	{Meade}, M.~R. and {Watson}, C. and {Whitney}, B.~A. and {Wolff}, M.~J. and 
	{Wolfire}, M.~G. and {Cohen}, M. and {Bania}, T.~M. and {Benjamin}, R.~A. and 
	{Clemens}, D.~P. and {Dickey}, J.~M. and {Jackson}, J.~M. and 
	{Kobulnicky}, H.~A. and {Marston}, A.~P. and {Mercer}, E.~P. and 
	{Stauffer}, J.~R. and {Stolovy}, S.~R. and {Churchwell}, E.},
    title = "{The Wavelength Dependence of Interstellar Extinction from 1.25 to 8.0 {$\mu$}m Using GLIMPSE Data}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0406403},
 keywords = {ISM: Dust, Extinction, Infrared: ISM},
     year = 2005,
    month = feb,
   volume = 619,
    pages = {931-938},
      doi = {10.1086/426679},
   adsurl = {http://adsabs.harvard.edu/abs/2005ApJ...619..931I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ingalls_apj_579_2002,
   author = {{Ingalls}, J.~G. and {Reach}, W.~T. and {Bania}, T.~M.},
    title = "{Photoelectric Heating and [C II] Cooling of High Galactic Latitude Translucent Clouds}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0207264},
 keywords = {ISM: Dust, Extinction, Infrared: ISM: Continuum, Infrared: ISM: Lines and Bands, ISM: Atoms, ISM: Clouds},
     year = 2002,
    month = nov,
   volume = 579,
    pages = {289-303},
      doi = {10.1086/342704},
   adsurl = {http://adsabs.harvard.edu/abs/2002ApJ...579..289I},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE J 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{jun_apj_472_1996,
       author = {{Jun}, Byung-Il and {Norman}, Michael L.},
        title = "{On the Origin of Radial Magnetic Fields in Young Supernova Remnants}",
      journal = {\apj},
     keywords = {INSTABILITIES, ISM: MAGNETIC FIELDS, METHODS: NUMERICAL, POLARIZATION, RADIO CONTINUUM: ISM, ISM: SUPERNOVA REMNANTS, TURBULENCE, Astrophysics},
         year = 1996,
        month = nov,
       volume = {472},
        pages = {245},
          doi = {10.1086/178059},
archivePrefix = {arXiv},
       eprint = {astro-ph/9606096},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1996ApJ...472..245J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{janka_review,
author = {Janka, Hans-Thomas},
title = {Explosion Mechanisms of Core-Collapse Supernovae},
journal = {Annual Review of Nuclear and Particle Science},
volume = {62},
number = {1},
pages = {407-451},
year = {2012},
doi = {10.1146/annurev-nucl-102711-094901},
URL = { https://doi.org/10.1146/annurev-nucl-102711-094901},
eprint = { https://doi.org/10.1146/annurev-nucl-102711-094901}
}


@ARTICLE{janka_arnps_66_2016,
       author = {{Janka}, Hans-Thomas and {Melson}, Tobias and {Summa}, Alexander},
        title = "{Physics of Core-Collapse Supernovae in Three Dimensions: A Sneak Preview}",
      journal = {Annual Review of Nuclear and Particle Science},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, High Energy Physics - Phenomenology, Nuclear Theory},
         year = 2016,
        month = oct,
       volume = {66},
       number = {1},
        pages = {341-375},
          doi = {10.1146/annurev-nucl-102115-044747},
archivePrefix = {arXiv},
       eprint = {1602.05576},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ARNPS..66..341J},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{james_aa_453_2006,
   author = {{James}, P.~A. and {Anderson}, J.~P.},
    title = "{The H{$\alpha$} Galaxy Survey . III. Constraints on supernova progenitors from spatial correlations with H{$\alpha$} emission}",
  journal = {\aap},
   eprint = {astro-ph/0602471},
 keywords = {galaxies: general, galaxies: spiral, galaxies: photometry, galaxies: statistics, stars: supernovae: general},
     year = 2006,
    month = jul,
   volume = 453,
    pages = {57-65},
      doi = {10.1051/0004-6361:20054509},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...453...57J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{jorissen_532_aa_2011,
   author = {{Jorissen}, A. and {Mayer}, A. and {van Eck}, S. and {Ottensamer}, R. and 
	{Kerschbaum}, F. and {Ueta}, T. and {Bergman}, P. and {Blommaert}, J.~A.~D.~L. and 
	{Decin}, L. and {Groenewegen}, M.~A.~T. and {Hron}, J. and {Nowotny}, W. and 
	{Olofsson}, H. and {Posch}, T. and {Sjouwerman}, L.~O. and {Vandenbussche}, B. and 
	{Waelkens}, C.},
    title = "{X Herculis and TX Piscium: two cases of ISM interaction with stellar winds observed by Herschel}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1106.3645},
 primaryClass = "astro-ph.SR",
 keywords = {ISM: general, stars: AGB and post-AGB, stars: mass-loss, infrared: stars, stars: carbon},
     year = 2011,
    month = aug,
   volume = 532,
      eid = {A135},
    pages = {A135},
      doi = {10.1051/0004-6361/201116927},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...532A.135J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{juvela_aa_397_2003,
   author = {{Juvela}, M. and {Padoan}, P.},
    title = "{Dust emission from inhomogeneous interstellar clouds: Radiative transfer in 3D with transiently heated particles}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0207379},
 keywords = {ISM: clouds, infrared: ISM, radiative transfer},
     year = 2003,
    month = jan,
   volume = 397,
    pages = {201-212},
      doi = {10.1051/0004-6361:20021433},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...397..201J},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{jager_aas_72_1988,
   author = {{de Jager}, C. and {Nieuwenhuijzen}, H. and {van der Hucht}, K.~A.
	},
    title = "{Mass loss rates in the Hertzsprung-Russell diagram}",
  journal = {\aaps},
 keywords = {HERTZSPRUNG-RUSSELL DIAGRAM, O STARS, PLANETARY NEBULAE, STELLAR LUMINOSITY, STELLAR MASS EJECTION, WOLF-RAYET STARS, B STARS, CARBON STARS, COMPUTATIONAL ASTROPHYSICS, HIGH TEMPERATURE, HOT STARS, STELLAR MASS},
     year = 1988,
    month = feb,
   volume = 72,
    pages = {259-289},
   adsurl = {http://adsabs.harvard.edu/abs/1988A%26AS...72..259D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE K 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{kothes_apj_746_2012,
       author = {{Kothes}, R. and {Foster}, T.},
        title = "{A Thorough Investigation of the Distance to the Supernova Remnant CTB109 and Its Pulsar AXP J2301+5852}",
      journal = {\apjl},
     keywords = {ISM: individual objects: CTB109, ISM: supernova remnants, pulsars: individual: AXP J2301+5852},
         year = 2012,
        month = feb,
       volume = {746},
       number = {1},
          eid = {L4},
        pages = {L4},
          doi = {10.1088/2041-8205/746/1/L4},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012ApJ...746L...4K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{kothes_aa_597_2017,
       author = {{Kothes}, Roland and {Reich}, Patricia and {Foster}, Tyler J. and {Reich}, Wolfgang},
        title = "{G181.1+9.5, a new high-latitude low-surface brightness supernova remnant}",
      journal = {\aap},
     keywords = {polarization, ISM: magnetic fields, ISM: supernova remnants, ISM: individual objects: G181.1+9.5, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = jan,
       volume = {597},
          eid = {A116},
        pages = {A116},
          doi = {10.1051/0004-6361/201629848},
archivePrefix = {arXiv},
       eprint = {1612.01956},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...597A.116K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{kogan_apss_166_1990,
       author = {{Bisnovatyi-Kogan}, G.~S. and {Lozinskaia}, T.~A. and {Silich}, S.~A.},
        title = "{Barrel-Like Supernova Remnants}",
      journal = {\apss},
     keywords = {Computational Astrophysics, Stellar Structure, Supernova Remnants, Digital Simulation, Radio Astronomy, Stellar Physics, Stellar Winds, Astrophysics},
         year = "1990",
        month = "Apr",
       volume = {166},
       number = {2},
        pages = {277-287},
          doi = {10.1007/BF01094899},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1990Ap&SS.166..277B},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{katushkina_MNRAS_473_2018,
   author = {{Katushkina}, O.~A. and {Alexashov}, D.~B. and {Gvaramadze}, V.~V. and 
	{Izmodenov}, V.~V.},
    title = "{An astrosphere around the blue supergiant {$\kappa$} Cas: possible explanation of its filamentary structure}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1709.09494},
 primaryClass = "astro-ph.SR",
 keywords = {shock waves, methods: numerical, stars: individual: {$\kappa$} Cas, dust, extinction},
     year = 2018,
    month = jan,
   volume = 473,
    pages = {1576-1588},
      doi = {10.1093/mnras/stx2488},
   adsurl = {http://adsabs.harvard.edu/abs/2018MNRAS.473.1576K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{katushkina_MNRAS_465_2017,
   author = {{Katushkina}, O.~A. and {Alexashov}, D.~B. and {Izmodenov}, V.~V. and 
	{Gvaramadze}, V.~V.},
    title = "{Non-monotonic spatial distribution of the interstellar dust in astrospheres: finite gyroradius effect}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1612.08349},
 primaryClass = "astro-ph.SR",
 keywords = {shock waves, methods: numerical, circumstellar matter, dust, extinction},
     year = 2017,
    month = feb,
   volume = 465,
    pages = {1573-1585},
      doi = {10.1093/mnras/stw2833},
   adsurl = {http://adsabs.harvard.edu/abs/2017MNRAS.465.1573K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kim_apj_422_1994,
   author = {{Kim}, S.-H. and {Martin}, P.~G. and {Hendry}, P.~D.},
    title = "{The size distribution of interstellar dust particles as determined from extinction}",
  journal = {\apj},
 keywords = {Abundance, Chemical Composition, Computational Astrophysics, Cosmic Dust, Infrared Radiation, Interstellar Extinction, Light Scattering, Mass Distribution, Size Distribution, Brightness, Curve Fitting, Maximum Entropy Method, Numerical Analysis, Parameterization},
     year = 1994,
    month = feb,
   volume = 422,
    pages = {164-175},
      doi = {10.1086/173714},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1994ApJ...422..164K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{katsuda_apj_863_2018,
       author = {{Katsuda}, Satoru and {Takiwaki}, Tomoya and {Tominaga}, Nozomu and
         {Moriya}, Takashi J. and {Nakamura}, Ko},
        title = "{Progenitor Mass Distribution of Core-collapse Supernova Remnants in Our Galaxy and Magellanic Clouds Based on Elemental Abundances}",
      journal = {\apj},
     keywords = {ISM: supernova remnants, supernovae: general, stars: massive, X-rays: general, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = aug,
       volume = {863},
       number = {2},
          eid = {127},
        pages = {127},
          doi = {10.3847/1538-4357/aad2d8},
archivePrefix = {arXiv},
       eprint = {1807.03426},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...863..127K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@ARTICLE{katsuda_apj_754_2012,
   author = {{Katsuda}, S. and {Tsunemi}, H. and {Mori}, K. and {Uchida}, H. and 
	{Petre}, R. and {Yamada}, S. and {Tamagawa}, T.},
    title = "{Discovery of a Pulsar Wind Nebula Candidate in the Cygnus Loop}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1206.4367},
 primaryClass = "astro-ph.HE",
 keywords = {ISM: individual objects: Cygnus Loop, ISM: supernova remnants, pulsars: general, stars: neutron, stars: winds, outflows, X-rays: ISM},
     year = 2012,
    month = jul,
   volume = 754,
      eid = {L7},
    pages = {L7},
      doi = {10.1088/2041-8205/754/1/L7},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012ApJ...754L...7K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{kane_apj_511_1999,
   author = {{Kane}, J. and {Drake}, R.~P. and {Remington}, B.~A.},
    title = "{An Evaluation of the Richtmyer-Meshkov Instability in Supernova Remnant Formation}",
  journal = {\apj},
 keywords = {HYDRODYNAMICS, INSTABILITIES, ISM: SUPERNOVA REMNANTS, STARS: SUPERNOVAE: GENERAL, Hydrodynamics, Instabilities, ISM: Supernova Remnants, Stars: Supernovae: General},
     year = 1999,
    month = jan,
   volume = 511,
    pages = {335-340},
      doi = {10.1086/306685},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...511..335K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kahn_mnras_212_1985,
   author = {{Kahn}, F.~D. and {West}, K.~A.},
    title = "{Shapes of planetary nebulae}",
  journal = {\mnras},
 keywords = {PLANETARY NEBULAE, STELLAR WINDS, ANGULAR MOMENTUM, GAS PRESSURE, STELLAR MASS EJECTION, STELLAR MODELS},
     year = 1985,
    month = feb,
   volume = 212,
    pages = {837-850},
   adsurl = {http://adsabs.harvard.edu/abs/1985MNRAS.212..837K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kaper_apj_475_1997,
   author = {{Kaper}, L. and {van Loon}, J.~T. and {Augusteijn}, T. and {Goudfrooij}, P. and 
	{Patat}, F. and {Waters}, L.~B.~F.~M. and {Zijlstra}, A.~A.},
    title = "{Discovery of a Bow Shock around VELA X-1}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/9611017},
 keywords = {STARS: BINARIES: CLOSE, GALAXY: OPEN CLUSTERS AND ASSOCIATIONS: INDIVIDUAL NAME: VEL OB1, STARS: INDIVIDUAL HENRY DRAPER NUMBER: HD 77581, STARS: MASS LOSS, STARS: PULSARS: INDIVIDUAL NAME: VELA X-1, STARS: SUPERNOVAE: GENERAL},
     year = 1997,
    month = jan,
   volume = 475,
    pages = {L37},
      doi = {10.1086/310454},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJ...475L..37K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@article{kaufman_EAS2009,
author = {Kaufman,M.J. and Kaufman,M.J.},
title = {Physical and Chemical Processes in the Diffuse and Dense Neutral ISM},
journal = {EAS Publications Series},
volume = {34},
month = {1},
year = {2009},
issn = {1638-1963},
pages = {151--161},
numpages = {11},
doi = {10.1051/eas:0934011},
URL = {http://www.eas-journal.org/article_S1633476009340119},
}

@ARTICLE{kesteven_aa_183_1987,
   author = {{Kesteven}, M.~J. and {Caswell}, J.~L.},
    title = "{Barrel-shaped supernova remnants}",
  journal = {\aap},
 keywords = {Astronomical Maps, Supernova Remnants, Morphology, Statistical Analysis, X Ray Astronomy},
     year = 1987,
    month = sep,
   volume = 183,
    pages = {118-128},
   adsurl = {http://adsabs.harvard.edu/abs/1987A%26A...183..118K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kroupa_mnras_322_2001,
   author = {{Kroupa}, P.},
    title = "{On the variation of the initial mass function}",
  journal = {\mnras},
   eprint = {astro-ph/0009005},
 keywords = {BINARIES: GENERAL, STARS: FORMATION, STARS: KINEMATICS, STARS: LUMINOSITY FUNCTION, MASS FUNCTION, GLOBULAR CLUSTERS: GENERAL, OPEN CLUSTERS AND ASSOCIATIONS: GENERAL},
     year = 2001,
    month = apr,
   volume = 322,
    pages = {231-246},
      doi = {10.1046/j.1365-8711.2001.04022.x},
   adsurl = {http://adsabs.harvard.edu/abs/2001MNRAS.322..231K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kwak_apj_739_2011,
   author = {{Kwak}, K. and {Henley}, D.~B. and {Shelton}, R.~L.},
    title = "{Simulations of High-velocity Clouds. I. Hydrodynamics and High-velocity High Ions}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1106.6326},
 primaryClass = "astro-ph.GA",
 keywords = {Galaxy: halo, hydrodynamics, ISM: clouds, methods: numerical, turbulence, ultraviolet: ISM},
     year = 2011,
    month = sep,
   volume = 739,
      eid = {30},
    pages = {30},
      doi = {10.1088/0004-637X/739/1/30},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...739...30K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kobulnicky_apj_710_2010,
   author = {{Kobulnicky}, H.~A. and {Gilbert}, I.~J. and {Kiminki}, D.~C.
	},
    title = "{OB Stars and Stellar Bow shocks in Cygnus-X: A Novel Laboratory Estimating Stellar Mass Loss Rates}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0912.1314},
 keywords = {open clusters and associations: individual: Cygnus OB2, stars: early-type, stars: individual: BD+43{\deg}3654 HD 195229 GSC 03161 {\ndash} 01188},
     year = 2010,
    month = feb,
   volume = 710,
    pages = {549-566},
      doi = {10.1088/0004-637X/710/1/549},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...710..549K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kobulnicky_apjs_227_2016,
       author = {{Kobulnicky}, Henry A. and {Chick}, William T. and
         {Schurhammer}, Danielle P. and {Andrews}, Julian E. and
         {Povich}, Matthew S. and {Munari}, Stephan A. and {Olivier}, Grace M. and
         {Sorber}, Rebecca L. and {Wernke}, Heather N. and {Dale}, Daniel A.},
        title = "{A Comprehensive Search for Stellar Bowshock Nebulae in the Milky Way: A Catalog of 709 Mid-infrared Selected Candidates}",
      journal = {\apjs},
     keywords = {dust, extinction, H ii regions, stars: early-type, stars: kinematics and dynamics, Stars: massive, surveys, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = "2016",
        month = "Dec",
       volume = {227},
       number = {2},
          eid = {18},
        pages = {18},
          doi = {10.3847/0067-0049/227/2/18},
archivePrefix = {arXiv},
       eprint = {1609.02204},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJS..227...18K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kobulnicky_apj_856_2018,
       author = {{Kobulnicky}, Henry A. and {Chick}, William T. and {Povich}, Matthew S.},
        title = "{Demonstration of a Novel Method for Measuring Mass-loss Rates for Massive Stars}",
      journal = {\apj},
     keywords = {catalogs, H ii regions, stars: massive, surveys, Astrophysics - Solar and Stellar Astrophysics},
         year = "2018",
        month = "Mar",
       volume = {856},
       number = {1},
          eid = {74},
        pages = {74},
          doi = {10.3847/1538-4357/aab3e0},
archivePrefix = {arXiv},
       eprint = {1803.02794},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...856...74K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kobulnicky_aj_154_2017,
       author = {{Kobulnicky}, Henry A. and {Schurhammer}, Danielle P. and
         {Baldwin}, Daniel J. and {Chick}, William T. and {Dixon}, Don M. and
         {Lee}, Daniel and {Povich}, Matthew S.},
        title = "{Infrared Photometric Properties of 709 Candidate Stellar Bowshock Nebulae}",
      journal = {\aj},
     keywords = {catalogs, HII regions, ISM: bubbles, stars: massive, surveys, Astrophysics - Solar and Stellar Astrophysics},
         year = "2017",
        month = "Nov",
       volume = {154},
       number = {5},
          eid = {201},
        pages = {201},
          doi = {10.3847/1538-3881/aa90ba},
archivePrefix = {arXiv},
       eprint = {1710.07892},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017AJ....154..201K},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{kothes_aa_457_2006,
   author = {{Kothes}, R. and {Fedotov}, K. and {Foster}, T.~J. and {Uyan{\i}ker}, B.
	},
    title = "{A catalogue of Galactic supernova remnants from the Canadian Galactic plane survey. I. Flux densities, spectra, and polarization characteristics}",
  journal = {\aap},
 keywords = {atlases, catalogs, polarization, ISM: supernova remnants},
     year = 2006,
    month = oct,
   volume = 457,
    pages = {1081-1093},
      doi = {10.1051/0004-6361:20065062},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...457.1081K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kwok_apj_198_1975,
   author = {{Kwok}, S.},
    title = "{Radiation pressure on grains as a mechanism for mass loss in red giants}",
  journal = {\apj},
 keywords = {GIANT STARS, LATE STARS, M STARS, RADIATION PRESSURE, STELLAR MASS EJECTION, ABSORPTION SPECTRA, COSMIC DUST, MOMENTUM TRANSFER, RADIATIVE TRANSFER, STELLAR ENVELOPES, STELLAR SPECTRA},
     year = 1975,
    month = jun,
   volume = 198,
    pages = {583-591},
      doi = {10.1086/153637},
   adsurl = {http://adsabs.harvard.edu/abs/1975ApJ...198..583K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{kudritzki_aa_219_1989,
   author = {{Kudritzki}, R.~P. and {Pauldrach}, A. and {Puls}, J. and {Abbott}, D.~C.
	},
    title = "{Radiation-driven winds of hot stars. VI - Analytical solutions for wind models including the finite cone angle effect}",
  journal = {\aap},
 keywords = {HOT STARS, STELLAR RADIATION, STELLAR WINDS, EQUATIONS OF MOTION, O STARS, PHOTOSPHERE, PLANETARY NEBULAE, STELLAR MASS EJECTION},
     year = 1989,
    month = jul,
   volume = 219,
    pages = {205-218},
   adsurl = {http://adsabs.harvard.edu/abs/1989A%26A...219..205K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{keppens_jplph_61_1999,
   author = {{Keppens}, R. and {T{\'o}th}, G. and {Westermann}, R.~H.~J. and 
	{Goedbloed}, J.~P.},
    title = "{Growth and saturation of the Kelvin-Helmholtz instability with parallel and antiparallel magnetic fields}",
  journal = {Journal of Plasma Physics},
   eprint = {astro-ph/9901166},
     year = 1999,
    month = jan,
   volume = 61,
    pages = {1-19},
      doi = {10.1017/S0022377898007223},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1999JPlPh..61....1K},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE L 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{2021arXiv210105771L,
       author = {{Lux}, O. and {Neuh{\"a}user}, R. and {Mugrauer}, M. and {Bischoff}, R.},
        title = "{A search for runaway stars in twelve Galactic supernova remnants}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2021,
        month = jan,
          eid = {arXiv:2101.05771},
        pages = {arXiv:2101.05771},
archivePrefix = {arXiv},
       eprint = {2101.05771},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2021arXiv210105771L},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{laor_apj_402_1993,
   author = {{Laor}, A. and {Draine}, B.~T.},
    title = "{Spectroscopic constraints on the properties of dust in active galactic nuclei}",
  journal = {\apj},
 keywords = {Active Galactic Nuclei, Astronomical Models, Astronomical Spectroscopy, Computational Astrophysics, Cosmic Dust, Emission Spectra, Grain Size, Graphite, Interstellar Extinction, Optical Properties, Optical Thickness, Silicon Carbides},
     year = 1993,
    month = jan,
   volume = 402,
    pages = {441-468},
      doi = {10.1086/172149},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...402..441L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lagache_aa_333_1998,
   author = {{Lagache}, G. and {Abergel}, A. and {Boulanger}, F. and {Puget}, J.-L.
	},
    title = "{The interstellar cold dust observed by COBE}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/9812474},
 keywords = {ISM: CLOUDS, DUST, EXTINCTION, STRUCTURE, GENERAL, INFRARED: ISM: CONTINUUM, RADIO CONTINUUM: ISM},
     year = 1998,
    month = may,
   volume = 333,
    pages = {709-720},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...333..709L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{1966hydr.book.....L,
   author = {{Landau}, L.~D. and {Lifshitz}, E.~M.},
    title = "{Hydrodynamik}",
booktitle = {Lehrbuch der theoretischen Physik},
publisher = {Berlin: Akademie-Verlag},
     year = 1966,
   adsurl = {http://cdsads.u-strasbg.fr/abs/1966hydr.book.....L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{langer_ApJ_520_1999,
   author = {{Langer}, N. and {Garc{\'{\i}}a-Segura}, G. and {Mac Low}, M.-M.
	},
    title = "{Giant Outbursts of Luminous Blue Variables and the Formation of the Homunculus Nebula around eta Carinae}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/9905025},
 keywords = {STARS: CIRCUMSTELLAR MATTER, HYDRODYNAMICS, STARS: EVOLUTION, STARS: INDIVIDUAL: CONSTELLATION NAME: ETA CARINAE, STARS: MASS LOSS, STARS: ROTATION},
     year = 1999,
    month = jul,
   volume = 520,
    pages = {L49-L53},
      doi = {10.1086/312131},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...520L..49L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{langer_araa_50_2012,
   author = {{Langer}, N.},
    title = "{Presupernova Evolution of Massive Single and Binary Stars}",
  journal = {\araa},
archivePrefix = "arXiv",
   eprint = {1206.5443},
 primaryClass = "astro-ph.SR",
     year = 2012,
    month = sep,
   volume = 50,
    pages = {107-164},
      doi = {10.1146/annurev-astro-081811-125534},
   adsurl = {http://adsabs.harvard.edu/abs/2012ARA%26A..50..107L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@TechReport{langer_dfg_2011,
	title = "DFG Priority Programme 1573 : the physics of the interstellar medium",
	author = "N. Langer",
	institution = "Argelander Institut fur Astronomie",
	month = "February",
	year = "2011"
}

@ARTICLE{lallement_aa_411_2003,
   author = {{Lallement}, R. and {Welsh}, B.~Y. and {Vergely}, J.~L. and 
	{Crifo}, F. and {Sfeir}, D.},
    title = "{3D mapping of the dense interstellar gas around the Local Bubble}",
  journal = {\aap},
 keywords = {Galaxy: solar neighborhood, ISM: atoms, ISM: clouds},
     year = 2003,
    month = dec,
   volume = 411,
    pages = {447-464},
      doi = {10.1051/0004-6361:20031214},
   adsurl = {http://adsabs.harvard.edu/abs/2003A%26A...411..447L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{lamer_cassinelli_1999,
   author = {{Lamers}, H.~J.~G.~L.~M. and {Cassinelli}, J.~P.},
    title = "{Introduction to Stellar Winds}",
booktitle = {Introduction to Stellar Winds, by Henny J.~G.~L.~M.~Lamers and Joseph P.~Cassinelli, pp.~452.~ISBN 0521593980.~Cambridge, UK: Cambridge University Press, June 1999.},
     year = 1999,
    month = jun,
   adsurl = {http://adsabs.harvard.edu/abs/1999isw..book.....L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@BOOK{lequeux_springerverlag,
   author = {{Lequeux}, J.},
    title = "{The Interstellar Medium}",
booktitle = {The interstellar medium, Translation from the French language edition 
of: Le Milieu Interstellaire by James Lequeux, EDP Sciences, 2003 Edited by J.~Lequeux.~ Astronomy and astrophysics library, Berlin: Springer, 2005},
     year = 2005,
      doi = {10.1007/b137959},
   adsurl = {http://adsabs.harvard.edu/abs/2005ism..book.....L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Book{lequeux_edp,
	title = "Le milieu interstellaire",
	author = "J. Lequeux",
	publisher = "CNRS Editions",
	edition = "EDP sciences",
	month = "March",
	year = "2002",
	isbn = "2 86889 533 3"
}

@ARTICLE{leeuwen_aa_474_2007,
   author = {{van Leeuwen}, F.},
    title = "{Validation of the new Hipparcos reduction}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0708.1752},
 keywords = {space vehicles: instruments, methods: data analysis, catalogs, astrometry, instrumentation: miscellaneous},
     year = 2007,
    month = nov,
   volume = 474,
    pages = {653-664},
      doi = {10.1051/0004-6361:20078357},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2007A%26A...474..653V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lebertre_mnras_422_2012,
   author = {{Le Bertre}, T. and {Matthews}, L.~D. and {G{\'e}rard}, E. and 
	{Libert}, Y.},
    title = "{Discovery of a detached H I gas shell surrounding {$\alpha$} Orionis}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1203.0255},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, stars: individual: {$\alpha$} Ori, stars: mass-loss, supergiants, radio lines: stars},
     year = 2012,
    month = jun,
   volume = 422,
    pages = {3433-3443},
      doi = {10.1111/j.1365-2966.2012.20853.x},
   adsurl = {http://adsabs.harvard.edu/abs/2012MNRAS.422.3433L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{liszt_499_aa_2009,
   author = {{Liszt}, H.~S. and {Pety}, J. and {Tachihara}, K.},
    title = "{Imaging galactic diffuse clouds: CO emission, reddening and turbulent flow in the gas around {$\zeta$} Ophiuchi}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0901.1111},
 keywords = {astrochemistry, ISM: molecules, ISM: clouds},
     year = 2009,
    month = may,
   volume = 499,
    pages = {503-513},
      doi = {10.1051/0004-6361:200810905},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...499..503L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lockett_apj_511_1999,
   author = {{Lockett}, P. and {Gauthier}, E. and {Elitzur}, M.},
    title = "{OH 1720 Megahertz Masers in Supernova Remnants: C-Shock Indicators}",
  journal = {\apj},
   eprint = {astro-ph/9809019},
 keywords = {ISM: CLOUDS, MASERS, SHOCK WAVES, ISM: SUPERNOVA REMNANTS, ISM: Clouds, Masers, Shock Waves, ISM: Supernova Remnants},
     year = 1999,
    month = jan,
   volume = 511,
    pages = {235-241},
      doi = {10.1086/306667},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...511..235L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lodders_apj_591_2003,
   author = {{Lodders}, K.},
    title = "{Solar System Abundances and Condensation Temperatures of the Elements}",
  journal = {\apj},
 keywords = {Astrochemistry, Meteors, Meteoroids, Solar System: Formation- Sun: Abundances, Sun: Photosphere},
     year = 2003,
    month = jul,
   volume = 591,
    pages = {1220-1247},
      doi = {10.1086/375492},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...591.1220L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{lopez_apj_757_2012,
   author = {{L{\'o}pez-Santiago}, J. and {Miceli}, M. and {del Valle}, M.~V. and 
	{Romero}, G.~E. and {Bonito}, R. and {Albacete-Colombo}, J.~F. and 
	{Pereira}, V. and {de Castro}, E. and {Damiani}, F.},
    title = "{AE Aurigae: First Detection of Non-thermal X-Ray Emission from a Bow Shock Produced by a Runaway Star}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1208.6511},
 primaryClass = "astro-ph.HE",
 keywords = {ISM: clouds, radiation mechanisms: non-thermal, stars: individual: AE Aur, stars: kinematics and dynamics, stars: massive, X-rays: general },
     year = 2012,
    month = sep,
   volume = 757,
      eid = {L6},
    pages = {L6},
      doi = {10.1088/2041-8205/757/1/L6},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...757L...6L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{lucy_aa_344_1999,
   author = {{Lucy}, L.~B.},
    title = "{Computing radiative equilibria with Monte Carlo techniques}",
  journal = {\aap},
 keywords = {RADIATIVE TRANSFER, METHODS: NUMERICAL, STARS: ATMOSPHERES},
     year = 1999,
    month = apr,
   volume = 344,
    pages = {282-288},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1999A%26A...344..282L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{lyne_natur_369_1994,
   author = {{Lyne}, A.~G. and {Lorimer}, D.~R.},
    title = "{High birth velocities of radio pulsars}",
  journal = {\nat},
     year = 1994,
    month = may,
   volume = 369,
    pages = {127-129},
      doi = {10.1038/369127a0},
   adsurl = {http://adsabs.harvard.edu/abs/1994Natur.369..127L},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE M 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{moranchel_mnras_472_2017,
       author = {{Moranchel-Basurto}, A. and {Vel{\'a}zquez}, P.~F. and {Giacani}, E. and {Toledo-Roy}, J.~C. and {Schneiter}, E.~M. and {De Colle}, F. and {Esquivel}, A.},
        title = "{Origin of the bilateral structure of the supernova remnant G296.5+10}",
      journal = {\mnras},
     keywords = {MHD, radiation mechanisms: non-thermal, shock waves, methods: numerical, ISM: supernova remnants, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2017,
        month = dec,
       volume = {472},
       number = {2},
        pages = {2117-2125},
          doi = {10.1093/mnras/stx2086},
archivePrefix = {arXiv},
       eprint = {1709.00460},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.472.2117M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{moranchel_mnras_494_2020,
       author = {{Moranchel-Basurto}, A. and {Vel{\'a}zquez}, P.~F. and {Ares de Parga}, G. and {Reynoso}, E.~M. and {Schneiter}, E.~M. and {Esquivel}, A.},
        title = "{Simulated synchrotron emission for the Tycho's supernova remnants: an asymmetric initial mass model}",
      journal = {\mnras},
     keywords = {MHD, radiation mechanisms: non-thermal, shock waves, methods: numerical, ISM: supernova remnants},
         year = 2020,
        month = mar,
       volume = {494},
       number = {2},
        pages = {1531-1538},
          doi = {10.1093/mnras/staa627},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.494.1531M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{moriya_mnras_476_2018,
       author = {{Moriya}, Takashi J. and {F{\"o}rster}, Francisco and {Yoon}, Sung-Chul and {Gr{\"a}fener}, G{\"o}tz and {Blinnikov}, Sergei I.},
        title = "{Type IIP supernova light curves affected by the acceleration of red supergiant winds}",
      journal = {\mnras},
     keywords = {stars: evolution, stars: mass-loss, supernovae: general, stars: winds, outflows, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = may,
       volume = {476},
       number = {2},
        pages = {2840-2851},
          doi = {10.1093/mnras/sty475},
archivePrefix = {arXiv},
       eprint = {1802.07752},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.476.2840M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{murray_mnras_475_2018,
       author = {{Murray}, Daniel and {Goyal}, Shivam and {Chang}, Philip},
        title = "{The effects of protostellar jet feedback on turbulent collapse}",
      journal = {\mnras},
     keywords = {turbulence, stars: formation, galaxies: star clusters: general, galaxies: star formation, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = 2018,
        month = mar,
       volume = {475},
       number = {1},
        pages = {1023-1035},
          doi = {10.1093/mnras/stx3153},
archivePrefix = {arXiv},
       eprint = {1710.09415},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.475.1023M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{Moffat1998,
       author = {{Moffat}, A.~F.~J. and {Marchenko}, S.~V. and {Seggewiss}, W. and
         {van der Hucht} et al. , K.~A. et al. },
        title = "{Wolf-Rayet stars and O-star runaways with HIPPARCOS. I. Kinematics}",
      journal = {\aap},
     keywords = {ASTROMETRY, STARS: KINEMATICS, STARS: EARLY-TYPE, STARS: WOLF-RAYET, GALAXY: KINEMATICS AND DYNAMICS},
         year = 1998,
        month = mar,
       volume = {331},
        pages = {949-958},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1998A&A...331..949M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{Munoz2017,
       author = {{Munoz}, Melissa and {Moffat}, Anthony F.~J. and {Hill}, Grant M. and
         {Shenar}, Tomer and {Richardson}, Noel D. and {Pablo}, Herbert and
         {St-Louis}, Nicole and {Ramiaramanantsoa}, Tahina},
        title = "{WR 148: identifying the companion of an extreme runaway massive binary$^{*}$}",
      journal = {\mnras},
     keywords = {binaries: spectroscopic, stars: individual: WR 148, stars: kinematics and dynamics, stars: mass-loss, stars: winds, outflows, stars: Wolf-Rayet, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = may,
       volume = {467},
       number = {3},
        pages = {3105-3121},
          doi = {10.1093/mnras/stw2283},
archivePrefix = {arXiv},
       eprint = {1609.08289},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.467.3105M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{meyer_mnras_496_2020,
       author = {{Meyer}, D.~M. -A. and {Oskinova}, L.~M. and {Pohl}, M. and {Petrov}, M.},
        title = "{On the ring nebulae around runaway Wolf─Rayet stars}",
      journal = {\mnras},
     keywords = {Radiative transfer, MHD, stars: circumstellar matter, methods: numerical, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = jul,
       volume = {496},
       number = {3},
        pages = {3906-3911},
          doi = {10.1093/mnras/staa1700},
archivePrefix = {arXiv},
       eprint = {2006.06027},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.496.3906M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{meyer_mnras_493_2020,
       author = {{Meyer}, D.~M. -A. and {Petrov}, M. and {Pohl}, M.},
        title = "{Wind nebulae and supernova remnants of very massive stars}",
      journal = {\mnras},
     keywords = {shock waves, methods: numerical, circumstellar matter, stars: massive, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies},
         year = 2020,
        month = apr,
       volume = {493},
       number = {3},
        pages = {3548-3564},
          doi = {10.1093/mnras/staa554},
archivePrefix = {arXiv},
       eprint = {2002.08268},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.493.3548M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{marchenko_apj_724_2010,
       author = {{Marchenko}, S.~V. and {Moffat}, A.~F.~J. and {Crowther}, P.~A.},
        title = "{Population I Wolf-Rayet Runaway Stars: The Case of WR124 and its Expanding Nebula M1-67}",
      journal = {\apjl},
     keywords = {gamma-ray burst: general, stars: distances, stars: individual: WR 124, stars: Wolf-Rayet, supernovae: general, Astrophysics - Solar and Stellar Astrophysics},
         year = "2010",
        month = "Nov",
       volume = {724},
       number = {1},
        pages = {L90-L94},
          doi = {10.1088/2041-8205/724/1/L90},
archivePrefix = {arXiv},
       eprint = {1011.0785},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010ApJ...724L..90M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{macdomald_mnras_197_1981,
   author = {{MacDonald}, J. and {Bailey}, M.~E.},
    title = "{The evolution of flows of stellar mass loss in active galaxies}",
  journal = {\mnras},
 keywords = {Active Galaxies, Astronomical Models, Elliptical Galaxies, Flow Characteristics, Galactic Evolution, Gas Flow, Stellar Winds, Equations Of State, Galactic Radiation, Galactic Structure, Numerical Analysis, Stellar Evolution, Supernovae},
     year = 1981,
    month = dec,
   volume = 197,
    pages = {995-1019},
   adsurl = {http://adsabs.harvard.edu/abs/1981MNRAS.197..995M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{maclow_apr_407_1993,
   author = {{Mac Low}, M.-M. and {Norman}, M.~L.},
    title = "{Nonlinear growth of dynamical overstabilities in blast waves}",
  journal = {\apj},
 keywords = {DYNAMIC STABILITY, INTERSTELLAR MATTER, SHOCK WAVES, SUPERNOVA REMNANTS, ASTRONOMICAL MODELS, HYDRODYNAMICS},
     year = 1993,
    month = apr,
   volume = 407,
    pages = {207-218},
      doi = {10.1086/172506},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJ...407..207M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{maclow_apj_369_1991,
   author = {{Mac Low}, M.-M. and {van Buren}, D. and {Wood}, D.~O.~S. and 
	{Churchwell}, E.},
    title = "{Bow shock models of ultracompact H II regions}",
  journal = {\apj},
 keywords = {ASTRONOMICAL MODELS, H II REGIONS, MOLECULAR CLOUDS, SHOCK WAVE PROPAGATION, STELLAR WINDS, ASTRONOMICAL MAPS, DIGITAL SIMULATION, INFRARED ASTRONOMY SATELLITE, INTERSTELLAR MATTER, MILKY WAY GALAXY, RADIATIVE TRANSFER},
     year = 1991,
    month = mar,
   volume = 369,
    pages = {395-409},
      doi = {10.1086/169769},
   adsurl = {http://adsabs.harvard.edu/abs/1991ApJ...369..395M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mackey_mnras_412_2010,
   author = {{Mackey}, J. and {Lim}, A.~J.},
    title = "{Effects of magnetic fields on photoionized pillars and globules}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1012.1500},
 primaryClass = "astro-ph.GA",
 keywords = {MHD, radiative transfer, methods: numerical, H II regions, ISM: magnetic fields},
     year = 2011,
    month = apr,
   volume = 412,
    pages = {2079-2094},
      doi = {10.1111/j.1365-2966.2010.18043.x},
   adsurl = {http://adsabs.harvard.edu/abs/2011MNRAS.412.2079M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mackey_bsrsl_2011,
   author = {{Mackey}, J. and {Lim}, A.~J.},
    title = "{Radiation-MHD models of elephant trunks and globules in HII regions}",
  journal = {Bulletin de la Societe Royale des Sciences de Liege},
archivePrefix = "arXiv",
   eprint = {1104.1073},
 primaryClass = "astro-ph.GA",
     year = 2011,
    month = jan,
   volume = 80,
    pages = {391-395},
   adsurl = {http://adsabs.harvard.edu/abs/2011BSRSL..80..391M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mackey_mnras_403_2010,
   author = {{Mackey}, J. and {Lim}, A.~J.},
    title = "{Dynamical models for the formation of elephant trunks in HII regions}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0912.1499},
 primaryClass = "astro-ph.GA",
 keywords = {hydrodynamics, radiative transfer, methods: numerical, HII regions},
     year = 2010,
    month = apr,
   volume = 403,
    pages = {714-730},
      doi = {10.1111/j.1365-2966.2009.16181.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.403..714M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mackey_apjlett_751_2012,
   author = {{Mackey}, J. and {Mohamed}, S. and {Neilson}, H.~R. and {Langer}, N. and 
	{Meyer}, D.~M.-A.},
    title = "{Double Bow Shocks around Young, Runaway Red Supergiants: Application to Betelgeuse}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1204.3925},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, hydrodynamics, stars: evolution, stars: individual: Betelgeuse, stars: winds, outflows },
     year = 2012,
    month = may,
   volume = 751,
      eid = {L10},
    pages = {L10},
      doi = {10.1088/2041-8205/751/1/L10},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...751L..10M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{mackey_sept_2014,
       author = {{Mackey}, Jonathan and {Gvaramadze}, Vasilii V. and {Mohamed}, Shazrene and
         {Langer}, Norbert},
        title = "{Wind bubbles within H ii regions around slowly moving stars}",
      journal = {\aap},
     keywords = {hydrodynamics, radiative transfer, methods: numerical, ISM: bubbles, Hii regions, stars: winds, outflows, Astrophysics - Astrophysics of Galaxies, Astrophysics - Solar and Stellar Astrophysics},
         year = "2015",
        month = "Jan",
       volume = {573},
          eid = {A10},
        pages = {A10},
          doi = {10.1051/0004-6361/201424716},
archivePrefix = {arXiv},
       eprint = {1410.0019},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...573A..10M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2014Natur.512..282M,
   author = {{Mackey}, J. and {Mohamed}, S. and {Gvaramadze}, V.~V. and {Kotak}, R. and 
	{Langer}, N. and {Meyer}, D.~M.-A. and {Moriya}, T.~J. and {Neilson}, H.~R.
	},
    title = "{Interacting supernovae from photoionization-confined shells around red supergiant stars}",
  journal = {\nat},
archivePrefix = "arXiv",
   eprint = {1408.2522},
 primaryClass = "astro-ph.SR",
     year = 2014,
    month = aug,
   volume = 512,
    pages = {282-285},
      doi = {10.1038/nature13522},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2014Natur.512..282M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
@ARTICLE{mackey_2013,
   author = {{Mackey}, J.},
    title = "{Moving HII regions around massive stars: Application to Betelgeuse}",
     year = 2013
}

@ARTICLE{mackey_mnras_2013,
   author = {{Mackey}, J. and {Langer}, N. and {Gvaramadze}, V.~V.},
    title = "{Dynamics of H II regions around exiled O stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1308.5192},
 primaryClass = "astro-ph.GA",
 keywords = {hydrodynamics, radiative transfer, methods: numerical, stars: early-type, stars: individual: {$\zeta$} Oph, H II regions},
     year = 2013,
    month = sep,
      doi = {10.1093/mnras/stt1621},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.tmp.2269M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{mackey_aa_586_2016,
   author = {{Mackey}, J. and {Haworth}, T.~J. and {Gvaramadze}, V.~V. and 
	{Mohamed}, S. and {Langer}, N. and {Harries}, T.~J.},
    title = "{Detecting stellar-wind bubbles through infrared arcs in H ii regions}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1512.06857},
 keywords = {hydrodynamics, radiative transfer, methods: numerical, Hii regions, ISM: bubbles, stars: winds, outflows},
     year = 2016,
    month = feb,
   volume = 586,
      eid = {A114},
    pages = {A114},
      doi = {10.1051/0004-6361/201527569},
   adsurl = {http://adsabs.harvard.edu/abs/2016A%26A...586A.114M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{maeder_rvmp_84_2012,
   author = {{Maeder}, A. and {Meynet}, G.},
    title = "{Rotating massive stars: From first stars to gamma ray bursts}",
  journal = {Reviews of Modern Physics},
 keywords = {Stellar rotation, Mass loss and stellar winds, Abundances, chemical composition, Main-sequence: early-type stars},
     year = 2012,
    month = jan,
   volume = 84,
    pages = {25-63},
      doi = {10.1103/RevModPhys.84.25},
   adsurl = {http://adsabs.harvard.edu/abs/2012RvMP...84...25M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Book{ maeder_2009,
	title = "Physics, Formation and Evolution of Rotating Stars",
	author = "A. Maeder",
	publisher = "Astronomy and Astrophysics Library",
	edition = "SPringer-Verlag",
	year = "2009"
}

@ARTICLE{manchester_aa_171_1987,
   author = {{Manchester}, R.~N.},
    title = "{The radio structure of supernova remnants}",
  journal = {\aap},
 keywords = {Radio Spectra, Spectral Energy Distribution, Stellar Models, Stellar Structure, Supernova Remnants, Astronomical Maps, Binary Stars, Pulsars, Stellar Evolution},
     year = 1987,
    month = jan,
   volume = 171,
    pages = {205-215},
   adsurl = {http://adsabs.harvard.edu/abs/1987A%26A...171..205M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{martins_aa_538_2012,
   author = {{Martins}, F. and {Escolano}, C. and {Wade}, G.~A. and {Donati}, J.~F. and 
	{Bouret}, J.~C. and {Mimes Collaboration}},
    title = "{Observational effects of magnetism in O stars: surface nitrogen abundances}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1112.2497},
 primaryClass = "astro-ph.SR",
 keywords = {stars: massive, stars: atmospheres, stars: fundamental parameters, stars: abundances, stars: magnetic field},
     year = 2012,
    month = feb,
   volume = 538,
      eid = {A29},
    pages = {A29},
      doi = {10.1051/0004-6361/201118039},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...538A..29M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{martin_aa_538b_2012,
   author = {{Martins}, F. and {Mahy}, L. and {Hillier}, D.~J. and {Rauw}, G.
	},
    title = "{A quantitative study of O stars in NGC 2244 and the Monoceros OB2 association}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1110.4509},
 primaryClass = "astro-ph.SR",
 keywords = {stars: fundamental parameters, stars: winds, outflows, stars: early-type, Hii regions},
     year = 2012,
    month = feb,
   volume = 538,
      eid = {A39},
    pages = {A39},
      doi = {10.1051/0004-6361/201117458},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012A%26A...538A..39M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mckee_apj_195_1975,
   author = {{McKee}, C.~F. and {Ostriker}, J.~P.},
    title = "{A theory of the interstellar medium - Three components regulated by supernova explosions in an inhomogeneous substrate}",
  journal = {\apj},
 keywords = {INTERSTELLAR MATTER, NEBULAE, SUPERNOVA REMNANTS, X RAY SOURCES, ABSORPTION SPECTRA, ADIABATIC CONDITIONS, ASTRONOMICAL MODELS, BACKGROUND RADIATION, CLOUDS, EVAPORATION, HIGH TEMPERATURE GASES, RAREFIED GASES},
     year = 1977,
    month = nov,
   volume = 218,
    pages = {148-169},
      doi = {10.1086/155667},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...218..148M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{1975ApJ...195..715M,
   author = {{McKee}, C.~F. and {Cowie}, L.~L.},
    title = "{The interaction between the blast wave of a supernova remnant and interstellar clouds}",
  journal = {\apj},
 keywords = {INTERSTELLAR GAS, SHOCK HEATING, SHOCK WAVE INTERACTION, SUPERNOVA REMNANTS, ABUNDANCE, ASTRONOMICAL MODELS, CLOUD PHYSICS, LIGHT EMISSION, STELLAR EVOLUTION, X RAY ASTRONOMY},
     year = 1975,
    month = feb,
   volume = 195,
    pages = {715-725},
      doi = {10.1086/153373},
   adsurl = {http://adsabs.harvard.edu/abs/1975ApJ...195..715M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{martins_aa_468_2007,
   author = {{Martins}, F. and {Genzel}, R. and {Hillier}, D.~J. and {Eisenhauer}, F. and 
	{Paumard}, T. and {Gillessen}, S. and {Ott}, T. and {Trippe}, S.
	},
    title = "{Stellar and wind properties of massive stars in the central parsec of the Galaxy}",
  journal = {\aap},
   eprint = {astro-ph/0703211},
 keywords = {stars: early-type, stars: Wolf-Rayet, stars: atmospheres, stars: fundamental parameters, stars: winds, outflows, Galaxy: center},
     year = 2007,
    month = jun,
   volume = 468,
    pages = {233-254},
      doi = {10.1051/0004-6361:20066688},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...468..233M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{martins_aa_436_2005,
   author = {{Martins}, F. and {Schaerer}, D. and {Hillier}, D.~J.},
    title = "{A new calibration of stellar parameters of Galactic O stars}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0503346},
 keywords = {stars: fundamental parameters, stars: atmospheres, stars: early-type},
     year = 2005,
    month = jun,
   volume = 436,
    pages = {1049-1065},
      doi = {10.1051/0004-6361:20042386},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...436.1049M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mathis_apj_217_1977,
   author = {{Mathis}, J.~S. and {Rumpl}, W. and {Nordsieck}, K.~H.},
    title = "{The size distribution of interstellar grains}",
  journal = {\apj},
 keywords = {COSMIC DUST, INTERSTELLAR EXTINCTION, INTERSTELLAR MATTER, PARTICLE SIZE DISTRIBUTION, ENSTATITE, GRAPHITE, MAGNETITE, OLIVINE, POLARIZATION CHARACTERISTICS, ULTRAVIOLET ASTRONOMY},
     year = 1977,
    month = oct,
   volume = 217,
    pages = {425-433},
      doi = {10.1086/155591},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...217..425M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@PROCEEDINGS{massaglia_lnp_754_2008,
   editor = {{Massaglia}, S. and {Bodo}, G. and {Mignone}, A. and {Rossi}, P.
	},
    title = "{Jets From Young Stars III}",
 keywords = {Physics, Astrophysics, Numerical and Computational Methods},
booktitle = {Jets From Young Stars III},
     year = 2008,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 754,
      doi = {10.1007/978-3-540-76967-5},
   adsurl = {http://adsabs.harvard.edu/abs/2008LNP...754.....M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mignone_apj_170_2007,
   author = {{Mignone}, A. and {Bodo}, G. and {Massaglia}, S. and {Matsakos}, T. and 
	{Tesileanu}, O. and {Zanni}, C. and {Ferrari}, A.},
    title = "{PLUTO: A Numerical Code for Computational Astrophysics}",
  journal = {\apjs},
   eprint = {arXiv:astro-ph/0701854},
 keywords = {Hydrodynamics, Methods: Numerical, Magnetohydrodynamics: MHD, Relativity, Shock Waves},
     year = 2007,
    month = may,
   volume = 170,
    pages = {228-242},
      doi = {10.1086/513316},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJS..170..228M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{mazzotta_aaps_133_1998,
   author = {{Mazzotta}, P. and {Mazzitelli}, G. and {Colafrancesco}, S. and 
	{Vittorio}, N.},
    title = "{Ionization balance for optically thin plasmas: Rate coefficients for all atoms and ions of the elements H to NI}",
  journal = {\aaps},
   eprint = {arXiv:astro-ph/9806391},
 keywords = {ATOMIC DATA, PLASMAS, RADIATION MECHANISMS: THERMAL, X-RAYS: GENERAL},
     year = 1998,
    month = dec,
   volume = 133,
    pages = {403-409},
      doi = {10.1051/aas:1998330},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26AS..133..403M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@PROCEEDINGS{2008LNP...754.....M,
   editor = {{Massaglia}, S. and {Bodo}, G. and {Mignone}, A. and {Rossi}, P.
	},
    title = "{Jets From Young Stars III}",
 keywords = {Physics, Astrophysics, Numerical and Computational Methods},
booktitle = {Jets From Young Stars III},
     year = 2008,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 754,
      doi = {10.1007/978-3-540-76967-5},
   adsurl = {http://adsabs.harvard.edu/abs/2008LNP...754.....M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{mccomas_apj_801_2015,
   author = {{McComas}, D.~J. and {Bzowski}, M. and {Frisch}, P. and {Fuselier}, S.~A. and 
	{Kubiak}, M.~A. and {Kucharek}, H. and {Leonard}, T. and {M{\"o}bius}, E. and 
	{Schwadron}, N.~A. and {Sok{\'o}{\l}}, J.~M. and {Swaczyna}, P. and 
	{Witte}, M.},
    title = "{Warmer Local Interstellar Medium: A Possible Resolution of the Ulysses-IBEX Enigma}",
  journal = {\apj},
 keywords = {local interstellar matter, interplanetary medium, ISM: general, Sun: heliosphere},
     year = 2015,
    month = mar,
   volume = 801,
      eid = {28},
    pages = {28},
      doi = {10.1088/0004-637X/801/1/28},
   adsurl = {http://adsabs.harvard.edu/abs/2015ApJ...801...28M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{medina_791_apj_2014,
   author = {{Medina}, A.~A. and {Raymond}, J.~C. and {Edgar}, R.~J. and 
	{Caldwell}, N. and {Fesen}, R.~A. and {Milisavljevic}, D.},
    title = "{Electron-Ion Equilibrium and Shock Precursors in the Northeast Limb of the Cygnus Loop}",
  journal = {\apj},
 keywords = {acceleration of particles, ISM: individual objects: Cygnus Loop, ISM: supernova remnants, shock waves},
     year = 2014,
    month = aug,
   volume = 791,
      eid = {30},
    pages = {30},
      doi = {10.1088/0004-637X/791/1/30},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...791...30M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{meyer_mnras_464_2017,
       author = {{Meyer}, D.~M. -A. and {Mignone}, A. and {Kuiper}, R. and {Raga}, A.~C. and
         {Kley}, W.},
        title = "{Bow shock nebulae of hot massive stars in a magnetized medium}",
      journal = {\mnras},
     keywords = {MHD, methods: numerical, circumstellar matter, stars: massive, Astrophysics - Solar and Stellar Astrophysics},
         year = "2017",
        month = "Jan",
       volume = {464},
       number = {3},
        pages = {3229-3248},
          doi = {10.1093/mnras/stw2537},
archivePrefix = {arXiv},
       eprint = {1610.00543},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.464.3229M},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{meyer_obs_2016,
   author = {{Meyer}, D.~M.-A. and {van Marle}, A.-J. and {Kuiper}, R. and 
	{Kley}, W.},
    title = "{On the observability of bow shocks of Galactic runaway OB stars}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1603.04755},
 primaryClass = "astro-ph.SR",
 keywords = {methods: numerical, circumstellar matter, stars: massive},
     year = 2016,
    month = jun,
   volume = 459,
    pages = {1146-1158},
      doi = {10.1093/mnras/stw651},
   adsurl = {http://adsabs.harvard.edu/abs/2016MNRAS.459.1146M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{meyer_mnras_450_2015,
   author = {{Meyer}, D.~M.-A. and {Langer}, N. and {Mackey}, J. and {Vel{\'a}zquez}, P.~F. and 
	{Gusdorf}, A.},
    title = "{Asymmetric supernova remnants generated by Galactic, massive runaway stars}",
  journal = {\mnras},
 keywords = {shock waves, methods: numerical, stars: massive, ISM: supernova remnants},
     year = 2015,
    month = jul,
   volume = 450,
    pages = {3080-3100},
      doi = {10.1093/mnras/stv898},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2015MNRAS.450.3080M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{meyer_2014a,
   author = {{Meyer}, D.~M.-A. and {Gvaramadze}, V.~V. and {Langer}, N. and 
	{Mackey}, J. and {Boumis}, P. and {Mohamed}, S.},
    title = "{On the stability of bow shocks generated by red supergiants: the case of IRC -10414}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1312.1687},
 primaryClass = "astro-ph.SR",
 keywords = {shock waves, methods: numerical, circumstellar matter, stars: individual: IRC -10414, stars: massive},
     year = 2014,
    month = mar,
   volume = 439,
    pages = {L41-L45},
      doi = {10.1093/mnrasl/slt176},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.439L..41M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{meyer_2014bb,
   author = {{Meyer}, D.~M.-A. and {Mackey}, J. and {Langer}, N. and {Gvaramadze}, V.~V. and 
	{Mignone}, A. and {Izzard}, R.~G. and {Kaper}, L.},
    title = "{Models of the circumstellar medium of evolving, massive runaway stars moving through the Galactic plane}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1408.2828},
 primaryClass = "astro-ph.SR",
 keywords = {shock waves, methods: numerical, circumstellar matter, stars: massive},
     year = 2014,
    month = nov,
   volume = 444,
    pages = {2754-2775},
      doi = {10.1093/mnras/stu1629},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.444.2754M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{mignone_lnp_754b_2008,
   author = {{Mignone}, A. and {Bodo}, G.},
    title = "{Shock-Capturing Schemes in Computational MHD}",
booktitle = {Jets From Young Stars III},
     year = 2008,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 754,
   editor = "{S.~Massaglia, G.~Bodo, A.~Mignone, \& P.~Rossi}",
    pages = {71-101},
      doi = {10.1007/978-3-540-76967-5_2},
   adsurl = {http://adsabs.harvard.edu/abs/2008LNP...754...71M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{mignone_lnp_754a_2008,
   author = {{Toro}, E.~F.},
    title = "{Computational Methods for Hyperbolic Equations}",
booktitle = {Jets From Young Stars III},
     year = 2008,
   series = {Lecture Notes in Physics, Berlin Springer Verlag},
   volume = 754,
   editor = "{S.~Massaglia, G.~Bodo, A.~Mignone, \& P.~Rossi}",
    pages = {3-69},
      doi = {10.1007/978-3-540-76967-5_1},
   adsurl = {http://adsabs.harvard.edu/abs/2008LNP...754....3T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@Manual{mignone_user_guide_pluto_2011,
	title = "Pluto User's Guide",
	author = "A. Mignone and P. Tzeferacos and G. Bodo and T. Matsakos and O. Tesileanu and C. Zanni",
	month = "April",
	year = "2011"
}

@ARTICLE{mitchell_mnras_362_2005,
   author = {{Mitchell}, D.~L. and {Bryce}, M. and {Meaburn}, J. and {L{\'o}pez}, J.~A. and 
	{Redman}, M.~P. and {Harman}, D. and {Richer}, M.~G. and {Riesgo}, H.
	},
    title = "{The kinematics of the large western knot in the halo of the young planetary nebula NGC 6543}",
  journal = {\mnras},
   eprint = {arXiv:astro-ph/0507204},
 keywords = {circumstellar matter, stars: kinematics, stars: mass-loss, stars: winds, outflows, ISM: planetary nebulae: individual: NGC 6543},
     year = 2005,
    month = oct,
   volume = 362,
    pages = {1286-1294},
      doi = {10.1111/j.1365-2966.2005.09399.x},
   adsurl = {http://adsabs.harvard.edu/abs/2005MNRAS.362.1286M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{mohamed_aa_541_2012,
   author = {{Mohamed}, S. and {Mackey}, J. and {Langer}, N.},
    title = "{3D simulations of Betelgeuse's bow shock}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1109.1555},
 primaryClass = "astro-ph.SR",
 keywords = {hydrodynamics, instabilities, circumstellar matter, stars: winds, outflows, supergiants, ISM: structure},
     year = 2012,
    month = may,
   volume = 541,
      eid = {A1},
    pages = {A1},
      doi = {10.1051/0004-6361/201118002},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...541A...1M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{mokiem_aa_465_2007,
   author = {{Mokiem}, M.~R. and {de Koter}, A. and {Evans}, C.~J. and {Puls}, J. and 
	{Smartt}, S.~J. and {Crowther}, P.~A. and {Herrero}, A. and 
	{Langer}, N. and {Lennon}, D.~J. and {Najarro}, F. and {Villamariz}, M.~R. and 
	{Vink}, J.~S.},
    title = "{The VLT-FLAMES survey of massive stars: wind properties and evolution of hot massive stars in the Large Magellanic Cloud}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0704.1113},
 keywords = {galaxies: Magellanic Clouds, stars: atmospheres, stars:, early-type, stars: fundamental parameters, stars: mass loss, stars: evolution},
     year = 2007,
    month = apr,
   volume = 465,
    pages = {1003-1019},
      doi = {10.1051/0004-6361:20066489},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...465.1003M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{moore_aj_124_2002,
   author = {{Moore}, B.~D. and {Walter}, D.~K. and {Hester}, J.~J. and {Scowen}, P.~A. and 
	{Dufour}, R.~J. and {Buckalew}, B.~A.},
    title = "{Hubble Space Telescope Observations of the Windblown Nebula NGC 7635}",
  journal = {\aj},
 keywords = {ISM: H II Regions, ISM: Individual: NGC Number: NGC 7635, ISM: Kinematics and Dynamics, Stars: Individual: Alphanumeric: BD +60{\deg}2522, Stars: Mass Loss},
     year = 2002,
    month = dec,
   volume = 124,
    pages = {3313-3324},
      doi = {10.1086/344596},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2002AJ....124.3313M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Manual{mignone_developer_guide_pluto_2011,
	title = "Pluto Developer's Guide",
	author = "A. Mignone",
	month = "April",
	year = "2011"
}


@ARTICLE{migmone_apjs_198_2012,
   author = {{Mignone}, A. and {Zanni}, C. and {Tzeferacos}, P. and {van Straalen}, B. and 
	{Colella}, P. and {Bodo}, G.},
    title = "{The PLUTO Code for Adaptive Mesh Computations in Astrophysical Fluid Dynamics}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1110.0740},
 primaryClass = "astro-ph.HE",
 keywords = {hydrodynamics, magnetohydrodynamics: MHD, methods: numerical },
     year = 2012,
    month = jan,
   volume = 198,
      eid = {7},
    pages = {7},
      doi = {10.1088/0067-0049/198/1/7},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJS..198....7M},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE N 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{neugebauer_278_apj_1984,
   author = {{Neugebauer}, G. and {Habing}, H.~J. and {van Duinen}, R. and 
	{Aumann}, H.~H. and {Baud}, B. and {Beichman}, C.~A. and {Beintema}, D.~A. and 
	{Boggess}, N. and {Clegg}, P.~E. and {de Jong}, T. and {Emerson}, J.~P. and 
	{Gautier}, T.~N. and {Gillett}, F.~C. and {Harris}, S. and {Hauser}, M.~G. and 
	{Houck}, J.~R. and {Jennings}, R.},
    title = "{The Infrared Astronomical Satellite (IRAS) mission}",
  journal = {\apjl},
 keywords = {Infrared Astronomy Satellite, Satellite-Borne Instruments, Spaceborne Astronomy, Calibrating, Cryogenic Cooling, Data Reduction, Focal Plane Devices, Infrared Telescopes, Spaceborne Telescopes},
     year = 1984,
    month = mar,
   volume = 278,
    pages = {L1-L6},
      doi = {10.1086/184209},
   adsurl = {http://adsabs.harvard.edu/abs/1984ApJ...278L...1N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{neufeld_apj_781_2014,
   author = {{Neufeld}, D.~A. and {Gusdorf}, A. and {G{\"u}sten}, R. and 
	{Herczeg}, G.~J. and {Kristensen}, L. and {Melnick}, G.~J. and 
	{Nisini}, B. and {Ossenkopf}, V. and {Tafalla}, M. and {van Dishoeck}, E.~F.
	},
    title = "{The Water Abundance behind Interstellar Shocks: Results from Herschel/PACS and Spitzer/IRS Observations of H$_{2}$O, CO, and H$_{2}$}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1312.6703},
 primaryClass = "astro-ph.GA",
 keywords = {infrared: ISM, ISM: abundances, ISM: molecules, molecular processes, shock waves},
     year = 2014,
    month = feb,
   volume = 781,
      eid = {102},
    pages = {102},
      doi = {10.1088/0004-637X/781/2/102},
   adsurl = {http://adsabs.harvard.edu/abs/2014ApJ...781..102N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{neilson_apj_716_2010,
   author = {{Neilson}, H.~R. and {Ngeow}, C.-C. and {Kanbur}, S.~M. and 
	{Lester}, J.~B.},
    title = "{Testing Mass Loss in Large Magellanic Cloud Cepheids using Infrared and Optical Observations. II. Predictions and Tests of the OGLE-III Fundamental-mode Cepheids}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1005.0622},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, Magellanic Clouds, stars: mass-loss, stars: variables: Cepheids},
     year = 2010,
    month = jun,
   volume = 716,
    pages = {1136-1150},
      doi = {10.1088/0004-637X/716/2/1136},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...716.1136N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{2012A&A...537A..35C,
   author = {{Cox}, N.~L.~J. and {Kerschbaum}, F. and {van Marle}, A.-J. and 
	{Decin}, L. and {Ladjal}, D. and {Mayer}, A. and {Groenewegen}, M.~A.~T. and 
	{van Eck}, S. and {Royer}, P. and {Ottensamer}, R. and {Ueta}, T. and 
	{Jorissen}, A. and {Mecina}, M. and {Meliani}, Z. and {Luntzer}, A. and 
	{Blommaert}, J.~A.~D.~L. and {Posch}, T. and {Vandenbussche}, B. and 
	{Waelkens}, C.},
    title = "{A far-infrared survey of bow shocks and detached shells around AGB stars and red supergiants}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1110.5486},
 primaryClass = "astro-ph.GA",
 keywords = {stars: AGB and post-AGB, circumstellar matter, infrared: ISM, hydrodynamics, stars: mass-loss, stars: winds, outflows},
     year = 2012,
    month = jan,
   volume = 537,
      eid = {A35},
    pages = {A35},
      doi = {10.1051/0004-6361/201117910},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...537A..35C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{neilson_aa_529_2011,
   author = {{Neilson}, H.~R. and {Cantiello}, M. and {Langer}, N.},
    title = "{The Cepheid mass discrepancy and pulsation-driven mass loss}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1104.1638},
 primaryClass = "astro-ph.SR",
 keywords = {stars: mass-loss, stars: variables: Cepheids, stars: fundamental parameters},
     year = 2011,
    month = may,
   volume = 529,
      eid = {L9},
    pages = {L9},
      doi = {10.1051/0004-6361/201116920},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...529L...9N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{noriegacrespo_aj_113_1997,
   author = {{Noriega-Crespo}, A. and {van Buren}, D. and {Dgani}, R.},
    title = "{Bow Shocks Around Runaway Stars.III.The High Resolution Maps}",
  journal = {\aj},
     year = 1997,
    month = feb,
   volume = 113,
    pages = {780-786},
      doi = {10.1086/118298},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1997AJ....113..780N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{noriegacrespo_aj_114_1997,
   author = {{Noriega-Crespo}, A. and {van Buren}, D. and {Cao}, Y. and {Dgani}, R.
	},
    title = "{A Parsec-Size Bow Shock around Betelgeuse}",
  journal = {\aj},
 keywords = {TURBULENCE, ISM: STRUCTURE, STARS: INDIVIDUAL: BETELGEUSE},
     year = 1997,
    month = aug,
   volume = 114,
    pages = {837-840},
      doi = {10.1086/118517},
   adsurl = {http://adsabs.harvard.edu/abs/1997AJ....114..837N},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE O 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{ohara_apj_598_2003,
   author = {{O'Hara}, T.~B. and {Meixner}, M. and {Speck}, A.~K. and {Ueta}, T. and 
	{Bobrowsky}, M.},
    title = "{The Dust Ring of Luminous Blue Variable Candidate HD 168625: Infrared Observations and Model Calculations}",
  journal = {\apj},
 keywords = {Stars: Circumstellar Matter, Infrared: Stars, Stars: Individual: Henry Draper Number: HD 168625, Stars: Mass Loss, Stars: Variables: Other},
     year = 2003,
    month = dec,
   volume = 598,
    pages = {1255-1264},
      doi = {10.1086/379058},
   adsurl = {https://ui.adsabs.harvard.edu/abs/2003ApJ...598.1255O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{ohno_mnras_262_1993,
   author = {{Ohno}, H. and {Shibata}, S.},
    title = "{The random magnetic field in the Galaxy}",
  journal = {\mnras},
 keywords = {Interstellar Magnetic Fields, Interstellar Matter, Pulsars, Random Processes, Radiative Transfer, Spatial Distribution},
     year = 1993,
    month = jun,
   volume = 262,
    pages = {953-962},
   adsurl = {http://adsabs.harvard.edu/abs/1993MNRAS.262..953O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{orlando_aa_470_2007,
   author = {{Orlando}, S. and {Bocchino}, F. and {Reale}, F. and {Peres}, G. and 
	{Petruk}, O.},
    title = "{On the origin of asymmetries in bilateral supernova remnants}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0704.0890},
 keywords = {magnetohydrodynamics (MHD), shock waves, ISM: supernova remnants, ISM: magnetic fields, radio continuum: ISM},
     year = 2007,
    month = aug,
   volume = 470,
    pages = {927-939},
      doi = {10.1051/0004-6361:20066045},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2007A%26A...470..927O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{orlando_apj_749_2012,
   author = {{Orlando}, S. and {Bocchino}, F. and {Miceli}, M. and {Petruk}, O. and 
	{Pumo}, M.~L.},
    title = "{Role of Ejecta Clumping and Back-reaction of Accelerated Cosmic Rays in the Evolution of Type Ia Supernova Remnants}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1202.3593},
 primaryClass = "astro-ph.HE",
 keywords = {cosmic rays, instabilities, ISM: supernova remnants, magnetohydrodynamics: MHD, shock waves, supernovae: individual: SN 1006},
     year = 2012,
    month = apr,
   volume = 749,
      eid = {156},
    pages = {156},
      doi = {10.1088/0004-637X/749/2/156},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2012ApJ...749..156O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ostriker_apj_184_1973,
   author = {{Ostriker}, J. and {Silk}, J.},
    title = "{Dust Cooling of Hot Gas}",
  journal = {\apjl},
     year = 1973,
    month = sep,
   volume = 184,
    pages = {L113},
      doi = {10.1086/181301},
   adsurl = {http://adsabs.harvard.edu/abs/1973ApJ...184L.113O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{ostriker_revmodphys_60_1988,
   author = {{Ostriker}, J.~P. and {McKee}, C.~F.},
    title = "{Astrophysical blastwaves}",
  journal = {Reviews of Modern Physics},
     year = 1988,
   volume = 60,
    pages = {1-68},
      doi = {10.1103/RevModPhys.60.1},
   adsurl = {http://adsabs.harvard.edu/abs/1988RvMP...60....1O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{orlando_aa_444_2005,
   author = {{Orlando}, S. and {Peres}, G. and {Reale}, F. and {Bocchino}, F. and 
	{Rosner}, R. and {Plewa}, T. and {Siegel}, A.},
    title = "{Crushing of interstellar gas clouds in supernova remnants. I. The role of thermal conduction and radiative losses}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0508638},
 keywords = {hydrodynamics, shock waves, ISM: clouds, ISM: supernova remnants},
     year = 2005,
    month = dec,
   volume = 444,
    pages = {505-519},
      doi = {10.1051/0004-6361:20052896},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...444..505O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{opher_natur_462_2009,
   author = {{Opher}, M. and {Bibi}, F.~A. and {Toth}, G. and {Richardson}, J.~D. and 
	{Izmodenov}, V.~V. and {Gombosi}, T.~I.},
    title = "{A strong, highly-tilted interstellar magnetic field near the Solar System}",
  journal = {\nat},
     year = 2009,
    month = dec,
   volume = 462,
    pages = {1036-1038},
      doi = {10.1038/nature08567},
   adsurl = {http://adsabs.harvard.edu/abs/2009Natur.462.1036O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{orlando_apj_678_2008,
   author = {{Orlando}, S. and {Bocchino}, F. and {Reale}, F. and {Peres}, G. and 
	{Pagano}, P.},
    title = "{The Importance of Magnetic-Field-Oriented Thermal Conduction in the Interaction of SNR Shocks with Interstellar Clouds}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0801.1403},
 keywords = {Conduction, ISM: Clouds, ISM: Magnetic Fields, Magnetohydrodynamics: MHD, Shock Waves, ISM: Supernova Remnants},
     year = 2008,
    month = may,
   volume = 678,
    pages = {274-286},
      doi = {10.1086/529420},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...678..274O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{osterbrock_1989,
   author = {{Osterbrock}, D.~E. and {Bochkarev}, N.~G.},
    title = "{Book-Review - Astrophysics of Gaseous Nebulae and Active Galactic Nuclei}",
  journal = {\sovast},
     year = 1989,
    month = nov,
   volume = 33,
    pages = {694},
   adsurl = {http://adsabs.harvard.edu/abs/1989SvA....33..694O},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE P 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{paron_aa_498_2009,
       author = {{Paron}, S. and {Ortega}, M.~E. and {Rubio}, M. and {Dubner}, G.},
        title = "{A molecular outflow revealing star formation activity in the vicinity of the HII region G034.8-0.7 and the SNR W44}",
      journal = {\aap},
     keywords = {ISM: molecules, ISM: clouds, ISM: jets and outflows, stars: formation, Astrophysics - Astrophysics of Galaxies},
         year = 2009,
        month = may,
       volume = {498},
       number = {2},
        pages = {445-453},
          doi = {10.1051/0004-6361/200811292},
archivePrefix = {arXiv},
       eprint = {0902.2333},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009A&A...498..445P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{2019arXiv190912332P,
       author = {{Prajapati}, Prachi and {Tej}, Anandmayee and {del Palacio}, Santiago and
         {Benaglia}, Paula and {CH}, Ishwara-Chandra and {Vig}, Sarita and {Mand
        al}, Samir and {Kanti Ghosh}, Swarna},
        title = "{Investigating Particle Acceleration in the Wolf-Rayet Bubble G2.4+1.4}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = "2019",
        month = "Sep",
          eid = {arXiv:1909.12332},
        pages = {arXiv:1909.12332},
archivePrefix = {arXiv},
       eprint = {1909.12332},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190912332P},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{pannuti_147_aj_2014,
   author = {{Pannuti}, T.~G. and {Rho}, J. and {Heinke}, C.~O. and {Moffitt}, W.~P.
	},
    title = "{The X-Ray Properties of Five Galactic Supernova Remnants Detected by the Spitzer GLIMPSE Survey}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1312.3929},
 primaryClass = "astro-ph.HE",
 keywords = {ISM: individual objects: SNR 304.6+0.1 SNR 311.5{\ndash}0.3 SNR 346.6{\ndash}0.2 SNR 348.5+0.1 SNR 348.5{\ndash}0.0, ISM: supernova remnants, X-rays: ISM},
     year = 2014,
    month = mar,
   volume = 147,
      eid = {55},
    pages = {55},
      doi = {10.1088/0004-6256/147/3/55},
   adsurl = {http://adsabs.harvard.edu/abs/2014AJ....147...55P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{panic_aa_501_2005,
   author = {{Pani{\'c}}, O. and {Hogerheijde}, M.~R. and {Wilner}, D. and 
	{Qi}, C.},
    title = "{A break in the gas and dust surface density of the disc around the T Tauri star IM Lupi}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0904.1127},
 primaryClass = "astro-ph.EP",
 keywords = {planetary systems: protoplanetary disks, stars:, individual: IM Lup, stars: pre-main sequence, circumstellar matter},
     year = 2009,
    month = jul,
   volume = 501,
    pages = {269-278},
      doi = {10.1051/0004-6361/200911883},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...501..269P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{pagani_aa_429_2005,
   author = {{Pagani}, L. and {Apponi}, A.~J. and {Bacmann}, A. and {Cabrit}, S. and 
	{Cambr{\'e}sy}, L. and {Lagache}, G. and {Motte}, F. and {Pardo}, J.-R.
	},
    title = "{L183 (=L134N) revisited}",
 keywords = {L183, Depletion, CO},
booktitle = {ESA Special Publication},
     year = 2005,
   series = {ESA Special Publication},
   volume = 577,
   editor = "{A.~Wilson}",
    month = jan,
    pages = {403-404},
   adsurl = {http://adsabs.harvard.edu/abs/2005ESASP.577..403P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{parker_paj_128_1958,
   author = {{Parker}, E.~N.},
    title = "{Dynamics of the Interplanetary Gas and Magnetic Fields.}",
  journal = {\apj},
     year = 1958,
    month = nov,
   volume = 128,
    pages = {664},
      doi = {10.1086/146579},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1958ApJ...128..664P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@BOOK{parker_1963_book,
   author = {{Parker}, E.~N.},
    title = "{Interplanetary dynamical processes}",
     year = 1963,
  publisher = {New York, Interscience Publishers},
   adsurl = {http://adsabs.harvard.edu/abs/1963QB505.P3.......},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{parker_mnras_362_2005,
   author = {{Parker}, Q.~A. and {Phillipps}, S. and {Pierce}, M.~J. and 
	{Hartley}, M. and {Hambly}, N.~C. and {Read}, M.~A. and {MacGillivray}},
    title = "{The AAO/UKST SuperCOSMOS H{$\alpha$} survey}",
  journal = {\mnras},
   eprint = {astro-ph/0506599},
 keywords = {astronomical data bases: miscellaneous, catalogues, surveys, stars: emission line, photometry},
     year = 2005,
    month = sep,
   volume = 362,
    pages = {689-710},
      doi = {10.1111/j.1365-2966.2005.09350.x},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2005MNRAS.362..689P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pellegrini_bsrsl_80_2011,
   author = {{Pellegrini}, E.~W. and {Oey}, M.~S. and {Winkler}, P.~F. and 
	{Smith}, R.~C. and {Points}, S.},
    title = "{Escaping Radiation from Massive Star HII regions in the Magellanic Clouds}",
  journal = {Bulletin de la Societe Royale des Sciences de Liege},
     year = 2011,
    month = jan,
   volume = 80,
    pages = {410-414},
   adsurl = {http://adsabs.harvard.edu/abs/2011BSRSL..80..410P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{peresrendon_aa_506_2009,
   author = {{P{\'e}rez-Rend{\'o}n}, B. and {Garc{\'{\i}}a-Segura}, G. and 
	{Langer}, N.},
    title = "{Supernova progenitor stars in the initial range of 23 to 33 solar masses and their relation with the SNR Cassiopeia A}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0905.1101},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, ISM: kinematics and dynamics, ISM: supernova remnants, ISM: bubbles, ISM: individual objects: Cassiopeia A},
     year = 2009,
    month = nov,
   volume = 506,
    pages = {1249-1259},
      doi = {10.1051/0004-6361/200809913},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...506.1249P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{peri_aa_578_2015,
   author = {{Peri}, C.~S. and {Benaglia}, P. and {Isequilla}, N.~L.},
    title = "{E-BOSS: An Extensive stellar BOw Shock Survey. II. Catalogue second release}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1504.04264},
 primaryClass = "astro-ph.SR",
 keywords = {catalogs, stars: early-type, infrared: ISM},
     year = 2015,
    month = jun,
   volume = 578,
      eid = {A45},
    pages = {A45},
      doi = {10.1051/0004-6361/201424676},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...578A..45P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{peri_aa_538_2012,
   author = {{Peri}, C.~S. and {Benaglia}, P. and {Brookes}, D.~P. and {Stevens}, I.~R. and 
	{Isequilla}, N.~L.},
    title = "{E-BOSS: an Extensive stellar BOw Shock Survey. I. Methods and first catalogue}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1109.3689},
 primaryClass = "astro-ph.SR",
 keywords = {infrared: ISM, infrared: stars, stars: early-type, catalogs},
     year = 2012,
    month = feb,
   volume = 538,
      eid = {A108},
    pages = {A108},
      doi = {10.1051/0004-6361/201118116},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...538A.108P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{peters_apj_711_2010,
   author = {{Peters}, T. and {Banerjee}, R. and {Klessen}, R.~S. and {Mac Low}, M.-M. and 
	{Galv{\'a}n-Madrid}, R. and {Keto}, E.~R.},
    title = "{H II Regions: Witnesses to Massive Star Formation}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1001.2470},
 primaryClass = "astro-ph.SR",
 keywords = {hydrodynamics, H II regions, radiative transfer, stars: massive},
     year = 2010,
    month = mar,
   volume = 711,
    pages = {1017-1028},
      doi = {10.1088/0004-637X/711/2/1017},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...711.1017P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{petrovic_aa_435_2005,
   author = {{Petrovic}, J. and {Langer}, N. and {Yoon}, S.-C. and {Heger}, A.
	},
    title = "{Which massive stars are gamma-ray burst progenitors?}",
  journal = {\aap},
   eprint = {astro-ph/0504175},
 keywords = {stars: evolution, stars: binaries: close, gamma rays: bursts, stars: rotation, stars: magnetic fields},
     year = 2005,
    month = may,
   volume = 435,
    pages = {247-259},
      doi = {10.1051/0004-6361:20042545},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...435..247P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{petri_aa_439_2005,
   author = {{P{\'e}tri}, J.},
    title = "{An explanation for the kHz-QPO twin peaks separation in slow and fast rotators}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0507167},
 keywords = {accretion, accretion disks, hydrodynamics, methods:, analytical, relativity, stars: neutron, X-rays: binaries},
     year = 2005,
    month = aug,
   volume = 439,
    pages = {L27-L30},
      doi = {10.1051/0004-6361:200500151},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...439L..27P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{petri_apr_302_2006,
   author = {{P'etri}, J.},
    title = "{Forced oscillations in a hydrodynamical accretion disk and QPOs}",
  journal = {\apss},
   eprint = {arXiv:astro-ph/0509668},
 keywords = {accretion, accretion disks, hydrodynamics, instabilities, methods: analytical, methods: numerical, Stars: neutrongoodbreak},
     year = 2006,
    month = apr,
   volume = 302,
    pages = {117-139},
      doi = {10.1007/s10509-005-9013-8},
   adsurl = {http://adsabs.harvard.edu/abs/2006Ap%26SS.302..117P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{petruk_393_mnras_2009,
   author = {{Petruk}, O. and {Dubner}, G. and {Castelletti}, G. and {Bocchino}, F. and 
	{Iakubovskyi}, D. and {Kirsch}, M.~G.~F. and {Miceli}, M. and 
	{Orlando}, S. and {Telezhinsky}, I.},
    title = "{Aspect angle for interstellar magnetic field in SN 1006}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0811.2319},
 keywords = {acceleration of particles , radiation mechanisms: non-thermal , shock waves , cosmic rays , ISM: individual: SN 1006 , supernova remnants},
     year = 2009,
    month = mar,
   volume = 393,
    pages = {1034-1040},
      doi = {10.1111/j.1365-2966.2008.14251.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.393.1034P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{penston_mnras_150_1970,
   author = {{Penston}, M.~V. and {Brown}, F.~E.},
    title = "{The doud-intercloud phase-change in the interstellar medium}",
  journal = {\mnras},
     year = 1970,
   volume = 150,
    pages = {373},
   adsurl = {http://adsabs.harvard.edu/abs/1970MNRAS.150..373P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{povich_apj_689_2008,
   author = {{Povich}, M.~S. and {Benjamin}, R.~A. and {Whitney}, B.~A. and 
	{Babler}, B.~L. and {Indebetouw}, R. and {Meade}, M.~R. and 
	{Churchwell}, E.},
    title = "{Interstellar Weather Vanes: GLIMPSE Mid-Infrared Stellar Wind Bow Shocks in M17 and RCW 49}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0808.2168},
 keywords = {H II regions, infrared: ISM, shock waves, stars: mass loss},
     year = 2008,
    month = dec,
   volume = 689,
      eid = {242-248},
    pages = {242-248},
      doi = {10.1086/592565},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...689..242P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{povich_apjs_194_2011,
   author = {{Povich}, M.~S. and {Smith}, N. and {Majewski}, S.~R. and {Getman}, K.~V. and 
	{Townsley}, L.~K. and {Babler}, B.~L. and {Broos}, P.~S. and 
	{Indebetouw}, R. and {Meade}, M.~R. and {Robitaille}, T.~P. and 
	{Stassun}, K.~G. and {Whitney}, B.~A. and {Yonekura}, Y. and 
	{Fukui}, Y.},
    title = "{A Pan-Carina Young Stellar Object Catalog: Intermediate-mass Young Stellar Objects in the Carina Nebula Identified Via Mid-infrared Excess Emission}",
  journal = {\apjs},
archivePrefix = "arXiv",
   eprint = {1103.2060},
 primaryClass = "astro-ph.SR",
 keywords = {circumstellar matter, ISM: individual objects: NGC 3372, stars: formation, stars: luminosity function, mass function, stars: pre-main sequence, X-rays: stars},
     year = 2011,
    month = may,
   volume = 194,
      eid = {14},
    pages = {14},
      doi = {10.1088/0067-0049/194/1/14},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJS..194...14P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pogolerov_aa_321_1997,
   author = {{Pogorelov}, N.~V. and {Semenov}, A.~Y.},
    title = "{Solar wind interaction with the magnetized interstellar medium. Shock-capturing modeling.}",
  journal = {\aap},
 keywords = {PHYSICAL DATA AND PROCESSES: MHD, SHOCK WAVES, STARS: MASS-LOSS, SUN: SOLAR WIND, ISM: KINEMATICS AND DYNAMICS},
     year = 1997,
    month = may,
   volume = 321,
    pages = {330-337},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1997A%26A...321..330P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pogolerov_aa_354_2000,
   author = {{Pogorelov}, N.~V. and {Matsuda}, T.},
    title = "{Nonevolutionary MHD shocks in the solar wind and interstellar medium interaction}",
  journal = {\aap},
 keywords = {MAGNETOHYDRODYNAMICS (MHD), SHOCK WAVES, SUN: SOLAR WIND, ISM: KINEMATICS AND DYNAMICS},
     year = 2000,
    month = feb,
   volume = 354,
    pages = {697-702},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2000A%26A...354..697P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{postnov_lrr_9_2006,
   author = {{Postnov}, K.~A. and {Yungelson}, L.~R.},
    title = "{The Evolution of Compact Binary Star Systems}",
  journal = {Living Reviews in Relativity},
   eprint = {arXiv:astro-ph/0701059},
 keywords = {relativity in astrophysics, binary systems, gravitational wave sources, supernovae, neutron stars, black holes, white dwarfs, AM CVn stars},
     year = 2006,
    month = dec,
   volume = 9,
    pages = {6},
   adsurl = {http://adsabs.harvard.edu/abs/2006LRR.....9....6P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pogorelov_JGR_103_1998,
   author = {{Pogorelov}, N.~V. and {Matsuda}, T.},
    title = "{Influence of the interstellar magnetic field direction on the shape of the global heliopause}",
  journal = {\jgr},
 keywords = {Interstellar Magnetic Fields, Heliosphere, Magnetic Field Configurations, Solar Wind Velocity, Plasma Interactions, Vectors (Mathematics), Velocity Distribution, Supersonic Flow, Approximation, Shock Wave Interaction},
     year = 1998,
    month = jan,
   volume = 103,
    pages = {237},
      doi = {10.1029/97JA02446},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1998JGR...103..237P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{pound_apss_307_2007,
   author = {{Pound}, M.~W. and {Kane}, J.~O. and {Ryutov}, D.~D. and {Remington}, B.~A. and 
	{Mizuta}, A.},
    title = "{Pillars of Heaven}",
  journal = {\apss},
 keywords = {Eagle Nebula, Radio astronomy, Hydrodynamic models, Aperture synthesis},
     year = 2007,
    month = jan,
   volume = 307,
    pages = {187-190},
      doi = {10.1007/s10509-006-9214-9},
   adsurl = {http://adsabs.harvard.edu/abs/2007Ap%26SS.307..187P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{pikelner_sovietastrlet_12_1969,
   author = {{Pikel'Ner}, S.~B. and {Shcheglov}, P.~V.},
    title = "{Gas Motions in Diffuse Nebulae and Stellar Wind.}",
  journal = {\sovast},
     year = 1969,
    month = apr,
   volume = 12,
    pages = {757},
   adsurl = {http://adsabs.harvard.edu/abs/1969SvA....12..757P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{piran_revmodphys_76_2004,
   author = {{Piran}, T.},
    title = "{The physics of gamma-ray bursts}",
  journal = {Reviews of Modern Physics},
   eprint = {arXiv:astro-ph/0405503},
     year = 2004,
    month = oct,
   volume = 76,
    pages = {1143-1210},
      doi = {10.1103/RevModPhys.76.1143},
   adsurl = {http://adsabs.harvard.edu/abs/2004RvMP...76.1143P},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE R 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{rho_apj_484_1997,
       author = {{Rho}, Jeonghee and {Petre}, R.},
        title = "{X-Ray Imaging and Spectroscopy of the Supernova Remnant CTB 109 and Its Associated Pulsar 1E 2259+586}",
      journal = {\apj},
     keywords = {ISM: Individual: Alphanumeric: CTB 109, pulsars: individual (PSR 1E 2259+586), ISM: Supernova Remnants, X-Rays: ISM},
         year = "1997",
        month = "Jul",
       volume = {484},
       number = {2},
        pages = {828-843},
          doi = {10.1086/304350},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1997ApJ...484..828R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2019arXiv190901424R,
       author = {{Rangelov}, Blagoy and {Montmerle}, Thierry and {Federman}, S.~R. and
         {Boisse}, Patrick and {Gabici}, Stefano},
        title = "{Runaway O-star Bow Shocks as Particle Accelerators? The Case of AE Aur revisited}",
      journal = {arXiv e-prints},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = "2019",
        month = "Sep",
          eid = {arXiv:1909.01424},
        pages = {arXiv:1909.01424},
archivePrefix = {arXiv},
       eprint = {1909.01424},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2019arXiv190901424R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{reynolds_apss_336_2011,
       author = {{Reynolds}, S.~P.},
        title = "{Particle acceleration in supernova-remnant shocks}",
      journal = {\apss},
     keywords = {Supernova remnants, Shock acceleration, X-ray emission, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2011",
        month = "Nov",
       volume = {336},
       number = {1},
        pages = {257-262},
          doi = {10.1007/s10509-010-0559-8},
archivePrefix = {arXiv},
       eprint = {1012.1306},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011Ap&SS.336..257R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{reimer_apss_309_2007,
       author = {{Reimer}, Anita and {Reimer}, Olaf and {Pohl}, Martin},
        title = "{Gamma rays from colliding winds of massive stars}",
      journal = {\apss},
     keywords = {Astrophysics},
         year = "2007",
        month = "Jun",
       volume = {309},
       number = {1-4},
        pages = {351-357},
          doi = {10.1007/s10509-007-9462-3},
archivePrefix = {arXiv},
       eprint = {astro-ph/0611647},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2007Ap&SS.309..351R},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{radhakrishnan_japa_1980,
   author = {{Radhakrishnan}, V. and {Srinivasan}, G.},
    title = "{Evidence for a Large Population of Shocked Interstellar Clouds}",
  journal = {Journal of Astrophysics and Astronomy},
 keywords = {21 CM ABSORPTION, SHOCKED CLOUDS, SPIN TEMPERATURE, HIGH VELOCITIES},
     year = 1980,
    month = sep,
   volume = 1,
    pages = {47-66},
      doi = {10.1007/BF02727949},
   adsurl = {http://adsabs.harvard.edu/abs/1980JApA....1...47R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{raga_rmxaa_33_1997,
   author = {{Raga}, A.~C. and {Noriega-Crespo}, A. and {Cant{\'o}}, J. and 
	{Steffen}, W. and {van Buren}, D. and {Mellema}, G. and {Lundqvist}, P.
	},
    title = "{The Bow Shock and H II Regions around a Runaway O Star}",
  journal = {\rmxaa},
     year = 1997,
    month = oct,
   volume = 33,
    pages = {73-81},
   adsurl = {http://adsabs.harvard.edu/abs/1997RMxAA..33...73R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{raga_apj_300_1086,
   author = {{Raga}, A.~C.},
    title = "{'Stromgren region' analysis of cometary H II regions}",
  journal = {\apj},
 keywords = {COMETS, H II REGIONS, NEBULAE, STELLAR MOTIONS, ASTRONOMICAL MODELS, GAS IONIZATION, PHOTONS, STELLAR ENVELOPES},
     year = 1986,
    month = jan,
   volume = 300,
    pages = {745-748},
      doi = {10.1086/163849},
   adsurl = {http://adsabs.harvard.edu/abs/1986ApJ...300..745R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{raga_apjs_109_1997,
   author = {{Raga}, A.~C. and {Mellema}, G. and {Lundqvist}, P.},
    title = "{An Axisymmetric, Radiative Bow Shock Model with a Realistic Treatment of Ionization and Cooling}",
  journal = {\apjs},
   eprint = {arXiv:astro-ph/9610134},
 keywords = {ATOMIC DATA, METHODS: NUMERICAL, RADIATIVE TRANSFER, SHOCK WAVES, STARS: PRE-MAIN-SEQUENCE},
     year = 1997,
    month = apr,
   volume = 109,
    pages = {517},
      doi = {10.1086/312987},
   adsurl = {http://adsabs.harvard.edu/abs/1997ApJS..109..517R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rand_apj_343_1989,
   author = {{Rand}, R.~J. and {Kulkarni}, S.~R.},
    title = "{The local Galactic magnetic field}",
  journal = {\apj},
 keywords = {Interstellar Magnetic Fields, Milky Way Galaxy, Pulsars, Astronomical Models, Field Strength, Stellar Rotation},
     year = 1989,
    month = aug,
   volume = 343,
    pages = {760-772},
      doi = {10.1086/167747},
   adsurl = {http://adsabs.harvard.edu/abs/1989ApJ...343..760R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rakowski_apj_590_2003,
   author = {{Rakowski}, C.~E. and {Ghavamian}, P. and {Hughes}, J.~P.},
    title = "{The Physics of Supernova Remnant Blast Waves. II. Electron-Ion Equilibration in DEM L71 in the Large Magellanic Cloud}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0303069},
 keywords = {ISM: Individual: Alphanumeric: DEM L71, ISM: Individual: Alphanumeric: SNR 0505-67.9, Shock Waves, ISM: Supernova Remnants, X-Rays: ISM},
     year = 2003,
    month = jun,
   volume = 590,
    pages = {846-857},
      doi = {10.1086/375162},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...590..846R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{reach_aj_131_2006,
   author = {{Reach}, W.~T. and {Rho}, J. and {Tappe}, A. and {Pannuti}, T.~G. and 
	{Brogan}, C.~L. and {Churchwell}, E.~B. and {Meade}, M.~R. and 
	{Babler}, B. and {Indebetouw}, R. and {Whitney}, B.~A.},
    title = "{A Spitzer Space Telescope Infrared Survey of Supernova Remnants in the Inner Galaxy}",
  journal = {\aj},
   eprint = {astro-ph/0510630},
 keywords = {Infrared: ISM, Shock Waves, ISM: Supernova Remnants},
     year = 2006,
    month = mar,
   volume = 131,
    pages = {1479-1500},
      doi = {10.1086/499306},
   adsurl = {http://adsabs.harvard.edu/abs/2006AJ....131.1479R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{reach_apj_511_1999,
   author = {{Reach}, W.~T. and {Rho}, J.},
    title = "{Excitation and Disruption of a Giant Molecular Cloud by the Supernova Remnant 3C 391}",
  journal = {\apj},
   eprint = {astro-ph/9804142},
 keywords = {ISM: INDIVIDUAL: ALPHANUMERIC: 3C 391, ISM: STRUCTURE, RADIO LINES: ISM, ISM: SUPERNOVA REMNANTS, ISM: Individual: Alphanumeric: 3C 391, ISM: Structure, Radio Lines: ISM, ISM: Supernova Remnants},
     year = 1999,
    month = feb,
   volume = 511,
    pages = {836-846},
      doi = {10.1086/306703},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJ...511..836R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@BOOK{rybicki_rap_1979,
   author = {{Rybicki}, G.~B. and {Lightman}, A.~P.},
    title = "{Radiative processes in astrophysics}",
 keywords = {Astrophysics, Radiative Transfer, Atomic Structure, Bremsstrahlung, Compton Effect, Covariance, Kinematics, Molecular Structure, Plasma Radiation, Radiation Distribution, Relativistic Effects, Synchrotron Radiation},
booktitle = {New York, Wiley-Interscience, 1979.~393 p.},
     year = 1979,
   adsurl = {http://adsabs.harvard.edu/abs/1979rpa..book.....R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{roepks_apj_668_2007,
   author = {{R{\"o}pke}, F.~K.},
    title = "{Flame-driven Deflagration-to-Detonation Transitions in Type Ia Supernovae?}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0709.4095},
 keywords = {Hydrodynamics, Instabilities, Methods: Numerical, Stars: Supernovae: General, Turbulence},
     year = 2007,
    month = oct,
   volume = 668,
    pages = {1103-1108},
      doi = {10.1086/520830},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...668.1103R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{reid_apj_705_2009,
   author = {{Reid}, M.~J. and {Menten}, K.~M. and {Zheng}, X.~W. and {Brunthaler}, A. and 
	{Xu}, Y.},
    title = "{A Trigonometric Parallax of Sgr B2}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0908.3637},
 primaryClass = "astro-ph.GA",
 keywords = {astrometry, Galaxy: fundamental parameters, Galaxy: halo, Galaxy: kinematics and dynamics, Galaxy: structure, stars: formation},
     year = 2009,
    month = nov,
   volume = 705,
    pages = {1548-1553},
      doi = {10.1088/0004-637X/705/2/1548},
   adsurl = {http://adsabs.harvard.edu/abs/2009ApJ...705.1548R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{roepke_apj_660_2007,
   author = {{R{\"o}pke}, F.~K. and {Woosley}, S.~E. and {Hillebrandt}, W.
	},
    title = "{Off-Center Ignition in Type Ia Supernovae. I. Initial Evolution and Implications for Delayed Detonation}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0609088},
 keywords = {Hydrodynamics, Instabilities, Methods: Numerical, Stars: Supernovae: General, Turbulence},
     year = 2007,
    month = may,
   volume = 660,
    pages = {1344-1356},
      doi = {10.1086/512769},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...660.1344R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{robitaille_aa_536_2011,
   author = {{Robitaille}, T.~P.},
    title = "{HYPERION: an open-source parallelized three-dimensional dust continuum radiative transfer code}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1112.1071},
 primaryClass = "astro-ph.IM",
 keywords = {methods: numerical, radiative transfer, scattering, polarization},
     year = 2011,
    month = dec,
   volume = 536,
      eid = {A79},
    pages = {A79},
      doi = {10.1051/0004-6361/201117150},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...536A..79R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{roepke_aa_420_2004,
   author = {{R{\"o}pke}, F.~K. and {Hillebrandt}, W. and {Niemeyer}, J.~C.
	},
    title = "{The cellular burning regime in type Ia supernova explosions. I. Flame propagation into quiescent fuel}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0312092},
 keywords = {stars: supernovae: general, hydrodynamics, instabilities},
     year = 2004,
    month = jun,
   volume = 420,
    pages = {411-422},
      doi = {10.1051/0004-6361:20035721},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...420..411R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{roepke_aa_421_2004,
   author = {{R{\"o}pke}, F.~K. and {Hillebrandt}, W. and {Niemeyer}, J.~C.
	},
    title = "{The cellular burning regime in type Ia supernova explosions. II. Flame propagation into vortical fuel}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0312203},
 keywords = {stars: supernovae: general, hydrodynamics, instabilities, turbulence},
     year = 2004,
    month = jul,
   volume = 421,
    pages = {783-795},
      doi = {10.1051/0004-6361:20035778},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...421..783R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{rozyczka_274_MNRAS_1995,
   author = {{Rozyczka}, M. and {Tenorio-Tagle}, G.},
    title = "{The evolution of compact supernova remnants in a strongly magnetized medium}",
  journal = {\mnras},
 keywords = {ISM: JETS AND OUTFLOWS, ISM: MAGNETIC FIELDS, SUPERNOVA REMNANTS, GALAXIES: ACTIVE},
     year = 1995,
    month = jun,
   volume = 274,
    pages = {1157-1164},
   adsurl = {http://adsabs.harvard.edu/abs/1995MNRAS.274.1157R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{rozyczka_aa_167_1986,
   author = {{Rozyczka}, M. and {Tenorio-Tagle}, G. and {Bodenheimer}, P.
	},
    title = "{Non-spherical supernova remnants. III - Oblique shock reflections and anomalous H I velocity features}",
  journal = {\aap},
 keywords = {Collisions, Interstellar Matter, Mach Reflection, Supernova Remnants, Adiabatic Conditions, Radiant Cooling, Two Dimensional Models},
     year = 1986,
    month = oct,
   volume = 167,
    pages = {120-128},
   adsurl = {http://adsabs.harvard.edu/abs/1986A%26A...167..120R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{rozyczka_mnras_261_1993,
   author = {{Rozyczka}, M. and {Tenorio-Tagle}, G. and {Franco}, J. and 
	{Bodenheimer}, P.},
    title = "{On the evolution of supernova remnants. III - Off-centred supernova explosions in pre-existing wind-driven bubbles}",
  journal = {\mnras},
 keywords = {Plasma Bubbles, Stellar Evolution, Stellar Winds, Supernova Remnants, Interstellar Matter, Stellar Structure},
     year = 1993,
    month = apr,
   volume = 261,
    pages = {674-680},
   adsurl = {http://adsabs.harvard.edu/abs/1993MNRAS.261..674R},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE S 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{schneiter_mnras_449_2015,
       author = {{Schneiter}, E.~M. and {Vel{\'a}zquez}, P.~F. and {Reynoso}, E.~M. and {Esquivel}, A. and {De Colle}, F.},
        title = "{3D MHD simulation of polarized emission in SN 1006}",
      journal = {\mnras},
     keywords = {MHD, radiation mechanisms: general, methods: numerical, supernovae: individual: SN 1006, ISM: supernova remnants, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2015,
        month = may,
       volume = {449},
       number = {1},
        pages = {88-93},
          doi = {10.1093/mnras/stv279},
archivePrefix = {arXiv},
       eprint = {1502.03133},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015MNRAS.449...88S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{smartt_arra_2009,
       author = {{Smartt}, Stephen J.},
        title = "{Progenitors of Core-Collapse Supernovae}",
      journal = {\araa},
     keywords = {Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Cosmology and Nongalactic Astrophysics},
         year = 2009,
        month = sep,
       volume = {47},
       number = {1},
        pages = {63-106},
          doi = {10.1146/annurev-astro-082708-101737},
archivePrefix = {arXiv},
       eprint = {0908.0700},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2009ARA&A..47...63S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}





@BOOK{shu_pavi_book_1992,
       author = {{Shu}, F.~H.},
        title = "{The physics of astrophysics. Volume II: Gas dynamics.}",
         year = 1992,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992pavi.book.....S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{stock_mnras_409_2010,
       author = {{Stock}, D.~J. and {Barlow}, M.~J.},
        title = "{A search for ejecta nebulae around Wolf-Rayet stars using the SHS H{\ensuremath{\alpha}} survey}",
      journal = {\mnras},
     keywords = {circumstellar matter, stars: evolution, stars: massive, stars: Wolf-Rayet, Astrophysics - Astrophysics of Galaxies},
         year = 2010,
        month = dec,
       volume = {409},
       number = {4},
        pages = {1429-1440},
          doi = {10.1111/j.1365-2966.2010.17124.x},
archivePrefix = {arXiv},
       eprint = {1006.0625},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2010MNRAS.409.1429S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{Sander2012,
       author = {{Sander}, A. and {Hamann}, W. -R. and {Todt}, H.},
        title = "{The Galactic WC stars. Stellar parameters from spectral analyses indicate a new evolutionary sequence}",
      journal = {\aap},
     keywords = {stars: massive, stars: mass-loss, stars: Wolf-Rayet, stars: evolution, stars: atmospheres, stars: winds, outflows, Astrophysics - Solar and Stellar Astrophysics},
         year = 2012,
        month = apr,
       volume = {540},
          eid = {A144},
        pages = {A144},
          doi = {10.1051/0004-6361/201117830},
archivePrefix = {arXiv},
       eprint = {1201.6354},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...540A.144S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{cruces_mnras_473_2018,
       author = {{S{\'a}nchez-Cruces}, M. and {Rosado}, M. and {Fuentes-Carrera}, I. and
         {Ambrocio-Cruz}, P.},
        title = "{Kinematics of the Galactic Supernova Remnant G109.1-1.0 (CTB 109)}",
      journal = {\mnras},
     keywords = {ISM: kinematics and dynamics, ISM: supernova remnants-G109.1-1.0-CTB 109, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2018",
        month = "Jan",
       volume = {473},
       number = {2},
        pages = {1705-1717},
          doi = {10.1093/mnras/stx2460},
archivePrefix = {arXiv},
       eprint = {1709.07986},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018MNRAS.473.1705S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{sasaki_apj_642_2006,
       author = {{Sasaki}, Manami and {Kothes}, Roland and {Plucinsky}, Paul P. and
         {Gaetz}, Terrance J. and {Brunt}, Christopher M.},
        title = "{Evidence for Shocked Molecular Gas in the Galactic Supernova Remnant CTB 109 (G109.1-1.0)}",
      journal = {\apjl},
     keywords = {ISM: Clouds, Shock Waves, ISM: Supernova Remnants, X-Rays: Individual: Alphanumeric: CTB 109, Astrophysics},
         year = "2006",
        month = "May",
       volume = {642},
       number = {2},
        pages = {L149-L152},
          doi = {10.1086/504844},
archivePrefix = {arXiv},
       eprint = {astro-ph/0604164},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006ApJ...642L.149S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{storey_aa_265_1992,
       author = {{Storey}, Michelle C. and {Staveley-Smith}, L. and {Manchester}, R.~N. and
         {Kesteven}, M.~J.},
        title = "{Bilateral symmetry in the supernova remnant G 296.5+10.0}",
      journal = {\aap},
     keywords = {Neutron Stars, Radio Sources (Astronomy), Supernova Remnants, Cross Correlation, Stellar Magnetic Fields, Stellar Mass Ejection, Stellar Models, Astrophysics},
         year = "1992",
        month = "Nov",
       volume = {265},
        pages = {752-756},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992A&A...265..752S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{sanyal_aa_597_2017,
       author = {{Sanyal}, D. and {Langer}, N. and {Sz{\'e}csi}, D. and {-C Yoon}, S. and
         {Grassitelli}, L.},
        title = "{Metallicity dependence of envelope inflation in massive stars}",
      journal = {\aap},
     keywords = {stars: evolution, stars: massive, stars: interiors, stars: mass-loss, Astrophysics - Solar and Stellar Astrophysics},
         year = "2017",
        month = "Jan",
       volume = {597},
          eid = {A71},
        pages = {A71},
          doi = {10.1051/0004-6361/201629612},
archivePrefix = {arXiv},
       eprint = {1611.07280},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017A&A...597A..71S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{seo_jkas_51_2018,
       author = {{Seo}, Jeongbhin and {Kang}, Hyesung and {Ryu}, Dongsu},
        title = "{The Contribution of Stellar Winds to Cosmic Ray Production}",
      journal = {Journal of Korean Astronomical Society},
     keywords = {stars: massive, stars: mass-loss, stars: winds, acceleration of particles, shock waves, cosmic rays, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = "2018",
        month = "Apr",
       volume = {51},
       number = {2},
        pages = {37-48},
          doi = {10.5303/JKAS.2018.51.2.37},
archivePrefix = {arXiv},
       eprint = {1804.07486},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018JKAS...51...37S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{schneps_apj_246_1981,
       author = {{Schneps}, M.~H. and {Haschick}, A.~D. and {Wright}, E.~L. and
         {Barrett}, A.~H.},
        title = "{The stellar wind bubble NGC 2359. I. CO, VLA, and optical observations.}",
      journal = {\apj},
         year = "1981",
        month = "Jan",
       volume = {243},
        pages = {184-196},
          doi = {10.1086/158582},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1981ApJ...243..184S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{smith_mnras_211_1984,
       author = {{Smith}, L.~J. and {Pettini}, M. and {Dyson}, J.~E. and
         {Hartquist}, T.~W.},
        title = "{The remarkavle kinematics of the WR wind-blown bubble RCW 58.}",
      journal = {\mnras},
     keywords = {Astronomical Models, Nebulae, Stellar Spectra, Stellar Winds, Wolf-Rayet Stars, Bubbles, Interstellar Matter, Iue, Ultraviolet Spectra, Visible Spectrum, Astrophysics},
         year = "1984",
        month = "Dec",
       volume = {211},
        pages = {679-693},
          doi = {10.1093/mnras/211.3.679},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1984MNRAS.211..679S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{schlegel_mnras_244_1990,
   author = {{Schlegel}, E.~M.},
    title = "{A new subclass of Type II supernovae?}",
  journal = {\mnras},
 keywords = {Stellar Evolution, Supernovae, Classifying, H Alpha Line, Stellar Spectra, Supernova 1987a},
     year = 1990,
    month = may,
   volume = 244,
    pages = {269-271},
   adsurl = {http://adsabs.harvard.edu/abs/1990MNRAS.244..269S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{schneiter_mnras_408_2010,
   author = {{Schneiter}, E.~M. and {Vel{\'a}zquez}, P.~F. and {Reynoso}, E.~M. and 
	{de Colle}, F.},
    title = "{An MHD study of SN 1006 and determination of the ambient magnetic field direction}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1006.1150},
 primaryClass = "astro-ph.SR",
 keywords = {MHD, radiation mechanisms: general, methods: numerical, supernovae: individual: SN 1006, ISM: supernova remnants},
     year = 2010,
    month = oct,
   volume = 408,
    pages = {430-435},
      doi = {10.1111/j.1365-2966.2010.17125.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.408..430S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{schonrich_mnras_403_2010,
   author = {{Sch{\"o}nrich}, R. and {Binney}, J. and {Dehnen}, W.},
    title = "{Local kinematics and the local standard of rest}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0912.3693},
 primaryClass = "astro-ph.GA",
 keywords = {stars: kinematics, Galaxy: disc, Galaxy: fundamental parameters, Galaxy: kinematics and dynamics, solar neighbourhood},
     year = 2010,
    month = apr,
   volume = 403,
    pages = {1829-1833},
      doi = {10.1111/j.1365-2966.2010.16253.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.403.1829S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{schure_mnras_435_2013,
   author = {{Schure}, K.~M. and {Bell}, A.~R.},
    title = "{Cosmic ray acceleration in young supernova remnants}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1307.6575},
 primaryClass = "astro-ph.HE",
 keywords = {acceleration of particles, instabilities, MHD, cosmic rays, ISM: supernova remnants},
     year = 2013,
    month = oct,
   volume = 435,
    pages = {1174-1185},
      doi = {10.1093/mnras/stt1371},
   adsurl = {http://adsabs.harvard.edu/abs/2013MNRAS.435.1174S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sedov_MoIzN_1977,
   author = {{Sedov}, L.~I.},
    title = "{Similarity methods and dimensional analysis in mechanics /8th revised edition/}",
  journal = {Moscow Izdatel Nauka},
 keywords = {DIMENSIONAL ANALYSIS, MATHEMATICAL MODELS, MECHANICS (PHYSICS), SIMILARITY THEOREM, AERODYNAMIC CHARACTERISTICS, ASTROPHYSICS, COMBUSTION PHYSICS, GAS DYNAMICS, PIPE FLOW, TURBULENT FLOW, UNSTEADY FLOW, VISCOUS FLOW, WAVE PROPAGATION},
     year = 1977,
   adsurl = {http://adsabs.harvard.edu/abs/1977MoIzN....Q....S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{seok_apj_779_2013,
   author = {{Seok}, J.~Y. and {Koo}, B.-C. and {Onaka}, T.},
    title = "{A Survey of Infrared Supernova Remnants in the Large Magellanic Cloud}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1312.0460},
 primaryClass = "astro-ph.HE",
 keywords = {dust, extinction, ISM: supernova remnants, Magellanic Clouds },
     year = 2013,
    month = dec,
   volume = 779,
      eid = {134},
    pages = {134},
      doi = {10.1088/0004-637X/779/2/134},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...779..134S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sexton_mnras_446_2015,
   author = {{Sexton}, R.~O. and {Povich}, M.~S. and {Smith}, N. and {Babler}, B.~L. and 
	{Meade}, M.~R. and {Rudolph}, A.~L.},
    title = "{Extended red objects and stellar-wind bow shocks in the Carina Nebula}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1410.3518},
 primaryClass = "astro-ph.SR",
 keywords = {shock waves, stars: early-type, stars: mass-loss, H II regions, open clusters and associations: individual (Carina Nebula), infrared: ISM},
     year = 2015,
    month = jan,
   volume = 446,
    pages = {1047-1059},
      doi = {10.1093/mnras/stu2143},
   adsurl = {http://adsabs.harvard.edu/abs/2015MNRAS.446.1047S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sharpless_apj_1959,
   author = {{Sharpless}, S.},
    title = "{A Catalogue of H II Regions.}",
  journal = {\apjs},
     year = 1959,
    month = dec,
   volume = 4,
    pages = {257},
      doi = {10.1086/190049},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1959ApJS....4..257S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shabala_mnras_405_2010,
   author = {{Shabala}, S.~S. and {Mead}, J.~M.~G. and {Alexander}, P.},
    title = "{Magnetic fields in galaxies - I. Radio discs in local late-type galaxies}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1003.3535},
 keywords = {turbulence, galaxies: evolution, galaxies: formation, galaxies: luminosity function, galaxies: magnetic fields},
     year = 2010,
    month = jul,
   volume = 405,
    pages = {1960-1968},
      doi = {10.1111/j.1365-2966.2010.16586.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.405.1960S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{shulyak_aap_428_2004,
   author = {{Shulyak}, D. and {Tsymbal}, V. and {Ryabchikova}, T. and {St{\"u}tz}, C. and 
	{Weiss}, W.~W.},
    title = "{Line-by-line opacity stellar model atmospheres}",
  journal = {\aap},
 keywords = {stars: atmospheres, stars: abundances, stars: chemically peculiar, stars: fundamental parameters, stars: individual: CU Vir, stars: individual: HD 124224},
     year = 2004,
    month = dec,
   volume = 428,
    pages = {993-1000},
      doi = {10.1051/0004-6361:20034169},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...428..993S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{smith_MNRAS_339_2003,
   author = {{Smith}, M.~D. and {Rosen}, A.},
    title = "{The instability of fast shocks in molecular clouds}",
  journal = {\mnras},
 keywords = {hydrodynamics, instabilities, molecular processes, shock waves, ISM: lines and bands, ISM: molecules},
     year = 2003,
    month = feb,
   volume = 339,
    pages = {133-147},
      doi = {10.1046/j.1365-8711.2003.06155.x},
   adsurl = {http://adsabs.harvard.edu/abs/2003MNRAS.339..133S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
  }

@ARTICLE{sterck_aa_343_1999,
   author = {{de Sterck}, H. and {Poedts}, S.},
    title = "{Field-aligned magnetohydrodynamic bow shock flows in the switch-on regime. Parameter study of the flow around a cylinder and results for the axi-symmetrical flow over a sphere}",
  journal = {\aap},
 keywords = {MAGNETOHYDRODYNAMICS (MHD), SHOCK WAVES, METHODS: NUMERICAL, SUN: CORONA, COMETS: GENERAL, PLANETS AND SATELLITES: GENERAL},
     year = 1999,
    month = mar,
   volume = 343,
    pages = {641-649},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1999A%26A...343..641D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{sterck_phpl_1998,
   author = {{de Sterck}, H. and {Low}, B.~C. and {Poedts}, S.},
    title = "{Complex magnetohydrodynamic bow shock topology in field-aligned low-{$\beta$} flow around a perfectly conducting cylinder}",
  journal = {Physics of Plasmas},
 keywords = {Plasma dynamics and flow, Magnetohydrodynamic and fluid equation, Plasma simulation, Shock waves and discontinuities, Plasma production and heating by shock waves and compression, Magnetosphere interactions, Solar wind plasma, sources of solar wind},
     year = 1998,
    month = nov,
   volume = 5,
    pages = {4015-4027},
      doi = {10.1063/1.873124},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1998PhPl....5.4015D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{stevens_apj_386_1992,
   author = {{Stevens}, I.~R. and {Blondin}, J.~M. and {Pollock}, A.~M.~T.	},
    title = "{Colliding winds from early-type stars in binary systems}",
  journal = {\apj},
 keywords = {BINARY STARS, EARLY STARS, PLASMA INTERACTIONS, STELLAR WINDS, WOLF-RAYET STARS, X RAY STARS, HYDRODYNAMIC EQUATIONS, RADIATIVE TRANSFER, SHOCK WAVE INTERACTION, STELLAR LUMINOSITY, STELLAR MODELS},
     year = 1992,
    month = feb,
   volume = 386,
    pages = {265-287},
      doi = {10.1086/171013},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJ...386..265S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{stroemgren_apj_89_1939,
   author = {{Str{\"o}mgren}, B.},
    title = "{The Physical State of Interstellar Hydrogen.}",
  journal = {\apj},
     year = 1939,
    month = may,
   volume = 89,
    pages = {526},
      doi = {10.1086/144074},
   adsurl = {http://adsabs.harvard.edu/abs/1939ApJ....89..526S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{stone_apjs_80_1992,
   author = {{Stone}, J.~M. and {Norman}, M.~L.},
    title = "{ZEUS-2D: A radiation magnetohydrodynamics code for astrophysical flows in two space dimensions. I - The hydrodynamic algorithms and tests.}",
  journal = {\apjs},
 keywords = {Computational Astrophysics, Cosmic Plasma, Hydrodynamic Equations, Magnetohydrodynamic Flow, Self Consistent Fields, Computational Grids, Finite Difference Theory, Plasma Radiation, Poisson Equation, Radiative Transfer},
     year = 1992,
    month = jun,
   volume = 80,
    pages = {753-790},
      doi = {10.1086/191680},
   adsurl = {http://adsabs.harvard.edu/abs/1992ApJS...80..753S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@Book{strunk_1918,
	title = "The elements of style",
	author = "W. Jr Strunk",
	edition = "New York",
	year = "1918"
}

@ARTICLE{spitzer_apj_164_1971,
   author = {{Spitzer}, Jr., L. and {Hart}, M.~H.},
    title = "{Random Gravitational Encounters and the Evolution of Spherical Systems. I. Method}",
  journal = {\apj},
     year = 1971,
    month = mar,
   volume = 164,
    pages = {399},
      doi = {10.1086/150855},
   adsurl = {http://adsabs.harvard.edu/abs/1971ApJ...164..399S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{spitzer_apj_166_1971,
   author = {{Spitzer}, Jr., L. and {Hart}, M.~H.},
    title = "{Random Gravitational Encounters and the Evolution of Spherical Systems. II. Models}",
  journal = {\apj},
     year = 1971,
    month = jun,
   volume = 166,
    pages = {483},
      doi = {10.1086/150977},
   adsurl = {http://adsabs.harvard.edu/abs/1971ApJ...166..483S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{spitzer_apj_173_1972,
   author = {{Spitzer}, Jr., L. and {Shapiro}, S.~L.},
    title = "{Random Gravitational Encounters and the Evolution of Spherical Systems. III. Halo}",
  journal = {\apj},
     year = 1972,
    month = may,
   volume = 173,
    pages = {529},
      doi = {10.1086/151442},
   adsurl = {http://adsabs.harvard.edu/abs/1972ApJ...173..529S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{spitzer_apj_175_1972,
   author = {{Spitzer}, Jr., L. and {Thuan}, T.~X.},
    title = "{Random Gravitational Encounters and the Evolution of Spherical Systems. IV Isolated Systems of Identical Stars}",
  journal = {\apj},
     year = 1972,
    month = jul,
   volume = 175,
    pages = {31},
      doi = {10.1086/151537},
   adsurl = {http://adsabs.harvard.edu/abs/1972ApJ...175...31S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@BOOK{spitzer_1962,
   author = {{Spitzer}, L.},
    title = "{Physics of Fully Ionized Gases}",
booktitle = {Physics of Fully Ionized Gases, New York: Interscience (2nd edition), 1962},
     year = 1962,
   adsurl = {http://adsabs.harvard.edu/abs/1962pfig.book.....S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{sutherland_apjs_88_1993,
   author = {{Sutherland}, R.~S. and {Dopita}, M.~A.},
    title = "{Cooling functions for low-density astrophysical plasmas}",
  journal = {\apjs},
 keywords = {Cooling Flows (Astrophysics), Cosmic Plasma, Nonequilibrium Ionization, One Dimensional Flow, Plasma Slabs, Radiative Transfer, Charge Exchange, Electron Impact, Grid Generation (Mathematics), Hydrogen Recombinations, Ionization, Mathematical Models, Metallicity, Photoionization, Radiative Recombination, Rarefied Plasmas, Resonance Lines},
     year = 1993,
    month = sep,
   volume = 88,
    pages = {253-327},
      doi = {10.1086/191823},
   adsurl = {http://adsabs.harvard.edu/abs/1993ApJS...88..253S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{soker_apj_484_1997,
   author = {{Soker}, N. and {Dgani}, R.},
    title = "{Interaction of Planetary Nebulae with a Magnetized ISM}",
  journal = {\apj},
 keywords = {Hydrodynamics, ISM: Magnetic Fields, Magnetohydrodynamics: MHD, ISM: Planetary Nebulae: General},
     year = 1997,
    month = jul,
   volume = 484,
    pages = {277-285},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1997ApJ...484..277S},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE T 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 
 
 
@ARTICLE{tilley_mnras_371_2006,
       author = {{Tilley}, David A. and {Balsara}, Dinshaw S. and {Howk}, J. Christopher},
        title = "{Simulations of mixed-morphology supernova remnants with anisotropic thermal conduction}",
      journal = {\mnras},
     keywords = {conduction: MHD: ISM: magnetic fields: supernova remnants: radio continuum: ISM: X-rays: ISM, conduction, MHD, ISM: magnetic fields, supernova remnants, radio continuum: ISM, X-rays: ISM, Astrophysics},
         year = 2006,
        month = sep,
       volume = {371},
       number = {3},
        pages = {1106-1112},
          doi = {10.1111/j.1365-2966.2006.10747.x},
archivePrefix = {arXiv},
       eprint = {astro-ph/0604474},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2006MNRAS.371.1106T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



 
@ARTICLE{Toala2018,
       author = {{Toal{\'a}}, J.~A. and {Oskinova}, L.~M. and {Hamann}, W. -R. and
         {Ignace}, R. et al. },
        title = "{On the Apparent Absence of Wolf-Rayet+Neutron Star Systems: The Curious Case of WR124}",
      journal = {\apjl},
     keywords = {circumstellar matter, ISM: jets and outflows, stars: massive, stars: evolution, stars: neutron, stars: Wolf─Rayet, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = dec,
       volume = {869},
       number = {1},
          eid = {L11},
        pages = {L11},
          doi = {10.3847/2041-8213/aaf39d},
archivePrefix = {arXiv},
       eprint = {1811.10691},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...869L..11T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
} 
 

@ARTICLE{telezhinsky_aph_35_2012,
       author = {{Telezhinsky}, I. and {Dwarkadas}, V.~V. and {Pohl}, M.},
        title = "{Particle spectra from acceleration at forward and reverse shocks of young Type Ia Supernova Remnants}",
      journal = {Astroparticle Physics},
     keywords = {Astrophysics - High Energy Astrophysical Phenomena},
         year = "2012",
        month = "Jan",
       volume = {35},
       number = {6},
        pages = {300-311},
          doi = {10.1016/j.astropartphys.2011.10.001},
archivePrefix = {arXiv},
       eprint = {1110.0361},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012APh....35..300T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{telezhinsky_aa_541_2012,
       author = {{Telezhinsky}, I. and {Dwarkadas}, V.~V. and {Pohl}, M.},
        title = "{Time-dependent escape of cosmic rays from supernova remnants, and their interaction with dense media}",
      journal = {\aap},
     keywords = {ISM: supernova remnants, ISM: clouds, cosmic rays, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2012",
        month = "May",
       volume = {541},
          eid = {A153},
        pages = {A153},
          doi = {10.1051/0004-6361/201118639},
archivePrefix = {arXiv},
       eprint = {1112.3194},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...541A.153T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{telezhinsky_aa_552_2013,
       author = {{Telezhinsky}, I. and {Dwarkadas}, V.~V. and {Pohl}, M.},
        title = "{Acceleration of cosmic rays by young core-collapse supernova remnants}",
      journal = {\aap},
     keywords = {ISM: supernova remnants, cosmic rays, magnetic fields, hydrodynamics, shock waves, radiation mechanisms: non-thermal, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2013",
        month = "Apr",
       volume = {552},
          eid = {A102},
        pages = {A102},
          doi = {10.1051/0004-6361/201220740},
archivePrefix = {arXiv},
       eprint = {1211.3627},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...552A.102T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{2014AJ....147...30T,
       author = {{Toal{\'a}}, J.~A. and {Guerrero}, M.~A. and {Gruendl}, R.~A. and
         {Chu}, Y. -H.},
        title = "{X-Ray Emission from the Wolf-Rayet Bubble NGC 6888. I. Chandra ACIS-S Observations}",
      journal = {\aj},
     keywords = {ISM: bubbles, ISM: individual objects: NGC 6888, stars: winds, outflows, stars: Wolf-Rayet, X-rays: individual: NGC 6888, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2014",
        month = "Feb",
       volume = {147},
       number = {2},
          eid = {30},
        pages = {30},
          doi = {10.1088/0004-6256/147/2/30},
archivePrefix = {arXiv},
       eprint = {1310.2801},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014AJ....147...30T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{toala_aj_147_2014,
       author = {{Toal{\'a}}, J.~A. and {Guerrero}, M.~A. and {Gruendl}, R.~A. and
         {Chu}, Y. -H.},
        title = "{X-Ray Emission from the Wolf-Rayet Bubble NGC 6888. I. Chandra ACIS-S Observations}",
      journal = {\aj},
     keywords = {ISM: bubbles, ISM: individual objects: NGC 6888, stars: winds, outflows, stars: Wolf-Rayet, X-rays: individual: NGC 6888, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2014",
        month = "Feb",
       volume = {147},
       number = {2},
          eid = {30},
        pages = {30},
          doi = {10.1088/0004-6256/147/2/30},
archivePrefix = {arXiv},
       eprint = {1310.2801},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014AJ....147...30T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{toala_aa_559_2013,
       author = {{Toal{\'a}}, J.~A. and {Guerrero}, M.~A.},
        title = "{Absence of hot gas within the Wolf-Rayet bubble around WR 16}",
      journal = {\aap},
     keywords = {circumstellar matter, stars: massive, stars: Wolf-Rayet, ISM: bubbles, pulsars: individual: WR16, Astrophysics - Solar and Stellar Astrophysics},
         year = "2013",
        month = "Nov",
       volume = {559},
          eid = {A52},
        pages = {A52},
          doi = {10.1051/0004-6361/201322286},
archivePrefix = {arXiv},
       eprint = {1309.0236},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2013A&A...559A..52T},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{toala_apj_838_2017,
   author = {{Toal{\'a}}, J.~A. and {Oskinova}, L.~M. and {Ignace}, R.},
    title = "{On the Absence of Non-thermal X-Ray Emission around Runaway O Stars}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1703.04059},
 primaryClass = "astro-ph.HE",
 keywords = {stars: massive, stars: mass-loss, stars: winds, outflows, X-rays: ISM},
     year = 2017,
    month = apr,
   volume = 838,
      eid = {L19},
    pages = {L19},
      doi = {10.3847/2041-8213/aa667c},
   adsurl = {http://adsabs.harvard.edu/abs/2017ApJ...838L..19T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{toala_apj_821_2016,
   author = {{Toal{\'a}}, J.~A. and {Oskinova}, L.~M. and {Gonz{\'a}lez-Gal{\'a}n}, A. and 
	{Guerrero}, M.~A. and {Ignace}, R. and {Pohl}, M.},
    title = "{X-Ray Observations of Bow Shocks around Runaway O Stars. The Case of {$\zeta$} Oph and BD+43{\deg}3654}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1602.07805},
 primaryClass = "astro-ph.HE",
 keywords = {stars: individual: {$\zeta$} Oph, BD+43{\deg}3654, stars: winds, outflows},
     year = 2016,
    month = apr,
   volume = 821,
      eid = {79},
    pages = {79},
      doi = {10.3847/0004-637X/821/2/79},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2016ApJ...821...79T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{tenoriotagle_aa_145_1985,
   author = {{Tenorio-Tagle}, G. and {Bodenheimer}, P. and {Yorke}, H.~W.
	},
    title = "{Non-spherical supernova remnants. II - The interaction of remnants with molecular clouds}",
  journal = {\aap},
 keywords = {Hydrodynamic Equations, Interstellar Matter, Molecular Clouds, Supernova Remnants, Ionizing Radiation, Morphology, Stellar Winds},
     year = 1985,
    month = apr,
   volume = 145,
    pages = {70-80},
   adsurl = {http://adsabs.harvard.edu/abs/1985A%26A...145...70T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}
     
@BOOK{1992pavi.book.....S,
       author = {{Shu}, F.~H.},
        title = "{The physics of astrophysics. Volume II: Gas dynamics.}",
         year = 1992,
       adsurl = {https://ui.adsabs.harvard.edu/abs/1992pavi.book.....S},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{tenoriotagle_aa_148_1985,
   author = {{Tenorio-Tagle}, G. and {Rozyczka}, M. and {Yorke}, H.~W.},
    title = "{The Cygnus loop - A supernova breaking out of a molecular cloud?}",
  journal = {\aap},
 keywords = {Computational Astrophysics, Cygnus Constellation, H Alpha Line, Molecular Clouds, Supernova Remnants, X Ray Sources, Astronomical Models, Density Distribution, Hydrodynamics, Isophotes, Radio Sources (Astronomy)},
     year = 1985,
    month = jul,
   volume = 148,
    pages = {52-58},
   adsurl = {http://adsabs.harvard.edu/abs/1985A%26A...148...52T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tenoriotagle_aa_182_1987,
   author = {{Tenorio-Tagle}, G. and {Bodenheimer}, P. and {Rozyczka}, M.
	},
    title = "{Nonspherical supernova remnants. IV - Sequential explosions in OB associations}",
  journal = {\aap},
 keywords = {B Stars, O Stars, Stellar Models, Stellar Structure, Supernova Remnants, Boundary Value Problems, Hydrodynamic Equations, Stellar Envelopes, Stellar Evolution, Taylor Instability, Two Dimensional Flow},
     year = 1987,
    month = aug,
   volume = 182,
    pages = {120-126},
   adsurl = {http://adsabs.harvard.edu/abs/1987A%26A...182..120T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tenoriotagle_mnras_244_1990,
   author = {{Tenorio-Tagle}, G. and {Bodenheimer}, P. and {Franco}, J. and 
	{Rozyczka}, M.},
    title = "{On the evolution of supernova remnants. I - Explosions inside pre-existing wind-driven bubbles}",
  journal = {\mnras},
 keywords = {Computational Astrophysics, Stellar Evolution, Stellar Mass Ejection, Stellar Winds, Supernova Remnants, Bubbles, Explosions, H Alpha Line, Kinetic Energy, Wind Velocity, X Ray Astronomy},
     year = 1990,
    month = jun,
   volume = 244,
    pages = {563-576},
   adsurl = {http://adsabs.harvard.edu/abs/1990MNRAS.244..563T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tenoriotagle_mnras_251_1991,
   author = {{Tenorio-Tagle}, G. and {Rozyczka}, M. and {Franco}, J. and 
	{Bodenheimer}, P.},
    title = "{On the evolution of supernova remnants. II - Two-dimensional calculations of explosions inside pre-existing wind-driven bubbles}",
  journal = {\mnras},
 keywords = {Astronomical Models, Star Distribution, Supernova Remnants, Two Dimensional Models, Interstellar Matter, Stellar Mass Ejection, Stellar Winds, Supernovae, Turbulent Mixing},
     year = 1991,
    month = jul,
   volume = 251,
    pages = {318-329},
   adsurl = {http://adsabs.harvard.edu/abs/1991MNRAS.251..318T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{toala_apj_737_2011,
   author = {{Toal{\'a}}, J.~A. and {Arthur}, S.~J.},
    title = "{Radiation-hydrodynamic Models of the Evolving Circumstellar Medium around Massive Stars}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1106.4493},
 primaryClass = "astro-ph.SR",
 keywords = {ISM: bubbles, ISM: kinematics and dynamics, stars: massive, stars: mass-loss, stars: winds, outflows},
     year = 2011,
    month = aug,
   volume = 737,
      eid = {100},
    pages = {100},
      doi = {10.1088/0004-637X/737/2/100},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...737..100T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tziamtzis_aa_527_2011,
   author = {{Tziamtzis}, A. and {Lundqvist}, P. and {Gr{\"o}ningsson}, P. and 
	{Nasoudi-Shoar}, S.},
    title = "{The outer rings of SN 1987A}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1008.3387},
 primaryClass = "astro-ph.SR",
 keywords = {line: profiles, ISM: supernova remnants, ISM: individual objects: SN 1987A},
     year = 2011,
    month = mar,
   volume = 527,
      eid = {A35},
    pages = {A35},
      doi = {10.1051/0004-6361/201015576},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...527A..35T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{tesileanu_aa_488_2008,
   author = {{Te{\c s}ileanu}, O. and {Mignone}, A. and {Massaglia}, S.},
    title = "{Simulating radiative astrophysical flows with the PLUTO code: a non-equilibrium, multi-species cooling function}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0807.3657},
 keywords = {radiation mechanisms: thermal, line: formation, ISM: Herbig-Haro objects, ISM: jets and outflows, methods: numerical, magnetohydrodynamics (MHD)},
     year = 2008,
    month = sep,
   volume = 488,
    pages = {429-440},
      doi = {10.1051/0004-6361:200809461},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...488..429T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{toledo_mnras_442_2014,
   author = {{Toledo-Roy}, J.~C. and {Esquivel}, A. and {Vel{\'a}zquez}, P.~F. and 
	{Reynoso}, E.~M.},
    title = "{A 3D numerical model for Kepler's supernova remnant}",
  journal = {\mnras},
 keywords = {hydrodynamics, radiation mechanisms: thermal, methods: numerical, ISM: supernova remnants, X-rays: ISM},
     year = 2014,
    month = jul,
   volume = 442,
    pages = {229-238},
      doi = {10.1093/mnras/stu880},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.442..229T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{troland_301_apj_1986,
   author = {{Troland}, T.~H. and {Heiles}, C.},
    title = "{Interstellar magnetic field strengths and gas densities Observational and theoretical perspectives}",
  journal = {\apj},
 keywords = {Faraday Effect, Gas Density, Interstellar Gas, Interstellar Magnetic Fields, Pulsars, Zeeman Effect, H Alpha Line, Hydrogen Clouds},
     year = 1986,
    month = feb,
   volume = 301,
    pages = {339-345},
      doi = {10.1086/163904},
   adsurl = {http://adsabs.harvard.edu/abs/1986ApJ...301..339T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{truelove_apjs_120_1999,
   author = {{Truelove}, J.~K. and {McKee}, C.~F.},
    title = "{Evolution of Nonradiative Supernova Remnants}",
  journal = {\apjs},
 keywords = {HYDRODYNAMICS, SHOCK WAVES, ISM: SUPERNOVA REMNANTS, STARS: SUPERNOVAE: GENERAL},
     year = 1999,
    month = feb,
   volume = 120,
    pages = {299-326},
      doi = {10.1086/313176},
   adsurl = {http://adsabs.harvard.edu/abs/1999ApJS..120..299T},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE U 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{uyaniker_aa_426_2004,
       author = {{Uyan{\i}ker}, B. and {Reich}, W. and {Yar}, A. and {F{\"u}rst}, E.},
        title = "{Radio emission from the Cygnus Loop and its spectral characteristics}",
      journal = {\aap},
     keywords = {ISM: supernova remnants, ISM: individual objects: Cygnus Loop, radio continuum: ISM, Astrophysics},
         year = 2004,
        month = nov,
       volume = {426},
        pages = {909-924},
          doi = {10.1051/0004-6361:200400040},
archivePrefix = {arXiv},
       eprint = {astro-ph/0409176},
 primaryClass = {astro-ph},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2004A&A...426..909U},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{uchida_pasj_61_2009,
   author = {{Uchida}, H. and {Tsunemi}, H. and {Katsuda}, S. and {Kimura}, M. and 
	{Kosugi}, H.},
    title = "{Ejecta Distributions of Heavy Elements in the Cygnus Loop}",
  journal = {\pasj},
archivePrefix = "arXiv",
   eprint = {0901.3433},
 keywords = {ISM: abundances, ISM: individual (Cygnus Loop), ISM: supernova remnants, X-rays: ISM},
     year = 2009,
    month = feb,
   volume = 61,
    pages = {301-},
      doi = {10.1093/pasj/61.2.301},
   adsurl = {http://adsabs.harvard.edu/abs/2009PASJ...61..301U},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE V 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{villagran_mnras_491_2020,
       author = {{Villagran}, Marco A. and {Vel{\'a}zquez}, P.~F. and {G{\'o}mez}, D.~O. and {Giacani}, E.~B.},
        title = "{Evolving supernova remnants in multiphase interstellar media}",
      journal = {\mnras},
     keywords = {MHD, ISM: magnetic fields, ISM: supernova remnants, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2020,
        month = jan,
       volume = {491},
       number = {2},
        pages = {2855-2863},
          doi = {10.1093/mnras/stz2811},
archivePrefix = {arXiv},
       eprint = {1910.01668},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2020MNRAS.491.2855V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{vaidya_apj_865_2018,
       author = {{Vaidya}, Bhargav and {Mignone}, Andrea and {Bodo}, Gianluigi and
         {Rossi}, Paola and {Massaglia}, Silvano},
        title = "{A Particle Module for the PLUTO Code. II. Hybrid Framework for Modeling Nonthermal Emission from Relativistic Magnetized Flows}",
      journal = {\apj},
     keywords = {acceleration of particles, methods: numerical, polarization, radiation mechanisms: non-thermal, relativistic processes, shock waves, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Instrumentation and Methods for Astrophysics},
         year = 2018,
        month = oct,
       volume = {865},
       number = {2},
          eid = {144},
        pages = {144},
          doi = {10.3847/1538-4357/aadd17},
archivePrefix = {arXiv},
       eprint = {1808.08960},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...865..144V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{vanmarle_584_aa_2015,
       author = {{van Marle}, A.~J. and {Meliani}, Z. and {Marcowith}, A.},
        title = "{Shape and evolution of wind-blown bubbles of massive stars: on the effect of the interstellar magnetic field}",
      journal = {\aap},
     keywords = {magnetohydrodynamics (MHD), circumstellar matter, stars: massive, ISM: bubbles, ISM: magnetic fields, ISM: structure, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena, Physics - Space Physics},
         year = 2015,
        month = dec,
       volume = {584},
          eid = {A49},
        pages = {A49},
          doi = {10.1051/0004-6361/201425230},
archivePrefix = {arXiv},
       eprint = {1509.00192},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2015A&A...584A..49V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{voelk_apj_253_1982,
       author = {{Voelk}, H.~J. and {Forman}, M.},
        title = "{Cosmic rays and gamma-rays from OB stars}",
      journal = {\apj},
     keywords = {Cosmic Rays, Early Stars, Gamma Ray Astronomy, O Stars, Stellar Winds, Energetic Particles, Interstellar Matter, Nucleons, Particle Acceleration, Shock Wave Interaction, Astrophysics},
         year = "1982",
        month = "Feb",
       volume = {253},
        pages = {188-198},
          doi = {10.1086/159623},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1982ApJ...253..188V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{vallee_newar_55_2011,
   author = {{Vall{\'e}e}, J.~P.},
    title = "{Magnetic fields in the nearby Universe, as observed in solar and planetary realms, stars, and interstellar starforming nurseries}",
  journal = {\nar},
     year = 2011,
    month = may,
   volume = 55,
    pages = {23-90},
      doi = {10.1016/j.newar.2011.01.001},
   adsurl = {http://adsabs.harvard.edu/abs/2011NewAR..55...23V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{valle_ApJ_864_2018,
   author = {{del Valle}, M.~V. and {Pohl}, M.},
    title = "{Nonthermal Emission from Stellar Bow Shocks}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1807.05895},
 primaryClass = "astro-ph.HE",
 keywords = {gamma-rays: stars, hydrodynamics, radiation mechanisms: nonthermal, stars: winds, outflows },
     year = 2018,
    month = sep,
   volume = 864,
      eid = {19},
    pages = {19},
      doi = {10.3847/1538-4357/aad333},
   adsurl = {http://adsabs.harvard.edu/abs/2018ApJ...864...19D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{valle_mnras_448_2015,
   author = {{del Valle}, M.~V. and {Romero}, G.~E. and {Santos-Lima}, R.
	},
    title = "{Runaway stars as cosmic ray injectors inside molecular clouds}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1412.6535},
 primaryClass = "astro-ph.HE",
 keywords = {radiation mechanisms: non-thermal, ISM: clouds, cosmic rays, gamma-rays: ISM},
     year = 2015,
    month = mar,
   volume = 448,
    pages = {207-220},
      doi = {10.1093/mnras/stu2732},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2015MNRAS.448..207D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{vanburen_aspc_35_1993,
   author = {{van Buren}, D.},
    title = "{Stellar Wind Bow Shocks}",
booktitle = {Massive Stars:  Their Lives in the Interstellar Medium},
     year = 1993,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 35,
   editor = {{Cassinelli}, J.~P. and {Churchwell}, E.~B.},
    month = jan,
    pages = {315},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1993ASPC...35..315V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanburen_aj_110_1995,
   author = {{van Buren}, D. and {Noriega-Crespo}, A. and {Dgani}, R.},
    title = "{An IRAS/ISSA Survey of Bow Shocks Around Runaway Stars}",
  journal = {\aj},
 keywords = {ISM: STRUCTURE, STARS: ATMOSPHERES},
     year = 1995,
    month = dec,
   volume = 110,
    pages = {2914},
      doi = {10.1086/117739},
   adsurl = {http://cdsads.u-strasbg.fr/abs/1995AJ....110.2914V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanburen_apj_329_1988,
   author = {{van Buren}, D. and {McCray}, R.},
    title = "{Bow shocks and bubbles are seen around hot stars by IRAS}",
  journal = {\apjl},
 keywords = {Bow Waves, Early Stars, Hot Stars, Infrared Stars, Interstellar Matter, Plasma Bubbles, Stellar Winds, Cosmic Dust, H Ii Regions, Infrared Astronomy Satellite, Radiation Pressure, Stellar Luminosity},
     year = 1988,
    month = jun,
   volume = 329,
    pages = {L93-L96},
      doi = {10.1086/185184},
   adsurl = {http://adsabs.harvard.edu/abs/1988ApJ...329L..93V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vandishoeck_aa_279_1993,
   author = {{van Dishoeck}, E.~F. and {Jansen}, D.~J. and {Phillips}, T.~G.
	},
    title = "{Submillimeter observations of the shocked molecular gas associated with the supernova remnant IC 443}",
  journal = {\aap},
 keywords = {Astronomical Models, Interstellar Gas, Molecular Gases, Molecular Spectra, Radio Astronomy, Shock Wave Interaction, Submillimeter Waves, Supernova Remnants, Abundance, Astronomical Spectroscopy, Hydrodynamics, Line Spectra, Mathematical Models, Radio Spectra},
     year = 1993,
    month = nov,
   volume = 279,
    pages = {541-566},
   adsurl = {http://adsabs.harvard.edu/abs/1993A%26A...279..541V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanallen_apj_71_2003,
   author = {{van Allen}, J.~A.},
    title = "{Gravitational assist in celestial mechanics-a tutorial}",
  journal = {American Journal of Physics},
 keywords = {Educational aids, Relativity and gravitation, Celestial mechanics, Celestial mechanics, Surveys and tutorial papers; resource letters, Spaceborne and space research instruments, apparatus, and components, Lunar, planetary, and deep-space probes, Experimental tests of gravitational theories},
     year = 2003,
    month = may,
   volume = 71,
    pages = {448-451},
      doi = {10.1119/1.1539102},
   adsurl = {http://adsabs.harvard.edu/abs/2003AmJPh..71..448V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@INPROCEEDINGS{vanmarle_revmexaa_22_2004,
   author = {{van Marle}, A.~J. and {Langer}, N. and {Garc{\'{\i}}a-Segura}, G.
	},
    title = "{Wind-Blown Bubbles around Massive Stars. The effects of stellar wind and photo-ionization on the circumstellar Medium}",
 keywords = {H II regions, stars: Circumstellar matter, Stars: mass loss, Stars: winds, outflows},
booktitle = {Revista Mexicana de Astronomia y Astrofisica Conference Series},
     year = 2004,
   series = {Revista Mexicana de Astronomia y Astrofisica Conference Series},
   volume = 22,
   editor = "{G.~Garcia-Segura, G.~Tenorio-Tagle, J.~Franco, \& H.~W.~Yorke
	}",
    month = dec,
    pages = {136-139},
   adsurl = {http://adsabs.harvard.edu/abs/2004RMxAC..22..136V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@PHDTHESIS{vanmarle_phd_2006,
   author = {{van Marle}, A.~J.},
    title = "{Models for the circumstellar medium of long gamma-ray burst progenitor candidates}",
 keywords = {afterglow, gamma-ray burst, circumstellar medium, stellar wind, hydrodynamics},
   school = {Utrecht University},
     year = 2006,
    month = May,
   adsurl = {http://adsabs.harvard.edu/abs/2006PhDT........80V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_apj_734_2011,
   author = {{van Marle}, A.~J. and {Meliani}, Z. and {Keppens}, R. and {Decin}, L.
	},
    title = "{Computing the Dust Distribution in the Bow Shock of a Fast-moving, Evolved Star}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1105.2387},
 primaryClass = "astro-ph.SR",
 keywords = {hydrodynamics, infrared: ISM, ISM: abundances, ISM: kinematics and dynamics, stars: winds, outflows},
     year = 2011,
    month = jun,
   volume = 734,
      eid = {L26},
    pages = {L26},
      doi = {10.1088/2041-8205/734/2/L26},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...734L..26V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_aa_444_2005,
   author = {{van Marle}, A.~J. and {Langer}, N. and {Garc{\'{\i}}a-Segura}, G.
	},
    title = "{Constraints on gamma-ray burst and supernova progenitors through circumstellar absorption lines}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0507659},
 keywords = {, stars: winds, outflows, stars: Wolf-Rayet, stars: supernovae: general, gamma rays: bursts, line: profiles, ISM: bubbles},
     year = 2005,
    month = dec,
   volume = 444,
    pages = {837-847},
      doi = {10.1051/0004-6361:20053520},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...444..837V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_aa_469_2007,
   author = {{van Marle}, A.~J. and {Langer}, N. and {Garc{\'{\i}}a-Segura}, G.
	},
    title = "{Constraints on gamma-ray burst and supernova progenitors through circumstellar absorption lines. II. Post-LBV Wolf-Rayet stars}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0704.2073},
 keywords = {stars: winds, outflows, stars: Wolf-Rayet, stars: supernovae: general, gamma rays: bursts, line: profiles, ISM: bubbles},
     year = 2007,
    month = jul,
   volume = 469,
    pages = {941-948},
      doi = {10.1051/0004-6361:20077207},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...469..941V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_aa_460_2006,
   author = {{van Marle}, A.~J. and {Langer}, N. and {Achterberg}, A. and 
	{Garc{\'{\i}}a-Segura}, G.},
    title = "{Forming a constant density medium close to long gamma-ray bursts}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0605698},
 keywords = {stars: Wolf-Rayet, stars: winds, outflows, gamma rays: bursts, ISM: bubbles, hydrodynamics},
     year = 2006,
    month = dec,
   volume = 460,
    pages = {105-116},
      doi = {10.1051/0004-6361:20065709},
   adsurl = {http://adsabs.harvard.edu/abs/2006A%26A...460..105V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_mnras_407_2010,
   author = {{van Marle}, A.~J. and {Smith}, N. and {Owocki}, S.~P. and {van Veelen}, B.
	},
    title = "{Numerical models of collisions between core-collapse supernovae and circumstellar shells}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1004.2791},
 primaryClass = "astro-ph.HE",
 keywords = {hydrodynamics, methods: numerical, stars: mass-loss, supernovae: general, stars: winds, outflows, ISM: supernova remnants},
     year = 2010,
    month = oct,
   volume = 407,
    pages = {2305-2327},
      doi = {10.1111/j.1365-2966.2010.16851.x},
   adsurl = {http://adsabs.harvard.edu/abs/2010MNRAS.407.2305V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_aa_537_2012,
   author = {{Cox}, N.~L.~J. and {Kerschbaum}, F. and {van Marle}, A.-J. and 
	{Decin}, L. and {Ladjal}, D. and {Mayer}, A.},
    title = "{A far-infrared survey of bow shocks and detached shells around AGB stars and red supergiants}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1110.5486},
 primaryClass = "astro-ph.GA",
 keywords = {stars: AGB and post-AGB, circumstellar matter, infrared: ISM, hydrodynamics, stars: mass-loss, stars: winds, outflows},
     year = 2012,
    month = jan,
   volume = 537,
      eid = {A35},
    pages = {A35},
      doi = {10.1051/0004-6361/201117910},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26A...537A..35C},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_aa_527_2011,
   author = {{van Marle}, A.~J. and {Keppens}, R. and {Meliani}, Z.},
    title = "{Thin shell morphology in the circumstellar medium of massive binaries}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1011.1734},
 primaryClass = "astro-ph.GA",
 keywords = {hydrodynamics, binaries: general, circumstellar matter, stars: massive, stars: winds, outflows},
     year = 2011,
    month = mar,
   volume = 527,
      eid = {A3},
    pages = {A3},
      doi = {10.1051/0004-6361/201015517},
   adsurl = {http://adsabs.harvard.edu/abs/2011A%26A...527A...3V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{vanmarle_asp_355_2006,
   author = {{van Marle}, A.~J. and {Langer}, N. and {Garc{\'{\i}}a-Segura}, G.
	},
    title = "{The Impact of a Luminous Blue Variable on its Circumstellar Medium}",
booktitle = {Stars with the B[e] Phenomenon},
     year = 2006,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 355,
   editor = "{M.~Kraus \& A.~S.~Miroshnichenko}",
    month = dec,
    pages = {203},
   adsurl = {http://adsabs.harvard.edu/abs/2006ASPC..355..203V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_comp&fluids_2010pdf,
   author = {{van Marle}, A.~J. and {Keppens}, R.},
    title = "{Radiative cooling in numerical astrophysics: the need for adaptive mesh refinement}",
  journal = {ArXiv e-prints},
archivePrefix = "arXiv",
   eprint = {1011.2610},
 primaryClass = "astro-ph.IM",
 keywords = {Astrophysics - Instrumentation and Methods for Astrophysics},
     year = 2010,
    month = nov,
   adsurl = {http://adsabs.harvard.edu/abs/2010arXiv1011.2610V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_aa_561_2014,
   author = {{van Marle}, A.~J. and {Decin}, L. and {Meliani}, Z.},
    title = "{Can the magnetic field in the Orion arm inhibit the growth of instabilities in the bow shock of Betelgeuse?}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1312.5877},
 primaryClass = "astro-ph.SR",
 keywords = {magnetohydrodynamics (MHD), instabilities, circumstellar matter, stars: individual: alpha Orionis, ISM: bubbles, ISM: magnetic fields},
     year = 2014,
    month = jan,
   volume = 561,
      eid = {A152},
    pages = {A152},
      doi = {10.1051/0004-6361/201321968},
   adsurl = {http://adsabs.harvard.edu/abs/2014A%26A...561A.152V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_bull_srs_liege_80_2011,
   author = {{van Marle}, A.~J. and {Keppens}, R. and {Meliani}, Z.},
    title = "{3-D simulations of shells around massive stars}",
  journal = {Bulletin de la Societe Royale des Sciences de Liege},
archivePrefix = "arXiv",
   eprint = {1102.0104},
 primaryClass = "astro-ph.SR",
     year = 2011,
    month = jan,
   volume = 80,
    pages = {310-315},
   adsurl = {http://adsabs.harvard.edu/abs/2011BSRSL..80..310V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_apjl_734_2011,
   author = {{van Marle}, A.~J. and {Meliani}, Z. and {Keppens}, R. and {Decin}, L.
	},
    title = "{Computing the Dust Distribution in the Bow Shock of a Fast-moving, Evolved Star}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1105.2387},
 primaryClass = "astro-ph.SR",
 keywords = {hydrodynamics, infrared: ISM, ISM: abundances, ISM: kinematics and dynamics, stars: winds, outflows},
     year = 2011,
    month = jun,
   volume = 734,
      eid = {L26},
    pages = {L26},
      doi = {10.1088/2041-8205/734/2/L26},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...734L..26V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_2015,
   author = {{van Marle}, A.~J. and {Meliani}, Z. and {Marcowith}, A.},
    title = "{Shape and evolution of wind-blown bubbles of massive stars: on the effect of the interstellar magnetic field}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {1509.00192},
 primaryClass = "astro-ph.SR",
 keywords = {magnetohydrodynamics (MHD), circumstellar matter, stars: massive, ISM: bubbles, ISM: magnetic fields, ISM: structure},
     year = 2015,
    month = dec,
   volume = 584,
      eid = {A49},
    pages = {A49},
      doi = {10.1051/0004-6361/201425230},
   adsurl = {http://adsabs.harvard.edu/abs/2015A%26A...584A..49V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vanmarle_aa_478_2008,
   author = {{van Marle}, A.~J. and {Langer}, N. and {Yoon}, S.-C. and {Garc{\'{\i}}a-Segura}, G.
	},
    title = "{The circumstellar medium around a rapidly rotating, chemically homogeneously evolving, possible gamma-ray burst progenitor}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0711.4807},
 keywords = {gamma-rays: bursts, hydrodynamics, ISM: bubbles, stars: winds, outflows, stars: Wolf-Rayet},
     year = 2008,
    month = feb,
   volume = 478,
    pages = {769-778},
      doi = {10.1051/0004-6361:20078802},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...478..769V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vanmarle_aa_541_2012,
       author = {{van Marle}, A.~J. and {Meliani}, Z. and {Marcowith}, A.},
        title = "{A hydrodynamical model of the circumstellar bubble created by two massive stars}",
      journal = {\aap},
     keywords = {hydrodynamics, circumstellar matter, stars: winds, outflows, supernovae: general, ISM: bubbles, ISM: supernova remnants, Astrophysics - Solar and Stellar Astrophysics, Astrophysics - Astrophysics of Galaxies, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2012",
        month = "May",
       volume = {541},
          eid = {L8},
        pages = {L8},
          doi = {10.1051/0004-6361/201219180},
archivePrefix = {arXiv},
       eprint = {1204.2078},
 primaryClass = {astro-ph.SR},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2012A&A...541L...8V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@PhDThesis{ vanveelen_phd,
	title = "Supernovae interacting with their circumstellar medium",
	author = "van Veelen, B.",
	school = "Utrecht University",
	year = "2010",
	address = "Netherland"
}

@ARTICLE{vanveelen_aa_50_2009,
   author = {{van Veelen}, B. and {Langer}, N. and {Vink}, J. and {Garc{\'{\i}}a-Segura}, G. and 
	{van Marle}, A.~J.},
    title = "{The hydrodynamics of the supernova remnant Cassiopeia A. The influence of the progenitor evolution on the velocity structure and clumping}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0907.1197},
 primaryClass = "astro-ph.HE",
 keywords = {hydrodynamics, stars: winds, outflows, stars: supernovae: general, stars: supernovae: individual: Cas A},
     year = 2009,
    month = aug,
   volume = 503,
    pages = {495-503},
      doi = {10.1051/0004-6361/200912393},
   adsurl = {http://adsabs.harvard.edu/abs/2009A%26A...503..495V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{velazquez_apj_601_2004,
   author = {{Vel{\'a}zquez}, P.~F. and {Martinell}, J.~J. and {Raga}, A.~C. and 
	{Giacani}, E.~B.},
    title = "{Effects of Thermal Conduction on the X-Ray and Synchrotron Emission from Supernova Remnants}",
  journal = {\apj},
 keywords = {Conduction, ISM: Magnetic Fields, Methods: Numerical, ISM: Supernova Remnants, X-Rays: ISM},
     year = 2004,
    month = feb,
   volume = 601,
    pages = {885-895},
      doi = {10.1086/380755},
   adsurl = {http://adsabs.harvard.edu/abs/2004ApJ...601..885V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{velazquez_mnras_466_2017,
       author = {{Vel{\'a}zquez}, P.~F. and {Schneiter}, E.~M. and {Reynoso}, E.~M. and {Esquivel}, A. and {De Colle}, F. and {Toledo-Roy}, J.~C. and {G{\'o}mez}, D.~O. and {Sieyra}, M.~V. and {Moranchel-Basurto}, A.},
        title = "{A 3D MHD simulation of SN 1006: a polarized emission study for the turbulent case}",
      journal = {\mnras},
     keywords = {MHD, polarization, radiation mechanisms: general, methods: numerical, supernovae: individual: SN 1006, ISM: supernova remnants, Astrophysics - High Energy Astrophysical Phenomena, Astrophysics - Solar and Stellar Astrophysics},
         year = 2017,
        month = apr,
       volume = {466},
       number = {4},
        pages = {4851-4857},
          doi = {10.1093/mnras/stx064},
archivePrefix = {arXiv},
       eprint = {1701.05589},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2017MNRAS.466.4851V},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{velazquez_apj_649_2006,
   author = {{Vel{\'a}zquez}, P.~F. and {Vigh}, C.~D. and {Reynoso}, E.~M. and 
	{G{\'o}mez}, D.~O. and {Schneiter}, E.~M.},
    title = "{Simulated X-Ray Emission for a Runaway Model of Kepler's Supernova Remnant}",
  journal = {\apj},
 keywords = {Hydrodynamics, ISM: individual (Kepler SNR), Methods: Numerical, Shock Waves, ISM: Supernova Remnants, X-Rays: ISM},
     year = 2006,
    month = oct,
   volume = 649,
    pages = {779-787},
      doi = {10.1086/506899},
   adsurl = {http://adsabs.harvard.edu/abs/2006ApJ...649..779V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{velusamy,
   author = {{Velusamy}, T.},
    title = "{Guest Stars - Historical Supernovae and Remnants}",
booktitle = {IAU Colloq. 91: History of Oriental Astronomy},
     year = 1987,
   editor = {{Swarup}, G. and {Bag}, A.~K. and {Shukla}, K.~S.},
    pages = {265},
   adsurl = {http://adsabs.harvard.edu/abs/1987hooa.coll..265V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vollmer_aa_491_2008,
   author = {{Vollmer}, B. and {Beckert}, T. and {Davies}, R.~I.},
    title = "{Starbursts and torus evolution in AGN}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0809.3397},
 keywords = {galaxies: active, galaxies: nuclei, ISM: clouds, ISM: structure, ISM: kinematics and dynamics},
     year = 2008,
    month = nov,
   volume = 491,
    pages = {441-453},
      doi = {10.1051/0004-6361:200810446},
   adsurl = {http://adsabs.harvard.edu/abs/2008A%26A...491..441V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vieser_472_aa_2007,
   author = {{Vieser}, W. and {Hensler}, G.},
    title = "{The evolution of interstellar clouds in a streaming hot plasma including heat conduction}",
  journal = {\aap},
archivePrefix = "arXiv",
   eprint = {0704.3592},
 keywords = {ISM: clouds, conduction, hydrodynamics, instabilities},
     year = 2007,
    month = sep,
   volume = 472,
    pages = {141-153},
      doi = {10.1051/0004-6361:20042120},
   adsurl = {http://adsabs.harvard.edu/abs/2007A%26A...472..141V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vigh_apj_727_2011,
   author = {{Vigh}, C.~D. and {Vel{\'a}zquez}, P.~F. and {G{\'o}mez}, D.~O. and 
	{Reynoso}, E.~M. and {Esquivel}, A. and {Matias Schneiter}, E.
	},
    title = "{Asymmetries in the Expansion and Emission from Young Supernova Remnants}",
  journal = {\apj},
 keywords = {hydrodynamics, ISM: supernova remnants, methods: numerical, shock waves, supernovae: individual: Tycho},
     year = 2011,
    month = jan,
   volume = 727,
      eid = {32},
    pages = {32},
      doi = {10.1088/0004-637X/727/1/32},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...727...32V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{villaver_apj_748_2012,
   author = {{Villaver}, E. and {Manchado}, A. and {Garc{\'{\i}}a-Segura}, G.
	},
    title = "{The Interaction of Asymptotic Giant Branch Stars with the Interstellar Medium}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1201.3378},
 primaryClass = "astro-ph.GA",
 keywords = {hydrodynamics, ISM: kinematics and dynamics, ISM: structure, stars: AGB and post-AGB, stars: winds, outflows},
     year = 2012,
    month = apr,
   volume = 748,
      eid = {94},
    pages = {94},
      doi = {10.1088/0004-637X/748/2/94},
   adsurl = {http://adsabs.harvard.edu/abs/2012ApJ...748...94V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@INPROCEEDINGS{vink_asp_353_2006,
   author = {{Vink}, J.~S.},
    title = "{Massive star feedback -- from the first stars to the present}",
booktitle = {Stellar Evolution at Low Metallicity: Mass Loss, Explosions, Cosmology},
     year = 2006,
   series = {Astronomical Society of the Pacific Conference Series},
   volume = 353,
   eprint = {astro-ph/0511048},
   editor = {{Lamers}, H.~J.~G.~L.~M. and {Langer}, N. and {Nugis}, T. and 
	{Annuk}, K.},
    month = dec,
    pages = {113},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2006ASPC..353..113V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vink_aa_362_2000,
   author = {{Vink}, J.~S. and {de Koter}, A. and {Lamers}, H.~J.~G.~L.~M.
	},
    title = "{New theoretical mass-loss rates of O and B stars}",
  journal = {\aap},
   eprint = {astro-ph/0008183},
 keywords = {STARS: EARLY-TYPE, STARS: MASS-LOSS, STARS: SUPERGIANTS, STARS: WINDS, OUTFLOWS, STARS: EVOLUTION},
     year = 2000,
    month = oct,
   volume = 362,
    pages = {295-309},
   adsurl = {http://adsabs.harvard.edu/abs/2000A%26A...362..295V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vink_aa_369_2001,
   author = {{Vink}, J.~S. and {de Koter}, A. and {Lamers}, H.~J.~G.~L.~M.
	},
    title = "{Mass-loss predictions for O and B stars as a function of metallicity}",
  journal = {\aap},
   eprint = {astro-ph/0101509},
 keywords = {STARS: EARLY-TYPE, STARS: MASS-LOSS, STARS: SUPERGIANTS, STARS: WINDS, STARS: EVOLUTION},
     year = 2001,
    month = apr,
   volume = 369,
    pages = {574-588},
      doi = {10.1051/0004-6361:20010127},
   adsurl = {http://adsabs.harvard.edu/abs/2001A%26A...369..574V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vink_aa_307_1996,
   author = {{Vink}, J. and {Kaastra}, J.~S. and {Bleeker}, J.~A.~M.},
    title = "{A new mass estimate and puzzling abundances of SNR Cassiopeia A.}",
  journal = {\aap},
 keywords = {ISM: ABUNDANCES, ISM: INDIVIDUAL OBJECTS: CAS A, ISM: SUPERNOVA REMNANTS, X-RAYS: ISM},
     year = 1996,
    month = mar,
   volume = 307,
    pages = {L41-L44},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26A...307L..41V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vink_aa_328_1997,
   author = {{Vink}, J. and {Kaastra}, J.~S. and {Bleeker}, J.~A.~M.},
    title = "{X-ray spectroscopy of the supernova remnant RCW 86. A new challenge for modeling the emission from supernova remnants}",
  journal = {\aap},
 keywords = {ATOMIC PROCESSES, ISM: ABUNDANCES, ISM: INDIVIDUAL OBJECTS: RCW 86, ISM: SUPERNOVA REMNANTS, X-RAYS: ISM},
     year = 1997,
    month = dec,
   volume = 328,
    pages = {628-633},
   adsurl = {http://adsabs.harvard.edu/abs/1997A%26A...328..628V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{broersen_mnras_441_2014,
   author = {{Broersen}, S. and {Chiotellis}, A. and {Vink}, J. and {Bamba}, A.
	},
    title = "{The many sides of RCW 86: a Type Ia supernova remnant evolving in its progenitor's wind bubble}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {1404.5434},
 primaryClass = "astro-ph.HE",
 keywords = {supernovae: general, supernovae: individual: RCW 86, ISM: supernova remnants},
     year = 2014,
    month = jul,
   volume = 441,
    pages = {3040-3054},
      doi = {10.1093/mnras/stu667},
   adsurl = {http://adsabs.harvard.edu/abs/2014MNRAS.441.3040B},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{viallet_473_aa_2007,
   author = {{Viallet}, M. and {Baty}, H.},
    title = "{Spatial simulations of the Kelvin-Helmholtz instability in astrophysical jets. A partial stabilization mechanism for weakly magnetized transonic flows}",
  journal = {\aap},
 keywords = {instabilities, magnetohydrodynamics (MHD), ISM: jets and outflows, methods: numerical, plasmas},
     year = 2007,
    month = oct,
   volume = 473,
    pages = {1-9},
      doi = {10.1051/0004-6361:20066947},
   adsurl = {http://cdsads.u-strasbg.fr/abs/2007A%26A...473....1V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{vink_aarv_20_2012,
   author = {{Vink}, J.},
    title = "{Supernova remnants: the X-ray perspective}",
  journal = {\aapr},
archivePrefix = "arXiv",
   eprint = {1112.0576},
 primaryClass = "astro-ph.HE",
 keywords = {Supernova remnants, Supernovae, X-ray, Cosmic rays},
     year = 2012,
    month = dec,
   volume = 20,
    pages = {49},
      doi = {10.1007/s00159-011-0049-1},
   adsurl = {http://adsabs.harvard.edu/abs/2012A%26ARv..20...49V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{vishniac_apj_428_1994,
   author = {{Vishniac}, E.~T.},
    title = "{Nonlinear instabilities in shock-bounded slabs}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/9306025},
 keywords = {COSMOLOGY, HYDRODYNAMICS, INTERSTELLAR GAS, NONLINEARITY, NORMAL SHOCK WAVES, SLABS, STABILITY, ASTRONOMICAL MODELS, DIMENSIONAL ANALYSIS, GALACTIC EVOLUTION, STELLAR EVOLUTION, VORTICITY},
     year = 1994,
    month = jun,
   volume = 428,
    pages = {186-208},
      doi = {10.1086/174231},
   adsurl = {http://adsabs.harvard.edu/abs/1994ApJ...428..186V},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE W 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

@ARTICLE{webb_apj_298_1985,
       author = {{Webb}, G.~M. and {Axford}, W.~I. and {Forman}, M.~A.},
        title = "{Cosmic-ray acceleration at stellar wind terminal shocks}",
      journal = {\apj},
     keywords = {Galactic Cosmic Rays, Particle Acceleration, Shock Wave Propagation, Stellar Winds, Computational Astrophysics, Milky Way Galaxy, Terminal Velocity, Transport Theory, Space Radiation},
         year = "1985",
        month = "Nov",
       volume = {298},
        pages = {684-709},
          doi = {10.1086/163652},
       adsurl = {https://ui.adsabs.harvard.edu/abs/1985ApJ...298..684W},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{WareingZijlstraOBrien_2007_MNRAS_382_1233_AGB_bowshocks,
   author = {{Wareing}, C.~J. and {Zijlstra}, A.~A. and {O'Brien}, T.~J.},
    title = "{The interaction of planetary nebulae and their asymptotic giant branch progenitors with the interstellar medium}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0709.2848},
 keywords = {hydrodynamics, stars: AGB and post-AGB, stars: mass-loss, planetary nebulae: general, ISM: structure},
     year = 2007,
    month = dec,
   volume = 382,
    pages = {1233-1245},
      doi = {10.1111/j.1365-2966.2007.12459.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.382.1233W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wareing_apj_660_2007,
   author = {{Wareing}, C.~J. and {Zijlstra}, A.~A. and {O'Brien}, T.~J.},
    title = "{Vortices in the Wakes of Asymptotic Giant Branch Stars}",
  journal = {\apjl},
   eprint = {arXiv:astro-ph/0703732},
 keywords = {Stars: Circumstellar Matter, Hydrodynamics, ISM: Structure, Stars: AGB and Post-AGB, Stars: Mass Loss, Turbulence},
     year = 2007,
    month = may,
   volume = 660,
    pages = {L129-L132},
      doi = {10.1086/518308},
   adsurl = {http://adsabs.harvard.edu/abs/2007ApJ...660L.129W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wang_MNRAS_261_1993,
   author = {{Wang}, L. and {Dyson}, J.~E. and {Kahn}, F.~D.},
    title = "{The nature of the Napoleon's Hat nebula of SN 1987A}",
  journal = {\mnras},
 keywords = {NEBULAE, STELLAR ENVELOPES, STELLAR EVOLUTION, STELLAR MASS EJECTION, SUPERNOVA 1987A, BUBBLES, INTERSTELLAR MATTER, STELLAR MODELS, STELLAR WINDS},
     year = 1993,
    month = mar,
   volume = 261,
    pages = {391-395},
   adsurl = {http://adsabs.harvard.edu/abs/1993MNRAS.261..391W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wang_nature_1992,
   author = {{Wang}, L. and {Mazzali}, P.~A.},
    title = "{Dynamical development of a ring-like structure in the supernova 1987A nebula}",
  journal = {\nat},
 keywords = {STELLAR EVOLUTION, STELLAR STRUCTURE, STELLAR WINDS, SUPERNOVA REMNANTS, SUPERNOVA 1987A, BLUE STARS, PLANETARY NEBULAE, STELLAR MODELS, STELLAR ROTATION, WOLF-RAYET STARS},
     year = 1992,
    month = jan,
   volume = 355,
    pages = {58-61},
      doi = {10.1038/355058a0},
   adsurl = {http://adsabs.harvard.edu/abs/1992Natur.355...58W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wampler_apj_362_1990,
   author = {{Wampler}, E.~J. and {Wang}, L. and {Baade}, D. and {Banse}, K. and 
	{D'Odorico}, S. and {Gouiffes}, C. and {Tarenghi}, M.},
    title = "{Observations of the nebulosities near SN 1987A}",
  journal = {\apjl},
 keywords = {Astronomical Spectroscopy, Cosmic Dust, Interstellar Gas, Nebulae, Supernovae, Astronomical Observatories, Charge Coupled Devices, Galactic Evolution, Pixels, Stellar Luminosity, Ultraviolet Spectra},
     year = 1990,
    month = oct,
   volume = 362,
    pages = {L13-L16},
      doi = {10.1086/185836},
   adsurl = {http://adsabs.harvard.edu/abs/1990ApJ...362L..13W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wolfire_apj_587_2003,
   author = {{Wolfire}, M.~G. and {McKee}, C.~F. and {Hollenbach}, D. and 
	{Tielens}, A.~G.~G.~M.},
    title = "{Neutral Atomic Phases of the Interstellar Medium in the Galaxy}",
  journal = {\apj},
   eprint = {arXiv:astro-ph/0207098},
 keywords = {ISM: Clouds, ISM: General, ISM: Structure},
     year = 2003,
    month = apr,
   volume = 587,
    pages = {278-311},
      doi = {10.1086/368016},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...587..278W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{williams_apj_741_2011,
   author = {{Williams}, B.~J. and {Blair}, W.~P. and {Blondin}, J.~M. and 
	{Borkowski}, K.~J. and {Ghavamian}, P. and {Long}, K.~S. and 
	{Raymond}, J.~C. and {Reynolds}, S.~P. and {Rho}, J. and {Winkler}, P.~F.
	},
    title = "{RCW 86: A Type Ia Supernova in a Wind-blown Bubble}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1108.1207},
 primaryClass = "astro-ph.GA",
 keywords = {cosmic rays, dust, extinction, ISM: supernova remnants},
     year = 2011,
    month = nov,
   volume = 741,
      eid = {96},
    pages = {96},
      doi = {10.1088/0004-637X/741/2/96},
   adsurl = {http://adsabs.harvard.edu/abs/2011ApJ...741...96W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wit_aa_425_2004,
   author = {{de Wit}, W.~J. and {Testi}, L. and {Palla}, F. and {Vanzi}, L. and 
	{Zinnecker}, H.},
    title = "{The origin of massive O-type field stars.  I. A search for clusters}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0405348},
 keywords = {stars: early-type, stars: formation},
     year = 2004,
    month = oct,
   volume = 425,
    pages = {937-948},
      doi = {10.1051/0004-6361:20040454},
   adsurl = {http://adsabs.harvard.edu/abs/2004A%26A...425..937D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wit_aa_437_2005,
   author = {{de Wit}, W.~J. and {Testi}, L. and {Palla}, F. and {Zinnecker}, H.
	},
    title = "{The origin of massive O-type field stars: II. Field O stars as runaways}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0503337},
 keywords = {stars: early-type, stars: formation, Galaxy: stellar content, stars: kinematics},
     year = 2005,
    month = jul,
   volume = 437,
    pages = {247-255},
      doi = {10.1051/0004-6361:20042489},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...437..247D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{whalen_apj_682_2008,
   author = {{Whalen}, D. and {van Veelen}, B. and {O'Shea}, B.~W. and {Norman}, M.~L.
	},
    title = "{The Destruction of Cosmological Minihalos by Primordial Supernovae}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {0801.3698},
 keywords = {Cosmology: Theory, Cosmology: Early Universe, Hydrodynamics, Stars: Early-Type, Stars: Supernovae: Individual},
     year = 2008,
    month = jul,
   volume = 682,
    pages = {49-67},
      doi = {10.1086/589643},
   adsurl = {http://adsabs.harvard.edu/abs/2008ApJ...682...49W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{whiteoak_aas_118_1996,
   author = {{Whiteoak}, J.~B.~Z. and {Green}, A.~J.},
    title = "{The MOST supernova remnant catalogue (MSC).}",
  journal = {\aaps},
 keywords = {ISM: SUPERNOVA REMNANTS, RADIO CONTINUUM: ISM, ATLASES, CATALOGUES, SURVEYS},
     year = 1996,
    month = aug,
   volume = 118,
    pages = {329-380},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26AS..118..329W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{weaver_apj_218_1977,
   author = {{Weaver}, R. and {McCray}, R. and {Castor}, J. and {Shapiro}, P. and 
	{Moore}, R.},
    title = "{Interstellar bubbles. II - Structure and evolution}",
  journal = {\apj},
 keywords = {INTERSTELLAR GAS, PLASMA INTERACTIONS, STELLAR WINDS, ADIABATIC FLOW, BUBBLES, CONDUCTIVE HEAT TRANSFER, EARLY STARS, ENERGY DISSIPATION, HYDRODYNAMICS, ION DENSITY (CONCENTRATION), RADIATIVE TRANSFER, STELLAR MOTIONS},
     year = 1977,
    month = dec,
   volume = 218,
    pages = {377-395},
      doi = {10.1086/155692},
   adsurl = {http://adsabs.harvard.edu/abs/1977ApJ...218..377W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{weaver_errata_1978,
   author = {{Weaver}, R. and {McCray}, R. and {Castor}, J. and {Shapiro}, P. and 
	{Moore}, R.},
    title = "{Errata: Interstellar Bubbles. II. Structure and Evolution}",
  journal = {\apj},
     year = 1978,
    month = mar,
   volume = 220,
    pages = {742},
      doi = {10.1086/155960},
   adsurl = {http://adsabs.harvard.edu/abs/1978ApJ...220..742W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wilkin_459_apj_1996,
   author = {{Wilkin}, F.~P.},
    title = "{Exact Analytic Solutions for Stellar Wind Bow Shocks}",
  journal = {\apjl},
 keywords = {STARS: MASS LOSS, HYDRODYNAMICS, SHOCK WAVES, ISM: BUBBLES},
     year = 1996,
    month = mar,
   volume = 459,
    pages = {L31},
      doi = {10.1086/309939},
   adsurl = {http://adsabs.harvard.edu/abs/1996ApJ...459L..31W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{williams_apj_770_2013,
   author = {{Williams}, B.~J. and {Borkowski}, K.~J. and {Ghavamian}, P. and 
	{Hewitt}, J.~W. and {Mao}, S.~A. and {Petre}, R. and {Reynolds}, S.~P. and 
	{Blondin}, J.~M.},
    title = "{Azimuthal Density Variations around the Rim of Tycho's Supernova Remnant}",
  journal = {\apj},
archivePrefix = "arXiv",
   eprint = {1305.0567},
 primaryClass = "astro-ph.HE",
 keywords = {dust, extinction, ISM: supernova remnants},
     year = 2013,
    month = jun,
   volume = 770,
      eid = {129},
    pages = {129},
      doi = {10.1088/0004-637X/770/2/129},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...770..129W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wiersma_mnras_393_2009,
   author = {{Wiersma}, R.~P.~C. and {Schaye}, J. and {Smith}, B.~D.},
    title = "{The effect of photoionization on the cooling rates of enriched, astrophysical plasmas}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0807.3748},
 keywords = {atomic processes , plasmas , cooling flows , galaxies: formation , intergalactic medium},
     year = 2009,
    month = feb,
   volume = 393,
    pages = {99-107},
      doi = {10.1111/j.1365-2966.2008.14191.x},
   adsurl = {http://adsabs.harvard.edu/abs/2009MNRAS.393...99W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wit_aa_437_2005,
   author = {{de Wit}, W.~J. and {Testi}, L. and {Palla}, F. and {Zinnecker}, H.
	},
    title = "{The origin of massive O-type field stars: II. Field O stars as runaways}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0503337},
 keywords = {stars: early-type, stars: formation, Galaxy: stellar content, stars: kinematics},
     year = 2005,
    month = jul,
   volume = 437,
    pages = {247-255},
      doi = {10.1051/0004-6361:20042489},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...437..247D},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{woosley_rvmp_74_2002,
   author = {{Woosley}, S.~E. and {Heger}, A. and {Weaver}, T.~A.},
    title = "{The evolution and explosion of massive stars}",
  journal = {Reviews of Modern Physics},
 keywords = {Nucleosynthesis in novae supernovae and other explosive environments, Supernovae, Hydrostatic stellar nucleosynthesis, Elementary particle processes, Stellar structure interiors evolution nucleosynthesis ages, Neutron stars, Relativity and gravitation},
     year = 2002,
    month = nov,
   volume = 74,
    pages = {1015-1071},
      doi = {10.1103/RevModPhys.74.1015},
   adsurl = {http://adsabs.harvard.edu/abs/2002RvMP...74.1015W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{whiteoak_aas_118_1996,
   author = {{Whiteoak}, J.~B.~Z. and {Green}, A.~J.},
    title = "{The MOST supernova remnant catalogue (MSC).}",
  journal = {\aaps},
 keywords = {ISM: SUPERNOVA REMNANTS, RADIO CONTINUUM: ISM, ATLASES, CATALOGUES, SURVEYS},
     year = 1996,
    month = aug,
   volume = 118,
    pages = {329-380},
   adsurl = {http://adsabs.harvard.edu/abs/1996A%26AS..118..329W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{wright_aj_140_2010,
   author = {{Wright}, E.~L. and {Eisenhardt}, P.~R.~M. and {Mainzer}, A.~K. and 
	{Ressler}, M.~E. and {Cutri}, R.~M. and {Jarrett}, T. and {Kirkpatrick}, J.~D. and 
	{Padgett}, D. and {McMillan}, R.~S. and {Skrutskie}, M. and 
	{Stanford}, S.},
    title = "{The Wide-field Infrared Survey Explorer (WISE): Mission Description and Initial On-orbit Performance}",
  journal = {\aj},
archivePrefix = "arXiv",
   eprint = {1008.0031},
 primaryClass = "astro-ph.IM",
 keywords = {infrared: general, space vehicles, surveys},
     year = 2010,
    month = dec,
   volume = 140,
      eid = {1868},
    pages = {1868-1881},
      doi = {10.1088/0004-6256/140/6/1868},
   adsurl = {http://adsabs.harvard.edu/abs/2010AJ....140.1868W},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE Y 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{yoon_mnras_380_2007,
   author = {{Yoon}, S.-C. and {Podsiadlowski}, P. and {Rosswog}, S.},
    title = "{Remnant evolution after a carbon-oxygen white dwarf merger}",
  journal = {\mnras},
archivePrefix = "arXiv",
   eprint = {0704.0297},
 keywords = {accretion, accretion discs, stars: evolution, supernovae: general, white dwarfs},
     year = 2007,
    month = sep,
   volume = 380,
    pages = {933-948},
      doi = {10.1111/j.1365-2966.2007.12161.x},
   adsurl = {http://adsabs.harvard.edu/abs/2007MNRAS.380..933Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{yoon_apj_717_2012,
   author = {{Yoon}, S.-C. and {Cantiello}, M.},
    title = "{Evolution of Massive Stars with Pulsation-driven Superwinds During the Red Supergiant Phase}",
  journal = {\apjl},
archivePrefix = "arXiv",
   eprint = {1005.4925},
 primaryClass = "astro-ph.SR",
 keywords = {stars: evolution, stars: massive, stars: mass-loss, supergiants, supernovae: general},
     year = 2010,
    month = jul,
   volume = 717,
    pages = {L62-L65},
      doi = {10.1088/2041-8205/717/1/L62},
   adsurl = {http://adsabs.harvard.edu/abs/2010ApJ...717L..62Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{yoon_443_aa_2005,
   author = {{Yoon}, S.-C. and {Langer}, N.},
    title = "{Evolution of rapidly rotating metal-poor massive stars towards gamma-ray bursts}",
  journal = {\aap},
   eprint = {arXiv:astro-ph/0508242},
 keywords = {stars: rotation, stars: evolution, stars: Wolf-Rayet, supernovae: general, gamma rays: bursts},
     year = 2005,
    month = nov,
   volume = 443,
    pages = {643-648},
      doi = {10.1051/0004-6361:20054030},
   adsurl = {http://adsabs.harvard.edu/abs/2005A%26A...443..643Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{yusefzadeh_apj_585_2003,
   author = {{Yusef-Zadeh}, F. and {Wardle}, M. and {Rho}, J. and {Sakano}, M.
	},
    title = "{OH (1720 MHz) Masers and Mixed-Morphology Supernova Remnants}",
  journal = {\apj},
   eprint = {astro-ph/0211191},
 keywords = {ISM: Clouds, ISM: General, Shock Waves, ISM: Supernova Remnants, X-Rays: ISM},
     year = 2003,
    month = mar,
   volume = 585,
    pages = {319-323},
      doi = {10.1086/345932},
   adsurl = {http://adsabs.harvard.edu/abs/2003ApJ...585..319Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{yu_apj_194_1974,
   author = {{Yu}, G.},
    title = "{The interstellar wake of the solar wind}",
  journal = {\apj},
 keywords = {GAS COOLING, INTERPLANETARY MAGNETIC FIELDS, INTERSTELLAR SPACE, SOLAR WIND, WAKES, HYDROGEN, INTERSTELLAR GAS, INTERSTELLAR MAGNETIC FIELDS, MAGNETIC EFFECTS, MAGNETIC FIELD CONFIGURATIONS, PLASMA DYNAMICS, SHOCK WAVE PROPAGATION, SUBSONIC FLOW},
     year = 1974,
    month = nov,
   volume = 194,
    pages = {187-202},
      doi = {10.1086/153235},
   adsurl = {http://adsabs.harvard.edu/abs/1974ApJ...194..187Y},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%				LETTRE Z 			%%%%%%%%%%%
%%%%%%%					 			%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


@ARTICLE{zhou_apj_865_2018,
       author = {{Zhou}, Ping and {Li}, Jiang-Tao and {Zhang}, Zhi-Yu and {Vink}, Jacco and {Chen}, Yang and {Arias}, Maria and {Patnaude}, Daniel and {Bregman}, Joel N.},
        title = "{Molecular Gas toward Supernova Remnant Cassiopeia A}",
      journal = {\apj},
     keywords = {cosmic rays, ISM: individual objects: Cas A, ISM: molecules, ISM: supernova remnants, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2018,
        month = sep,
       volume = {865},
       number = {1},
          eid = {6},
        pages = {6},
          doi = {10.3847/1538-4357/aad960},
archivePrefix = {arXiv},
       eprint = {1808.03058},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018ApJ...865....6Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{zhou_apj_791_2014,
       author = {{Zhou}, Ping and {Safi-Harb}, Samar and {Chen}, Yang and {Zhang}, Xiao and {Jiang}, Bing and {Ferrand}, Gilles},
        title = "{An XMM-Newton Study of the Mixed-morphology Supernova Remnant W28 (G6.4-0.1)}",
      journal = {\apj},
     keywords = {cosmic rays, ISM: individual objects: G6.4-0.1 \&equals W28, ISM: supernova remnants, radiation mechanisms: non-thermal, radiation mechanisms: thermal, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2014,
        month = aug,
       volume = {791},
       number = {2},
          eid = {87},
        pages = {87},
          doi = {10.1088/0004-637X/791/2/87},
archivePrefix = {arXiv},
       eprint = {1407.6717},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014ApJ...791...87Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{zank_apj_763_2013,
   author = {{Zank}, G.~P. and {Heerikhuisen}, J. and {Wood}, B.~E. and {Pogorelov}, N.~V. and 
	{Zirnstein}, E. and {McComas}, D.~J.},
    title = "{Heliospheric Structure: The Bow Wave and the Hydrogen Wall}",
  journal = {\apj},
 keywords = {interplanetary medium, ISM: magnetic fields, local interstellar matter, plasmas, shock waves, solar wind, Sun: heliosphere},
     year = 2013,
    month = jan,
   volume = 763,
      eid = {20},
    pages = {20},
      doi = {10.1088/0004-637X/763/1/20},
   adsurl = {http://adsabs.harvard.edu/abs/2013ApJ...763...20Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zank_araa_53_2015,
   author = {{Zank}, G.~P.},
    title = "{Faltering Steps Into the Galaxy: The Boundary Regions of the Heliosphere}",
  journal = {\araa},
     year = 2015,
    month = aug,
   volume = 53,
    pages = {449-500},
      doi = {10.1146/annurev-astro-082214-122254},
   adsurl = {http://adsabs.harvard.edu/abs/2015ARA%26A..53..449Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zank_phpl_2001,
   author = {{Zank}, G.~P. and {M{\"u}ller}, H.-R. and {Wood}, B.~E.},
    title = "{The interaction of the solar wind and stellar winds with the partially ionized interstellar medium}",
  journal = {Physics of Plasmas},
 keywords = {Solar wind plasma, sources of solar wind, Surveys and tutorial papers, resource letters, Interstellar medium  and nebulae in Milky Way, Mass loss and stellar winds},
     year = 2001,
    month = may,
   volume = 8,
    pages = {2385-2393},
      doi = {10.1063/1.1345502},
   adsurl = {http://adsabs.harvard.edu/abs/2001PhPl....8.2385Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zank_ssrv_146_2009,
   author = {{Zank}, G.~P. and {Pogorelov}, N.~V. and {Heerikhuisen}, J. and 
	{Washimi}, H. and {Florinski}, V. and {Borovikov}, S. and {Kryukov}, I. and 
	{M{\"u}ller}, H.~R.},
    title = "{Physics of the Solar Wind-Local Interstellar Medium Interaction: Role of Magnetic Fields}",
  journal = {\ssr},
 keywords = {Solar wind boundaries, Interstellar medium, Pickup ions, Energetic neutral atoms},
     year = 2009,
    month = aug,
   volume = 146,
    pages = {295-327},
      doi = {10.1007/s11214-009-9497-6},
   adsurl = {http://adsabs.harvard.edu/abs/2009SSRv..146..295Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zavlin_aa_331_1998,
   author = {{Zavlin}, V.~E. and {Pavlov}, G.~G. and {Trumper}, J.},
    title = "{The neutron star in the supernova remnant PKS 1209-52}",
  journal = {\aap},
   eprint = {astro-ph/9709267},
 keywords = {STARS: NEUTRON, SUPERNOVAE: INDIVIDUAL PKS 1209-52, X-RAYS: STARS, RADIATION MECHANISMS: THERMAL},
     year = 1998,
    month = mar,
   volume = 331,
    pages = {821-828},
   adsurl = {http://adsabs.harvard.edu/abs/1998A%26A...331..821Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}

@ARTICLE{zhekov_mnras_443_2014,
       author = {{Zhekov}, Svetozar A.},
        title = "{X-rays from wind-blown bubbles: an XMM-Newton detection of NGC 2359}",
      journal = {\mnras},
     keywords = {shock waves, stars: individual: WR 7, ISM: bubbles, ISM: individual objects: NGC 2359, X-rays: ISM, X-rays: stars, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2014",
        month = "Sep",
       volume = {443},
       number = {1},
        pages = {12-18},
          doi = {10.1093/mnras/stu1138},
archivePrefix = {arXiv},
       eprint = {1406.2463},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2014MNRAS.443...12Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



@ARTICLE{zhekov_na_3_1998,
   author = {{Zhekov}, S.~A. and {Myasnikov}, A.~V.},
    title = "{1D gasdynamics of wind-blown bubbles: effects of thermal conduction}",
  journal = {\na},
 keywords = {Hydrodynamics, Conduction, Shock waves, ISM, bubbles, Hydrodynamics, Circumstellar shells, clouds, and expanding envelopes; circumstellar masers},
     year = 1998,
    month = mar,
   volume = 3,
    pages = {57-73},
      doi = {10.1016/S1384-1076(97)00043-2},
   adsurl = {http://adsabs.harvard.edu/abs/1998NewA....3...57Z},
  adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{zhou_apj_743_2011,
       author = {{Zhou}, Ping and {Chen}, Yang},
        title = "{Molecular Environment and an X-Ray Spectroscopy of Supernova Remnant Kesteven 78}",
      journal = {\apj},
     keywords = {ISM: individual objects: G32.8-0.1 = Kes 78, ISM: molecules, ISM: supernova remnants, Astrophysics - Astrophysics of Galaxies},
         year = 2011,
        month = dec,
       volume = {743},
       number = {1},
          eid = {4},
        pages = {4},
          doi = {10.1088/0004-637X/743/1/4},
archivePrefix = {arXiv},
       eprint = {1103.2527},
 primaryClass = {astro-ph.GA},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2011ApJ...743....4Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}


@ARTICLE{zhou_apj_831_2016,
       author = {{Zhou}, Ping and {Chen}, Yang and {Safi-Harb}, Samar and {Zhou}, Xin and {Sun}, Ming and {Zhang}, Zhi-Yu and {Zhang}, Gao-Yuan},
        title = "{Multi-wavelength Study of the Supernova Remnant Kes 79 (G33.6+0.1): On Its Supernova Properties and Expansion into a Molecular Environment}",
      journal = {\apj},
     keywords = {ISM: individual objects: G33.6+0.1 \& Kes 79, ISM: supernova remnants, pulsars: individual: PSR J1852+0040, Astrophysics - High Energy Astrophysical Phenomena},
         year = 2016,
        month = nov,
       volume = {831},
       number = {2},
          eid = {192},
        pages = {192},
          doi = {10.3847/0004-637X/831/2/192},
archivePrefix = {arXiv},
       eprint = {1612.03476},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2016ApJ...831..192Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}




@ARTICLE{zirakashvili_aph_98_2018,
       author = {{Zirakashvili}, V.~N. and {Ptuskin}, V.~S.},
        title = "{Cosmic ray acceleration in magnetic circumstellar bubbles}",
      journal = {Astroparticle Physics},
     keywords = {Cosmic rays, Acceleration, Supernovae, Astrophysics - High Energy Astrophysical Phenomena},
         year = "2018",
        month = "Mar",
       volume = {98},
        pages = {21-27},
          doi = {10.1016/j.astropartphys.2018.01.005},
archivePrefix = {arXiv},
       eprint = {1712.02174},
 primaryClass = {astro-ph.HE},
       adsurl = {https://ui.adsabs.harvard.edu/abs/2018APh....98...21Z},
      adsnote = {Provided by the SAO/NASA Astrophysics Data System}
}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%




